On the use of higher order waveforms in the search for gravitational waves emitted by compact binary coalescences

This thesis concerns the use, in gravitational wave data analysis, of higher order waveform models of the gravitational radiation emitted by compact binary coalescences. We begin with an introductory chapter that includes an overview of the theory of general relativity, gravitational radiation and ground-based interferometric gravitational wave detectors. We then discuss, in Chapter 2, the gravitational waves emitted by compact binary coalescences, with an explanation of higher order waveforms and how they differ from leading order waveforms; we also introduce the post-Newtonian formalism. In Chapter 3 the method and results of a gravitational wave search for low mass compact binary coalescences using a subset of LIGO's 5th science run data are presented and in the subsequent chapter we examine how one could use higher order waveforms in such analyses. We follow the development of a new search algorithm that incorporates higher order waveforms with promising results for detection efficiency and parameter estimation. In Chapter 5, a new method of windowing time-domain waveforms that offers benefit to gravitational wave searches is presented. The final chapter covers the development of a game designed as an outreach project to raise public awareness and understanding of the search for gravitational waves.

==> Figures/12to18bns.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{018}[cl][cl]{\matlabtextA 90\% Upper limit}%
\psfrag{019}[cl][cl]{\matlabtextA Combined}%
\psfrag{020}[cl][cl]{\matlabtextA S5YR1}%
\psfrag{021}[cl][cl]{\matlabtextA Month 4}%
\psfrag{022}[cl][cl]{\matlabtextA Month 5}%
\psfrag{023}[cl][cl]{\matlabtextA Month 3}%
\psfrag{024}[cl][cl]{\matlabtextA Month 6}%
\psfrag{025}[cl][cl]{\matlabtextA Month 2}%
\psfrag{026}[cl][cl]{\matlabtextA Month 0}%
\psfrag{027}[cl][cl]{\matlabtextA Month 1}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{028}[bc][bc]{\matlabtextB BNS (12-to-18 and S51YR)}%
\psfrag{029}[tc][tc]{\matlabtextB Rate /$\, {\rm yr}^{-1}{\rm L}^{-1}_{10}$}%
\psfrag{030}[bc][bc]{\matlabtextB Unnormalised probability}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $0$}%
\psfrag{001}[ct][ct]{\matlabtextC $0.01$}%
\psfrag{002}[ct][ct]{\matlabtextC $0.02$}%
\psfrag{003}[ct][ct]{\matlabtextC $0.03$}%
\psfrag{004}[ct][ct]{\matlabtextC $0.04$}%
\psfrag{005}[ct][ct]{\matlabtextC $0.05$}%
\psfrag{006}[ct][ct]{\matlabtextC $0.06$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{007}[rc][rc]{\matlabtextC $0$}%
\psfrag{008}[rc][rc]{\matlabtextC $0.1$}%
\psfrag{009}[rc][rc]{\matlabtextC $0.2$}%
\psfrag{010}[rc][rc]{\matlabtextC $0.3$}%
\psfrag{011}[rc][rc]{\matlabtextC $0.4$}%
\psfrag{012}[rc][rc]{\matlabtextC $0.5$}%
\psfrag{013}[rc][rc]{\matlabtextC $0.6$}%
\psfrag{014}[rc][rc]{\matlabtextC $0.7$}%
\psfrag{015}[rc][rc]{\matlabtextC $0.8$}%
\psfrag{016}[rc][rc]{\matlabtextC $0.9$}%
\psfrag{017}[rc][rc]{\matlabtextC $1$}%
%
%% </ytick>


==> Figures/L1-TMPLTBANK_DATAFIND-852351639-2048.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{12}{12}\selectfont\strut}%
\psfrag{014}[bc][bc]{\matlabtextA $\tau_3 /\, {\rm s}$}%
\psfrag{015}[tc][tc]{\matlabtextA $\tau_0 /\, {\rm s}$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $0$}%
\psfrag{001}[ct][ct]{\matlabtextB $5$}%
\psfrag{002}[ct][ct]{\matlabtextB $10$}%
\psfrag{003}[ct][ct]{\matlabtextB $15$}%
\psfrag{004}[ct][ct]{\matlabtextB $20$}%
\psfrag{005}[ct][ct]{\matlabtextB $25$}%
\psfrag{006}[ct][ct]{\matlabtextB $30$}%
\psfrag{007}[ct][ct]{\matlabtextB $35$}%
\psfrag{008}[ct][ct]{\matlabtextB $40$}%
\psfrag{009}[ct][ct]{\matlabtextB $45$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{010}[rc][rc]{\matlabtextB $0$}%
\psfrag{011}[rc][rc]{\matlabtextB $0.5$}%
\psfrag{012}[rc][rc]{\matlabtextB $1$}%
\psfrag{013}[rc][rc]{\matlabtextB $1.5$}%
%
%% </ytick>

==> Figures/ambbbh1.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{020}[bc][bc]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{021}[bc][bc]{\matlabtextB $\tau_3 /{\, \rm s}$}%
\psfrag{022}[tc][tc]{\matlabtextB $\tau_0 /{\, \rm s}$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{006}[ct][ct]{\matlabtextC $2$}%
\psfrag{007}[ct][ct]{\matlabtextC $4$}%
\psfrag{008}[ct][ct]{\matlabtextC $6$}%
\psfrag{009}[ct][ct]{\matlabtextC $8$}%
\psfrag{010}[ct][ct]{\matlabtextC $10$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{000}[lc][lc]{\matlabtextC $0$}%
\psfrag{001}[lc][lc]{\matlabtextC $0.2$}%
\psfrag{002}[lc][lc]{\matlabtextC $0.4$}%
\psfrag{003}[lc][lc]{\matlabtextC $0.6$}%
\psfrag{004}[lc][lc]{\matlabtextC $0.8$}%
\psfrag{005}[lc][lc]{\matlabtextC $1$}%
\psfrag{011}[rc][rc]{\matlabtextC $0.3$}%
\psfrag{012}[rc][rc]{\matlabtextC $0.4$}%
\psfrag{013}[rc][rc]{\matlabtextC $0.5$}%
\psfrag{014}[rc][rc]{\matlabtextC $0.6$}%
\psfrag{015}[rc][rc]{\matlabtextC $0.7$}%
\psfrag{016}[rc][rc]{\matlabtextC $0.8$}%
\psfrag{017}[rc][rc]{\matlabtextC $0.9$}%
\psfrag{018}[rc][rc]{\matlabtextC $1$}%
\psfrag{019}[rc][rc]{\matlabtextC $1.1$}%
%
%% </ytick>

==> Figures/ambbbh2.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{021}[bc][bc]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{022}[bc][bc]{\matlabtextB $\tau_3 /{\, \rm s}$}%
\psfrag{023}[tc][tc]{\matlabtextB $\tau_0 /{\, \rm s}$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{006}[ct][ct]{\matlabtextC $0$}%
\psfrag{007}[ct][ct]{\matlabtextC $1$}%
\psfrag{008}[ct][ct]{\matlabtextC $2$}%
\psfrag{009}[ct][ct]{\matlabtextC $3$}%
\psfrag{010}[ct][ct]{\matlabtextC $4$}%
\psfrag{011}[ct][ct]{\matlabtextC $5$}%
\psfrag{012}[ct][ct]{\matlabtextC $6$}%
\psfrag{013}[ct][ct]{\matlabtextC $7$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{000}[lc][lc]{\matlabtextC $0$}%
\psfrag{001}[lc][lc]{\matlabtextC $0.2$}%
\psfrag{002}[lc][lc]{\matlabtextC $0.4$}%
\psfrag{003}[lc][lc]{\matlabtextC $0.6$}%
\psfrag{004}[lc][lc]{\matlabtextC $0.8$}%
\psfrag{005}[lc][lc]{\matlabtextC $1$}%
\psfrag{014}[rc][rc]{\matlabtextC $0.2$}%
\psfrag{015}[rc][rc]{\matlabtextC $0.4$}%
\psfrag{016}[rc][rc]{\matlabtextC $0.6$}%
\psfrag{017}[rc][rc]{\matlabtextC $0.8$}%
\psfrag{018}[rc][rc]{\matlabtextC $1$}%
\psfrag{019}[rc][rc]{\matlabtextC $1.2$}%
\psfrag{020}[rc][rc]{\matlabtextC $1.4$}%
%
%% </ytick>

==> Figures/ambbns.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{020}[bc][bc]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{021}[bc][bc]{\matlabtextB $\tau_3 /{\, \rm s}$}%
\psfrag{022}[tc][tc]{\matlabtextB $\tau_0 /{\, \rm s}$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{006}[ct][ct]{\matlabtextC $22$}%
\psfrag{007}[ct][ct]{\matlabtextC $24$}%
\psfrag{008}[ct][ct]{\matlabtextC $26$}%
\psfrag{009}[ct][ct]{\matlabtextC $28$}%
\psfrag{010}[ct][ct]{\matlabtextC $30$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{000}[lc][lc]{\matlabtextC $0$}%
\psfrag{001}[lc][lc]{\matlabtextC $0.2$}%
\psfrag{002}[lc][lc]{\matlabtextC $0.4$}%
\psfrag{003}[lc][lc]{\matlabtextC $0.6$}%
\psfrag{004}[lc][lc]{\matlabtextC $0.8$}%
\psfrag{005}[lc][lc]{\matlabtextC $1$}%
\psfrag{011}[rc][rc]{\matlabtextC $0.82$}%
\psfrag{012}[rc][rc]{\matlabtextC $0.84$}%
\psfrag{013}[rc][rc]{\matlabtextC $0.86$}%
\psfrag{014}[rc][rc]{\matlabtextC $0.88$}%
\psfrag{015}[rc][rc]{\matlabtextC $0.9$}%
\psfrag{016}[rc][rc]{\matlabtextC $0.92$}%
\psfrag{017}[rc][rc]{\matlabtextC $0.94$}%
\psfrag{018}[rc][rc]{\matlabtextC $0.96$}%
\psfrag{019}[rc][rc]{\matlabtextC $0.98$}%
%
%% </ytick>

==> Figures/ambimbbh1.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{017}[bc][bc]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{018}[bc][bc]{\matlabtextB $\tau_3 /{\, \rm s}$}%
\psfrag{019}[tc][tc]{\matlabtextB $\tau_0 /{\, \rm s}$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{006}[ct][ct]{\matlabtextC $0$}%
\psfrag{007}[ct][ct]{\matlabtextC $1$}%
\psfrag{008}[ct][ct]{\matlabtextC $2$}%
\psfrag{009}[ct][ct]{\matlabtextC $3$}%
\psfrag{010}[ct][ct]{\matlabtextC $4$}%
\psfrag{011}[ct][ct]{\matlabtextC $5$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{000}[lc][lc]{\matlabtextC $0$}%
\psfrag{001}[lc][lc]{\matlabtextC $0.2$}%
\psfrag{002}[lc][lc]{\matlabtextC $0.4$}%
\psfrag{003}[lc][lc]{\matlabtextC $0.6$}%
\psfrag{004}[lc][lc]{\matlabtextC $0.8$}%
\psfrag{005}[lc][lc]{\matlabtextC $1$}%
\psfrag{012}[rc][rc]{\matlabtextC $0$}%
\psfrag{013}[rc][rc]{\matlabtextC $0.5$}%
\psfrag{014}[rc][rc]{\matlabtextC $1$}%
\psfrag{015}[rc][rc]{\matlabtextC $1.5$}%
\psfrag{016}[rc][rc]{\matlabtextC $2$}%
%
%% </ytick>

==> Figures/ambimbbh2.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{016}[bc][bc]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{017}[bc][bc]{\matlabtextB $\tau_3 /{\, \rm s}$}%
\psfrag{018}[tc][tc]{\matlabtextB $\tau_0 /{\, \rm s}$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{006}[ct][ct]{\matlabtextC $0$}%
\psfrag{007}[ct][ct]{\matlabtextC $0.5$}%
\psfrag{008}[ct][ct]{\matlabtextC $1$}%
\psfrag{009}[ct][ct]{\matlabtextC $1.5$}%
\psfrag{010}[ct][ct]{\matlabtextC $2$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{000}[lc][lc]{\matlabtextC $0$}%
\psfrag{001}[lc][lc]{\matlabtextC $0.2$}%
\psfrag{002}[lc][lc]{\matlabtextC $0.4$}%
\psfrag{003}[lc][lc]{\matlabtextC $0.6$}%
\psfrag{004}[lc][lc]{\matlabtextC $0.8$}%
\psfrag{005}[lc][lc]{\matlabtextC $1$}%
\psfrag{011}[rc][rc]{\matlabtextC $0$}%
\psfrag{012}[rc][rc]{\matlabtextC $0.5$}%
\psfrag{013}[rc][rc]{\matlabtextC $1$}%
\psfrag{014}[rc][rc]{\matlabtextC $1.5$}%
\psfrag{015}[rc][rc]{\matlabtextC $2$}%
%
%% </ytick>

==> Figures/ambnsbh.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{020}[bc][bc]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{021}[bc][bc]{\matlabtextB $\tau_3 /{\, \rm s}$}%
\psfrag{022}[tc][tc]{\matlabtextB $\tau_0 /{\, \rm s}$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{006}[ct][ct]{\matlabtextC $0$}%
\psfrag{007}[ct][ct]{\matlabtextC $5$}%
\psfrag{008}[ct][ct]{\matlabtextC $10$}%
\psfrag{009}[ct][ct]{\matlabtextC $15$}%
\psfrag{010}[ct][ct]{\matlabtextC $20$}%
\psfrag{011}[ct][ct]{\matlabtextC $25$}%
\psfrag{012}[ct][ct]{\matlabtextC $30$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{000}[lc][lc]{\matlabtextC $0$}%
\psfrag{001}[lc][lc]{\matlabtextC $0.2$}%
\psfrag{002}[lc][lc]{\matlabtextC $0.4$}%
\psfrag{003}[lc][lc]{\matlabtextC $0.6$}%
\psfrag{004}[lc][lc]{\matlabtextC $0.8$}%
\psfrag{005}[lc][lc]{\matlabtextC $1$}%
\psfrag{013}[rc][rc]{\matlabtextC $0.2$}%
\psfrag{014}[rc][rc]{\matlabtextC $0.4$}%
\psfrag{015}[rc][rc]{\matlabtextC $0.6$}%
\psfrag{016}[rc][rc]{\matlabtextC $0.8$}%
\psfrag{017}[rc][rc]{\matlabtextC $1$}%
\psfrag{018}[rc][rc]{\matlabtextC $1.2$}%
\psfrag{019}[rc][rc]{\matlabtextC $1.4$}%
%
%% </ytick>

==> Figures/ambnsbh_const.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{017}[bc][bc]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{018}[bc][bc]{\matlabtextB $\tau_3$}%
\psfrag{019}[tc][tc]{\matlabtextB $\tau_0$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{006}[ct][ct]{\matlabtextC $0$}%
\psfrag{007}[ct][ct]{\matlabtextC $5$}%
\psfrag{008}[ct][ct]{\matlabtextC $10$}%
\psfrag{009}[ct][ct]{\matlabtextC $15$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{000}[lc][lc]{\matlabtextC $0$}%
\psfrag{001}[lc][lc]{\matlabtextC $0.2$}%
\psfrag{002}[lc][lc]{\matlabtextC $0.4$}%
\psfrag{003}[lc][lc]{\matlabtextC $0.6$}%
\psfrag{004}[lc][lc]{\matlabtextC $0.8$}%
\psfrag{005}[lc][lc]{\matlabtextC $1$}%
\psfrag{010}[rc][rc]{\matlabtextC $0.2$}%
\psfrag{011}[rc][rc]{\matlabtextC $0.4$}%
\psfrag{012}[rc][rc]{\matlabtextC $0.6$}%
\psfrag{013}[rc][rc]{\matlabtextC $0.8$}%
\psfrag{014}[rc][rc]{\matlabtextC $1$}%
\psfrag{015}[rc][rc]{\matlabtextC $1.2$}%
\psfrag{016}[rc][rc]{\matlabtextC $1.4$}%
%
%% </ytick>

==> Figures/ampSNR10_1.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{12}{12}\selectfont\strut}%
\psfrag{019}[bc][bc]{\matlabtextA Recovered total mass /$M_\odot$}%
\psfrag{020}[tc][tc]{\matlabtextA Injected total mass /$M_\odot$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\fontsize{10}{10}\selectfont\strut}%
\psfrag{004}[ct][ct]{\matlabtextB $20$}%
\psfrag{005}[ct][ct]{\matlabtextB $40$}%
\psfrag{006}[ct][ct]{\matlabtextB $60$}%
\psfrag{007}[ct][ct]{\matlabtextB $80$}%
\psfrag{008}[ct][ct]{\matlabtextB $100$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{000}[lc][lc]{\matlabtextB $0$}%
\psfrag{001}[lc][lc]{\matlabtextB $5$}%
\psfrag{002}[lc][lc]{\matlabtextB $10$}%
\psfrag{003}[lc][lc]{\matlabtextB $15$}%
\psfrag{009}[rc][rc]{\matlabtextB $10$}%
\psfrag{010}[rc][rc]{\matlabtextB $20$}%
\psfrag{011}[rc][rc]{\matlabtextB $30$}%
\psfrag{012}[rc][rc]{\matlabtextB $40$}%
\psfrag{013}[rc][rc]{\matlabtextB $50$}%
\psfrag{014}[rc][rc]{\matlabtextB $60$}%
\psfrag{015}[rc][rc]{\matlabtextB $70$}%
\psfrag{016}[rc][rc]{\matlabtextB $80$}%
\psfrag{017}[rc][rc]{\matlabtextB $90$}%
\psfrag{018}[rc][rc]{\matlabtextB $100$}%
%
%% </ytick>

==> Figures/ampSNR10_1eta.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{12}{12}\selectfont\strut}%
\psfrag{021}[bc][bc]{\matlabtextA Recovered total mass /$M_\odot$}%
\psfrag{022}[tc][tc]{\matlabtextA Injected total mass /$M_\odot$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\fontsize{10}{10}\selectfont\strut}%
\psfrag{006}[ct][ct]{\matlabtextB $20$}%
\psfrag{007}[ct][ct]{\matlabtextB $40$}%
\psfrag{008}[ct][ct]{\matlabtextB $60$}%
\psfrag{009}[ct][ct]{\matlabtextB $80$}%
\psfrag{010}[ct][ct]{\matlabtextB $100$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{000}[lc][lc]{\matlabtextB $0$}%
\psfrag{001}[lc][lc]{\matlabtextB $0.05$}%
\psfrag{002}[lc][lc]{\matlabtextB $0.1$}%
\psfrag{003}[lc][lc]{\matlabtextB $0.15$}%
\psfrag{004}[lc][lc]{\matlabtextB $0.2$}%
\psfrag{005}[lc][lc]{\matlabtextB $0.25$}%
\psfrag{011}[rc][rc]{\matlabtextB $10$}%
\psfrag{012}[rc][rc]{\matlabtextB $20$}%
\psfrag{013}[rc][rc]{\matlabtextB $30$}%
\psfrag{014}[rc][rc]{\matlabtextB $40$}%
\psfrag{015}[rc][rc]{\matlabtextB $50$}%
\psfrag{016}[rc][rc]{\matlabtextB $60$}%
\psfrag{017}[rc][rc]{\matlabtextB $70$}%
\psfrag{018}[rc][rc]{\matlabtextB $80$}%
\psfrag{019}[rc][rc]{\matlabtextB $90$}%
\psfrag{020}[rc][rc]{\matlabtextB $100$}%
%
%% </ytick>

==> Figures/ampSNR10cons1fix.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{018}[bc][bc]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{019}[bc][bc]{\matlabtextB Recovered total mass /$\, M_\odot$}%
\psfrag{020}[tc][tc]{\matlabtextB Injected total mass /$\, M_\odot$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{004}[ct][ct]{\matlabtextC $20$}%
\psfrag{005}[ct][ct]{\matlabtextC $40$}%
\psfrag{006}[ct][ct]{\matlabtextC $60$}%
\psfrag{007}[ct][ct]{\matlabtextC $80$}%
\psfrag{008}[ct][ct]{\matlabtextC $100$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{000}[lc][lc]{\matlabtextC $0$}%
\psfrag{001}[lc][lc]{\matlabtextC $5$}%
\psfrag{002}[lc][lc]{\matlabtextC $10$}%
\psfrag{003}[lc][lc]{\matlabtextC $15$}%
\psfrag{009}[rc][rc]{\matlabtextC $20$}%
\psfrag{010}[rc][rc]{\matlabtextC $30$}%
\psfrag{011}[rc][rc]{\matlabtextC $40$}%
\psfrag{012}[rc][rc]{\matlabtextC $50$}%
\psfrag{013}[rc][rc]{\matlabtextC $60$}%
\psfrag{014}[rc][rc]{\matlabtextC $70$}%
\psfrag{015}[rc][rc]{\matlabtextC $80$}%
\psfrag{016}[rc][rc]{\matlabtextC $90$}%
\psfrag{017}[rc][rc]{\matlabtextC $100$}%
%
%% </ytick>

==> Figures/ampSNR10cons2.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{018}[bc][bc]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{019}[bc][bc]{\matlabtextB Recovered total mass /$\, M_\odot$}%
\psfrag{020}[tc][tc]{\matlabtextB Injected total mass /$\, M_\odot$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{004}[ct][ct]{\matlabtextC $20$}%
\psfrag{005}[ct][ct]{\matlabtextC $40$}%
\psfrag{006}[ct][ct]{\matlabtextC $60$}%
\psfrag{007}[ct][ct]{\matlabtextC $80$}%
\psfrag{008}[ct][ct]{\matlabtextC $100$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{000}[lc][lc]{\matlabtextC $0$}%
\psfrag{001}[lc][lc]{\matlabtextC $5$}%
\psfrag{002}[lc][lc]{\matlabtextC $10$}%
\psfrag{003}[lc][lc]{\matlabtextC $15$}%
\psfrag{009}[rc][rc]{\matlabtextC $20$}%
\psfrag{010}[rc][rc]{\matlabtextC $30$}%
\psfrag{011}[rc][rc]{\matlabtextC $40$}%
\psfrag{012}[rc][rc]{\matlabtextC $50$}%
\psfrag{013}[rc][rc]{\matlabtextC $60$}%
\psfrag{014}[rc][rc]{\matlabtextC $70$}%
\psfrag{015}[rc][rc]{\matlabtextC $80$}%
\psfrag{016}[rc][rc]{\matlabtextC $90$}%
\psfrag{017}[rc][rc]{\matlabtextC $100$}%
%
%% </ytick>

==> Figures/ampSNR10cons2fix.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{018}[bc][bc]{\matlabtextA FWF (constrained)}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{019}[bc][bc]{\matlabtextB Recovered total mass /$\, M_\odot$}%
\psfrag{020}[tc][tc]{\matlabtextB Injected total mass /$\, M_\odot$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{004}[ct][ct]{\matlabtextC $20$}%
\psfrag{005}[ct][ct]{\matlabtextC $40$}%
\psfrag{006}[ct][ct]{\matlabtextC $60$}%
\psfrag{007}[ct][ct]{\matlabtextC $80$}%
\psfrag{008}[ct][ct]{\matlabtextC $100$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{000}[lc][lc]{\matlabtextC $0$}%
\psfrag{001}[lc][lc]{\matlabtextC $5$}%
\psfrag{002}[lc][lc]{\matlabtextC $10$}%
\psfrag{003}[lc][lc]{\matlabtextC $15$}%
\psfrag{009}[rc][rc]{\matlabtextC $20$}%
\psfrag{010}[rc][rc]{\matlabtextC $30$}%
\psfrag{011}[rc][rc]{\matlabtextC $40$}%
\psfrag{012}[rc][rc]{\matlabtextC $50$}%
\psfrag{013}[rc][rc]{\matlabtextC $60$}%
\psfrag{014}[rc][rc]{\matlabtextC $70$}%
\psfrag{015}[rc][rc]{\matlabtextC $80$}%
\psfrag{016}[rc][rc]{\matlabtextC $90$}%
\psfrag{017}[rc][rc]{\matlabtextC $100$}%
%
%% </ytick>

==> Figures/ampSNR10cons2fixeta.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{020}[bc][bc]{\matlabtextA FWF (constrained)}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{021}[bc][bc]{\matlabtextB Recovered total mass /$\, M_\odot$}%
\psfrag{022}[tc][tc]{\matlabtextB Injected total mass /$\, M_\odot$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{006}[ct][ct]{\matlabtextC $20$}%
\psfrag{007}[ct][ct]{\matlabtextC $40$}%
\psfrag{008}[ct][ct]{\matlabtextC $60$}%
\psfrag{009}[ct][ct]{\matlabtextC $80$}%
\psfrag{010}[ct][ct]{\matlabtextC $100$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{000}[lc][lc]{\matlabtextC $0$}%
\psfrag{001}[lc][lc]{\matlabtextC $0.05$}%
\psfrag{002}[lc][lc]{\matlabtextC $0.1$}%
\psfrag{003}[lc][lc]{\matlabtextC $0.15$}%
\psfrag{004}[lc][lc]{\matlabtextC $0.2$}%
\psfrag{005}[lc][lc]{\matlabtextC $0.25$}%
\psfrag{011}[rc][rc]{\matlabtextC $20$}%
\psfrag{012}[rc][rc]{\matlabtextC $30$}%
\psfrag{013}[rc][rc]{\matlabtextC $40$}%
\psfrag{014}[rc][rc]{\matlabtextC $50$}%
\psfrag{015}[rc][rc]{\matlabtextC $60$}%
\psfrag{016}[rc][rc]{\matlabtextC $70$}%
\psfrag{017}[rc][rc]{\matlabtextC $80$}%
\psfrag{018}[rc][rc]{\matlabtextC $90$}%
\psfrag{019}[rc][rc]{\matlabtextC $100$}%
%
%% </ytick>

==> Figures/ampSNR10etanew.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{020}[bc][bc]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{021}[bc][bc]{\matlabtextB Recovered total mass /$\, M_\odot$}%
\psfrag{022}[tc][tc]{\matlabtextB Injected total mass /$\, M_\odot$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{006}[ct][ct]{\matlabtextC $20$}%
\psfrag{007}[ct][ct]{\matlabtextC $40$}%
\psfrag{008}[ct][ct]{\matlabtextC $60$}%
\psfrag{009}[ct][ct]{\matlabtextC $80$}%
\psfrag{010}[ct][ct]{\matlabtextC $100$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{000}[lc][lc]{\matlabtextC $0$}%
\psfrag{001}[lc][lc]{\matlabtextC $0.05$}%
\psfrag{002}[lc][lc]{\matlabtextC $0.1$}%
\psfrag{003}[lc][lc]{\matlabtextC $0.15$}%
\psfrag{004}[lc][lc]{\matlabtextC $0.2$}%
\psfrag{005}[lc][lc]{\matlabtextC $0.25$}%
\psfrag{011}[rc][rc]{\matlabtextC $20$}%
\psfrag{012}[rc][rc]{\matlabtextC $30$}%
\psfrag{013}[rc][rc]{\matlabtextC $40$}%
\psfrag{014}[rc][rc]{\matlabtextC $50$}%
\psfrag{015}[rc][rc]{\matlabtextC $60$}%
\psfrag{016}[rc][rc]{\matlabtextC $70$}%
\psfrag{017}[rc][rc]{\matlabtextC $80$}%
\psfrag{018}[rc][rc]{\matlabtextC $90$}%
\psfrag{019}[rc][rc]{\matlabtextC $100$}%
%
%% </ytick>

==> Figures/ampSNR10new.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{018}[bc][bc]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{019}[bc][bc]{\matlabtextB Recovered total mass /$\, M_\odot$}%
\psfrag{020}[tc][tc]{\matlabtextB Injected total mass /$\ ,M_\odot$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{004}[ct][ct]{\matlabtextC $20$}%
\psfrag{005}[ct][ct]{\matlabtextC $40$}%
\psfrag{006}[ct][ct]{\matlabtextC $60$}%
\psfrag{007}[ct][ct]{\matlabtextC $80$}%
\psfrag{008}[ct][ct]{\matlabtextC $100$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{000}[lc][lc]{\matlabtextC $0$}%
\psfrag{001}[lc][lc]{\matlabtextC $5$}%
\psfrag{002}[lc][lc]{\matlabtextC $10$}%
\psfrag{003}[lc][lc]{\matlabtextC $15$}%
\psfrag{009}[rc][rc]{\matlabtextC $20$}%
\psfrag{010}[rc][rc]{\matlabtextC $30$}%
\psfrag{011}[rc][rc]{\matlabtextC $40$}%
\psfrag{012}[rc][rc]{\matlabtextC $50$}%
\psfrag{013}[rc][rc]{\matlabtextC $60$}%
\psfrag{014}[rc][rc]{\matlabtextC $70$}%
\psfrag{015}[rc][rc]{\matlabtextC $80$}%
\psfrag{016}[rc][rc]{\matlabtextC $90$}%
\psfrag{017}[rc][rc]{\matlabtextC $100$}%
%
%% </ytick>

==> Figures/ampSNR10newnocon.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{018}[bc][bc]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{019}[bc][bc]{\matlabtextB Recovered total mass /$\, M_\odot$}%
\psfrag{020}[tc][tc]{\matlabtextB Injected total mass /$\, M_\odot$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{004}[ct][ct]{\matlabtextC $20$}%
\psfrag{005}[ct][ct]{\matlabtextC $40$}%
\psfrag{006}[ct][ct]{\matlabtextC $60$}%
\psfrag{007}[ct][ct]{\matlabtextC $80$}%
\psfrag{008}[ct][ct]{\matlabtextC $100$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{000}[lc][lc]{\matlabtextC $0$}%
\psfrag{001}[lc][lc]{\matlabtextC $5$}%
\psfrag{002}[lc][lc]{\matlabtextC $10$}%
\psfrag{003}[lc][lc]{\matlabtextC $15$}%
\psfrag{009}[rc][rc]{\matlabtextC $20$}%
\psfrag{010}[rc][rc]{\matlabtextC $30$}%
\psfrag{011}[rc][rc]{\matlabtextC $40$}%
\psfrag{012}[rc][rc]{\matlabtextC $50$}%
\psfrag{013}[rc][rc]{\matlabtextC $60$}%
\psfrag{014}[rc][rc]{\matlabtextC $70$}%
\psfrag{015}[rc][rc]{\matlabtextC $80$}%
\psfrag{016}[rc][rc]{\matlabtextC $90$}%
\psfrag{017}[rc][rc]{\matlabtextC $100$}%
%
%% </ytick>

==> Figures/ampSNR10nocon.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{018}[bc][bc]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{019}[bc][bc]{\matlabtextB Recovered total mass /$\, M_\odot$}%
\psfrag{020}[tc][tc]{\matlabtextB Injected total mass /$\, M_\odot$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{004}[ct][ct]{\matlabtextC $20$}%
\psfrag{005}[ct][ct]{\matlabtextC $40$}%
\psfrag{006}[ct][ct]{\matlabtextC $60$}%
\psfrag{007}[ct][ct]{\matlabtextC $80$}%
\psfrag{008}[ct][ct]{\matlabtextC $100$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{000}[lc][lc]{\matlabtextC $0$}%
\psfrag{001}[lc][lc]{\matlabtextC $5$}%
\psfrag{002}[lc][lc]{\matlabtextC $10$}%
\psfrag{003}[lc][lc]{\matlabtextC $15$}%
\psfrag{009}[rc][rc]{\matlabtextC $20$}%
\psfrag{010}[rc][rc]{\matlabtextC $30$}%
\psfrag{011}[rc][rc]{\matlabtextC $40$}%
\psfrag{012}[rc][rc]{\matlabtextC $50$}%
\psfrag{013}[rc][rc]{\matlabtextC $60$}%
\psfrag{014}[rc][rc]{\matlabtextC $70$}%
\psfrag{015}[rc][rc]{\matlabtextC $80$}%
\psfrag{016}[rc][rc]{\matlabtextC $90$}%
\psfrag{017}[rc][rc]{\matlabtextC $100$}%
%
%% </ytick>

==> Figures/ampevolve.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{12}{12}\selectfont\strut}%
\psfrag{000}[bc][bc]{\matlabtextA $A(t)$}%
\psfrag{001}[tc][tc]{\matlabtextA Time}%
%
%% </text>

==> Figures/ampmchirp.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{020}[bc][bc]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{021}[bc][bc]{\matlabtextB Recovered chirp mass /\, $M_\odot$}%
\psfrag{022}[tc][tc]{\matlabtextB Injected chirp mass /$\, M_\odot$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{006}[ct][ct]{\matlabtextC $0$}%
\psfrag{007}[ct][ct]{\matlabtextC $10$}%
\psfrag{008}[ct][ct]{\matlabtextC $20$}%
\psfrag{009}[ct][ct]{\matlabtextC $30$}%
\psfrag{010}[ct][ct]{\matlabtextC $40$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{000}[lc][lc]{\matlabtextC $0$}%
\psfrag{001}[lc][lc]{\matlabtextC $0.2$}%
\psfrag{002}[lc][lc]{\matlabtextC $0.4$}%
\psfrag{003}[lc][lc]{\matlabtextC $0.6$}%
\psfrag{004}[lc][lc]{\matlabtextC $0.8$}%
\psfrag{005}[lc][lc]{\matlabtextC $1$}%
\psfrag{011}[rc][rc]{\matlabtextC $0$}%
\psfrag{012}[rc][rc]{\matlabtextC $5$}%
\psfrag{013}[rc][rc]{\matlabtextC $10$}%
\psfrag{014}[rc][rc]{\matlabtextC $15$}%
\psfrag{015}[rc][rc]{\matlabtextC $20$}%
\psfrag{016}[rc][rc]{\matlabtextC $25$}%
\psfrag{017}[rc][rc]{\matlabtextC $30$}%
\psfrag{018}[rc][rc]{\matlabtextC $35$}%
\psfrag{019}[rc][rc]{\matlabtextC $40$}%
%
%% </ytick>

==> Figures/ampmtot.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{020}[bc][bc]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{021}[bc][bc]{\matlabtextB Recovered total mass /$\, M_\odot$}%
\psfrag{022}[tc][tc]{\matlabtextB Injected total mass /$\ ,M_\odot$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{006}[ct][ct]{\matlabtextC $20$}%
\psfrag{007}[ct][ct]{\matlabtextC $40$}%
\psfrag{008}[ct][ct]{\matlabtextC $60$}%
\psfrag{009}[ct][ct]{\matlabtextC $80$}%
\psfrag{010}[ct][ct]{\matlabtextC $100$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{000}[lc][lc]{\matlabtextC $0$}%
\psfrag{001}[lc][lc]{\matlabtextC $0.2$}%
\psfrag{002}[lc][lc]{\matlabtextC $0.4$}%
\psfrag{003}[lc][lc]{\matlabtextC $0.6$}%
\psfrag{004}[lc][lc]{\matlabtextC $0.8$}%
\psfrag{005}[lc][lc]{\matlabtextC $1$}%
\psfrag{011}[rc][rc]{\matlabtextC $20$}%
\psfrag{012}[rc][rc]{\matlabtextC $30$}%
\psfrag{013}[rc][rc]{\matlabtextC $40$}%
\psfrag{014}[rc][rc]{\matlabtextC $50$}%
\psfrag{015}[rc][rc]{\matlabtextC $60$}%
\psfrag{016}[rc][rc]{\matlabtextC $70$}%
\psfrag{017}[rc][rc]{\matlabtextC $80$}%
\psfrag{018}[rc][rc]{\matlabtextC $90$}%
\psfrag{019}[rc][rc]{\matlabtextC $100$}%
%
%% </ytick>

==> Figures/chidist.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{12}{12}\selectfont\strut}%
\psfrag{012}[bc][bc]{\matlabtextA Constrained $(10,20)M_\odot$}%
\psfrag{013}[tc][tc]{\matlabtextA SNR}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $0$}%
\psfrag{001}[ct][ct]{\matlabtextB $5$}%
\psfrag{002}[ct][ct]{\matlabtextB $10$}%
\psfrag{003}[ct][ct]{\matlabtextB $15$}%
%
%% </xtick>
%
%% <yscale>
%
\psfrag{004}[bc][bc]{\matlabtextB $\times10^{5}$}%
%
%% </yscale>
%
%% <ytick>
%
\psfrag{005}[rc][rc]{\matlabtextB $0$}%
\psfrag{006}[rc][rc]{\matlabtextB $0.5$}%
\psfrag{007}[rc][rc]{\matlabtextB $1$}%
\psfrag{008}[rc][rc]{\matlabtextB $1.5$}%
\psfrag{009}[rc][rc]{\matlabtextB $2$}%
\psfrag{010}[rc][rc]{\matlabtextB $2.5$}%
\psfrag{011}[rc][rc]{\matlabtextB $3$}%
%
%% </ytick>

==> Figures/chidistLMR.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{12}{12}\selectfont\strut}%
\psfrag{012}[bc][bc]{\matlabtextA Constrained $(1,49)M_\odot$}%
\psfrag{013}[tc][tc]{\matlabtextA SNR}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $0$}%
\psfrag{001}[ct][ct]{\matlabtextB $5$}%
\psfrag{002}[ct][ct]{\matlabtextB $10$}%
\psfrag{003}[ct][ct]{\matlabtextB $15$}%
%
%% </xtick>
%
%% <yscale>
%
\psfrag{004}[bc][bc]{\matlabtextB $\times10^{5}$}%
%
%% </yscale>
%
%% <ytick>
%
\psfrag{005}[rc][rc]{\matlabtextB $0$}%
\psfrag{006}[rc][rc]{\matlabtextB $0.5$}%
\psfrag{007}[rc][rc]{\matlabtextB $1$}%
\psfrag{008}[rc][rc]{\matlabtextB $1.5$}%
\psfrag{009}[rc][rc]{\matlabtextB $2$}%
\psfrag{010}[rc][rc]{\matlabtextB $2.5$}%
\psfrag{011}[rc][rc]{\matlabtextB $3$}%
%
%% </ytick>

==> Figures/commit.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{12}{12}\selectfont\strut}%
\psfrag{015}[bc][bc]{\matlabtextA Subsversion revision}%
\psfrag{016}[tc][tc]{\matlabtextA Days}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $0$}%
\psfrag{001}[ct][ct]{\matlabtextB $50$}%
\psfrag{002}[ct][ct]{\matlabtextB $100$}%
\psfrag{003}[ct][ct]{\matlabtextB $150$}%
\psfrag{004}[ct][ct]{\matlabtextB $200$}%
\psfrag{005}[ct][ct]{\matlabtextB $250$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{006}[rc][rc]{\matlabtextB $0$}%
\psfrag{007}[rc][rc]{\matlabtextB $100$}%
\psfrag{008}[rc][rc]{\matlabtextB $200$}%
\psfrag{009}[rc][rc]{\matlabtextB $300$}%
\psfrag{010}[rc][rc]{\matlabtextB $400$}%
\psfrag{011}[rc][rc]{\matlabtextB $500$}%
\psfrag{012}[rc][rc]{\matlabtextB $600$}%
\psfrag{013}[rc][rc]{\matlabtextB $700$}%
\psfrag{014}[rc][rc]{\matlabtextB $800$}%
%
%% </ytick>

==> Figures/commithist.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{12}{12}\selectfont\strut}%
\psfrag{015}[bc][bc]{\matlabtextA Subversion revision}%
\psfrag{016}[tc][tc]{\matlabtextA Days}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $0$}%
\psfrag{001}[ct][ct]{\matlabtextB $50$}%
\psfrag{002}[ct][ct]{\matlabtextB $100$}%
\psfrag{003}[ct][ct]{\matlabtextB $150$}%
\psfrag{004}[ct][ct]{\matlabtextB $200$}%
\psfrag{005}[ct][ct]{\matlabtextB $250$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{006}[rc][rc]{\matlabtextB $0$}%
\psfrag{007}[rc][rc]{\matlabtextB $100$}%
\psfrag{008}[rc][rc]{\matlabtextB $200$}%
\psfrag{009}[rc][rc]{\matlabtextB $300$}%
\psfrag{010}[rc][rc]{\matlabtextB $400$}%
\psfrag{011}[rc][rc]{\matlabtextB $500$}%
\psfrag{012}[rc][rc]{\matlabtextB $600$}%
\psfrag{013}[rc][rc]{\matlabtextB $700$}%
\psfrag{014}[rc][rc]{\matlabtextB $800$}%
%
%% </ytick>

==> Figures/cons2_snr1.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{12}{12}\selectfont\strut}%
\psfrag{019}[bc][bc]{\matlabtextA Recovered total mass /$M_\odot$}%
\psfrag{020}[tc][tc]{\matlabtextA Injected total mass /$M_\odot$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\fontsize{10}{10}\selectfont\strut}%
\psfrag{004}[ct][ct]{\matlabtextB $20$}%
\psfrag{005}[ct][ct]{\matlabtextB $40$}%
\psfrag{006}[ct][ct]{\matlabtextB $60$}%
\psfrag{007}[ct][ct]{\matlabtextB $80$}%
\psfrag{008}[ct][ct]{\matlabtextB $100$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{000}[lc][lc]{\matlabtextB $0$}%
\psfrag{001}[lc][lc]{\matlabtextB $5$}%
\psfrag{002}[lc][lc]{\matlabtextB $10$}%
\psfrag{003}[lc][lc]{\matlabtextB $15$}%
\psfrag{009}[rc][rc]{\matlabtextB $10$}%
\psfrag{010}[rc][rc]{\matlabtextB $20$}%
\psfrag{011}[rc][rc]{\matlabtextB $30$}%
\psfrag{012}[rc][rc]{\matlabtextB $40$}%
\psfrag{013}[rc][rc]{\matlabtextB $50$}%
\psfrag{014}[rc][rc]{\matlabtextB $60$}%
\psfrag{015}[rc][rc]{\matlabtextB $70$}%
\psfrag{016}[rc][rc]{\matlabtextB $80$}%
\psfrag{017}[rc][rc]{\matlabtextB $90$}%
\psfrag{018}[rc][rc]{\matlabtextB $100$}%
%
%% </ytick>

==> Figures/conschidist.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{12}{12}\selectfont\strut}%
\psfrag{012}[bc][bc]{\matlabtextA Constrained $(10,20)M_\odot$}%
\psfrag{013}[tc][tc]{\matlabtextA SNR}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $0$}%
\psfrag{001}[ct][ct]{\matlabtextB $5$}%
\psfrag{002}[ct][ct]{\matlabtextB $10$}%
\psfrag{003}[ct][ct]{\matlabtextB $15$}%
%
%% </xtick>
%
%% <yscale>
%
\psfrag{004}[bc][bc]{\matlabtextB $\times10^{5}$}%
%
%% </yscale>
%
%% <ytick>
%
\psfrag{005}[rc][rc]{\matlabtextB $0$}%
\psfrag{006}[rc][rc]{\matlabtextB $0.5$}%
\psfrag{007}[rc][rc]{\matlabtextB $1$}%
\psfrag{008}[rc][rc]{\matlabtextB $1.5$}%
\psfrag{009}[rc][rc]{\matlabtextB $2$}%
\psfrag{010}[rc][rc]{\matlabtextB $2.5$}%
\psfrag{011}[rc][rc]{\matlabtextB $3$}%
%
%% </ytick>

==> Figures/conschidistLMR.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{12}{12}\selectfont\strut}%
\psfrag{012}[bc][bc]{\matlabtextA Constrained $(1,49)M_\odot$}%
\psfrag{013}[tc][tc]{\matlabtextA SNR}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $0$}%
\psfrag{001}[ct][ct]{\matlabtextB $5$}%
\psfrag{002}[ct][ct]{\matlabtextB $10$}%
\psfrag{003}[ct][ct]{\matlabtextB $15$}%
%
%% </xtick>
%
%% <yscale>
%
\psfrag{004}[bc][bc]{\matlabtextB $\times10^{5}$}%
%
%% </yscale>
%
%% <ytick>
%
\psfrag{005}[rc][rc]{\matlabtextB $0$}%
\psfrag{006}[rc][rc]{\matlabtextB $0.5$}%
\psfrag{007}[rc][rc]{\matlabtextB $1$}%
\psfrag{008}[rc][rc]{\matlabtextB $1.5$}%
\psfrag{009}[rc][rc]{\matlabtextB $2$}%
\psfrag{010}[rc][rc]{\matlabtextB $2.5$}%
\psfrag{011}[rc][rc]{\matlabtextB $3$}%
%
%% </ytick>

==> Figures/conschidistLMR_new.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{12}{12}\selectfont\strut}%
\psfrag{009}[bc][bc]{\matlabtextA Constrained $(1,49)M_\odot$}%
\psfrag{010}[tc][tc]{\matlabtextA SNR}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $0$}%
\psfrag{001}[ct][ct]{\matlabtextB $5$}%
\psfrag{002}[ct][ct]{\matlabtextB $10$}%
\psfrag{003}[ct][ct]{\matlabtextB $15$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{004}[rc][rc]{\matlabtextB $0$}%
\psfrag{005}[rc][rc]{\matlabtextB $50$}%
\psfrag{006}[rc][rc]{\matlabtextB $100$}%
\psfrag{007}[rc][rc]{\matlabtextB $150$}%
\psfrag{008}[rc][rc]{\matlabtextB $200$}%
%
%% </ytick>

==> Figures/conschidist_new.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{12}{12}\selectfont\strut}%
\psfrag{015}[bc][bc]{\matlabtextA Constrained $(10,20)M_\odot$}%
\psfrag{016}[tc][tc]{\matlabtextA SNR}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $0$}%
\psfrag{001}[ct][ct]{\matlabtextB $5$}%
\psfrag{002}[ct][ct]{\matlabtextB $10$}%
\psfrag{003}[ct][ct]{\matlabtextB $15$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{004}[rc][rc]{\matlabtextB $0$}%
\psfrag{005}[rc][rc]{\matlabtextB $5$}%
\psfrag{006}[rc][rc]{\matlabtextB $10$}%
\psfrag{007}[rc][rc]{\matlabtextB $15$}%
\psfrag{008}[rc][rc]{\matlabtextB $20$}%
\psfrag{009}[rc][rc]{\matlabtextB $25$}%
\psfrag{010}[rc][rc]{\matlabtextB $30$}%
\psfrag{011}[rc][rc]{\matlabtextB $35$}%
\psfrag{012}[rc][rc]{\matlabtextB $40$}%
\psfrag{013}[rc][rc]{\matlabtextB $45$}%
\psfrag{014}[rc][rc]{\matlabtextB $50$}%
%
%% </ytick>

==> Figures/designpsd.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{12}{12}\selectfont\strut}%
\psfrag{011}[bc][bc]{\matlabtextA Strain amplitude spectrum /$1/\sqrt{\rm Hz}$}%
\psfrag{012}[tc][tc]{\matlabtextA Frequency /$\rm Hz$}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\bfseries\boldmath\selectfont\strut}%
\psfrag{009}[cl][cl]{\matlabtextB Shot Noise}%
\psfrag{010}[cl][cl]{\matlabtextB Thermal Noise}%
\psfrag{013}[cl][cl]{\matlabtextB Seismic Noise}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $10^{1}$}%
\psfrag{001}[ct][ct]{\matlabtextC $10^{2}$}%
\psfrag{002}[ct][ct]{\matlabtextC $10^{3}$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{003}[rc][rc]{\matlabtextC $10^{-23}$}%
\psfrag{004}[rc][rc]{\matlabtextC $10^{-22}$}%
\psfrag{005}[rc][rc]{\matlabtextC $10^{-21}$}%
\psfrag{006}[rc][rc]{\matlabtextC $10^{-20}$}%
\psfrag{007}[rc][rc]{\matlabtextC $10^{-19}$}%
\psfrag{008}[rc][rc]{\matlabtextC $10^{-18}$}%
%
%% </ytick>

==> Figures/eob.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{12}{12}\selectfont\strut}%
\psfrag{001}[tr][tr]{\matlabtextA $y$}%
\psfrag{002}[tl][tl]{\matlabtextA $x$}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{000}[bc][bc]{\matlabtextB Time}%
%
%% </text>


==> Figures/eobplung.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{12}{12}\selectfont\strut}%
\psfrag{001}[tr][tr]{\matlabtextA $y$}%
\psfrag{002}[tl][tl]{\matlabtextA $x$}%
%
\providecommand\matlabtextB{\fontsize{15}{15}\selectfont\strut}%
\psfrag{000}[bc][bc]{\matlabtextB Time}%
%
%% </text>

==> Figures/faithfulness.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{014}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{015}[bc][bc]{\matlabtextB Faithfulness}%
\psfrag{016}[tc][tc]{\matlabtextB Injected total mass /$\, M_\odot$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $20$}%
\psfrag{001}[ct][ct]{\matlabtextC $30$}%
\psfrag{002}[ct][ct]{\matlabtextC $40$}%
\psfrag{003}[ct][ct]{\matlabtextC $50$}%
\psfrag{004}[ct][ct]{\matlabtextC $60$}%
\psfrag{005}[ct][ct]{\matlabtextC $70$}%
\psfrag{006}[ct][ct]{\matlabtextC $80$}%
\psfrag{007}[ct][ct]{\matlabtextC $90$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{008}[rc][rc]{\matlabtextC $0$}%
\psfrag{009}[rc][rc]{\matlabtextC $0.2$}%
\psfrag{010}[rc][rc]{\matlabtextC $0.4$}%
\psfrag{011}[rc][rc]{\matlabtextC $0.6$}%
\psfrag{012}[rc][rc]{\matlabtextC $0.8$}%
\psfrag{013}[rc][rc]{\matlabtextC $1$}%
%
%% </ytick>

==> Figures/faithfulnesstt3.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{014}[cl][cl]{\matlabtextA RWF (TT3)}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{015}[bc][bc]{\matlabtextB Faithfulness}%
\psfrag{016}[tc][tc]{\matlabtextB Injected total mass /$\, M_\odot$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $20$}%
\psfrag{001}[ct][ct]{\matlabtextC $30$}%
\psfrag{002}[ct][ct]{\matlabtextC $40$}%
\psfrag{003}[ct][ct]{\matlabtextC $50$}%
\psfrag{004}[ct][ct]{\matlabtextC $60$}%
\psfrag{005}[ct][ct]{\matlabtextC $70$}%
\psfrag{006}[ct][ct]{\matlabtextC $80$}%
\psfrag{007}[ct][ct]{\matlabtextC $90$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{008}[rc][rc]{\matlabtextC $0$}%
\psfrag{009}[rc][rc]{\matlabtextC $0.2$}%
\psfrag{010}[rc][rc]{\matlabtextC $0.4$}%
\psfrag{011}[rc][rc]{\matlabtextC $0.6$}%
\psfrag{012}[rc][rc]{\matlabtextC $0.8$}%
\psfrag{013}[rc][rc]{\matlabtextC $1$}%
%
%% </ytick>

==> Figures/freqevolve.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{12}{12}\selectfont\strut}%
\psfrag{000}[bc][bc]{\matlabtextA $\omega_s(t)$}%
\psfrag{001}[tc][tc]{\matlabtextA Time}%
%
%% </text>

==> Figures/freqwindows2.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{008}[tc][tc]{\matlabtextA $\widetilde{w}_T(f;0.1)$}%
\psfrag{009}[bc][bc]{\matlabtextA $\widetilde{w}_T(f;0.01)$}%
\psfrag{010}[bc][bc]{\matlabtextA $\widetilde{w}_T(f;0.033)$}%
\psfrag{011}[bc][bc]{\matlabtextA $\widetilde{s}_T(f)$}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{007}[tc][tc]{\matlabtextB Frequency /Hz}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $10^{0}$}%
\psfrag{001}[ct][ct]{\matlabtextC $10^{1}$}%
\psfrag{002}[ct][ct]{\matlabtextC $10^{2}$}%
\psfrag{003}[ct][ct]{\matlabtextC $10^{3}$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{004}[rc][rc]{\matlabtextC $10^{-10}$}%
\psfrag{005}[rc][rc]{\matlabtextC $10^{-5}$}%
\psfrag{006}[rc][rc]{\matlabtextC $10^{0}$}%
%
%% </ytick>


==> Figures/ftermflso.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{12}{12}\selectfont\strut}%
\psfrag{022}[bc][bc]{\matlabtextA $m_2$}%
\psfrag{023}[tc][tc]{\matlabtextA $m_1$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\fontsize{10}{10}\selectfont\strut}%
\psfrag{006}[ct][ct]{\matlabtextB $5$}%
\psfrag{007}[ct][ct]{\matlabtextB $10$}%
\psfrag{008}[ct][ct]{\matlabtextB $15$}%
\psfrag{009}[ct][ct]{\matlabtextB $20$}%
\psfrag{010}[ct][ct]{\matlabtextB $25$}%
\psfrag{011}[ct][ct]{\matlabtextB $30$}%
\psfrag{012}[ct][ct]{\matlabtextB $35$}%
\psfrag{013}[ct][ct]{\matlabtextB $40$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{000}[lc][lc]{\matlabtextB $0.5$}%
\psfrag{001}[lc][lc]{\matlabtextB $0.6$}%
\psfrag{002}[lc][lc]{\matlabtextB $0.7$}%
\psfrag{003}[lc][lc]{\matlabtextB $0.8$}%
\psfrag{004}[lc][lc]{\matlabtextB $0.9$}%
\psfrag{005}[lc][lc]{\matlabtextB $1$}%
\psfrag{014}[rc][rc]{\matlabtextB $5$}%
\psfrag{015}[rc][rc]{\matlabtextB $10$}%
\psfrag{016}[rc][rc]{\matlabtextB $15$}%
\psfrag{017}[rc][rc]{\matlabtextB $20$}%
\psfrag{018}[rc][rc]{\matlabtextB $25$}%
\psfrag{019}[rc][rc]{\matlabtextB $30$}%
\psfrag{020}[rc][rc]{\matlabtextB $35$}%
\psfrag{021}[rc][rc]{\matlabtextB $40$}%
%
%% </ytick>

==> Figures/hist_first.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{012}[cl][cl]{\matlabtextA Tapered}%
\psfrag{013}[cl][cl]{\matlabtextA Untapered}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{014}[tc][tc]{\matlabtextB Total mass /$M_\odot$}%
\psfrag{015}[bc][bc]{\matlabtextB $\#$ First stage triggers ( $\times10^6$ )}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $20$}%
\psfrag{001}[ct][ct]{\matlabtextC $40$}%
\psfrag{002}[ct][ct]{\matlabtextC $60$}%
\psfrag{003}[ct][ct]{\matlabtextC $80$}%
\psfrag{004}[ct][ct]{\matlabtextC $100$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{005}[rc][rc]{\matlabtextC $1$}%
\psfrag{006}[rc][rc]{\matlabtextC $2$}%
\psfrag{007}[rc][rc]{\matlabtextC $3$}%
\psfrag{008}[rc][rc]{\matlabtextC $4$}%
\psfrag{009}[rc][rc]{\matlabtextC $5$}%
\psfrag{010}[rc][rc]{\matlabtextC $6$}%
\psfrag{011}[rc][rc]{\matlabtextC $7$}%
%
%% </ytick>

==> Figures/hist_second.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{010}[cl][cl]{\matlabtextA Tapered}%
\psfrag{011}[cl][cl]{\matlabtextA Untapered}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{012}[tc][tc]{\matlabtextB Total mass /$M_\odot$}%
\psfrag{013}[bc][bc]{\matlabtextB $\#$ Second stage triggers ( $\times10^3$ )}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $20$}%
\psfrag{001}[ct][ct]{\matlabtextC $40$}%
\psfrag{002}[ct][ct]{\matlabtextC $60$}%
\psfrag{003}[ct][ct]{\matlabtextC $80$}%
\psfrag{004}[ct][ct]{\matlabtextC $100$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{005}[rc][rc]{\matlabtextC $2$}%
\psfrag{006}[rc][rc]{\matlabtextC $4$}%
\psfrag{007}[rc][rc]{\matlabtextC $6$}%
\psfrag{008}[rc][rc]{\matlabtextC $8$}%
\psfrag{009}[rc][rc]{\matlabtextC $10$}%
%
%% </ytick>

==> Figures/hplusevolve.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{12}{12}\selectfont\strut}%
\psfrag{000}[bc][bc]{\matlabtextA $h_+(t)$}%
\psfrag{001}[tc][tc]{\matlabtextA Time}%
%
%% </text>

==> Figures/massreach.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{017}[cl][cl]{\matlabtextA RWF}%
\psfrag{018}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{019}[bc][bc]{\matlabtextB SNR}%
\psfrag{020}[tc][tc]{\matlabtextB Total mass /$M_\odot$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $30$}%
\psfrag{001}[ct][ct]{\matlabtextC $50$}%
\psfrag{002}[ct][ct]{\matlabtextC $70$}%
\psfrag{003}[ct][ct]{\matlabtextC $90$}%
\psfrag{004}[ct][ct]{\matlabtextC $110$}%
\psfrag{005}[ct][ct]{\matlabtextC $130$}%
\psfrag{006}[ct][ct]{\matlabtextC $150$}%
\psfrag{007}[ct][ct]{\matlabtextC $170$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{008}[rc][rc]{\matlabtextC $70$}%
\psfrag{009}[rc][rc]{\matlabtextC $80$}%
\psfrag{010}[rc][rc]{\matlabtextC $90$}%
\psfrag{011}[rc][rc]{\matlabtextC $100$}%
\psfrag{012}[rc][rc]{\matlabtextC $110$}%
\psfrag{013}[rc][rc]{\matlabtextC $120$}%
\psfrag{014}[rc][rc]{\matlabtextC $130$}%
\psfrag{015}[rc][rc]{\matlabtextC $140$}%
\psfrag{016}[rc][rc]{\matlabtextC $150$}%
%
%% </ytick>

==> Figures/maxh1h2.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{12}{12}\selectfont\strut}%
\psfrag{024}[bc][bc]{\matlabtextA $\left[\left<h_1,h_1\right>/\left<h_2,h_2\right>\right]_{max}$}%
\psfrag{025}[bc][bc]{\matlabtextA Total mass /$M_\odot$}%
\psfrag{026}[tc][tc]{\matlabtextA $\eta$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\fontsize{10}{10}\selectfont\strut}%
\psfrag{008}[ct][ct]{\matlabtextB $0.222$}%
\psfrag{009}[ct][ct]{\matlabtextB $0.160$}%
\psfrag{010}[ct][ct]{\matlabtextB $0.122$}%
\psfrag{011}[ct][ct]{\matlabtextB $0.099$}%
\psfrag{012}[ct][ct]{\matlabtextB $0.083$}%
\psfrag{013}[ct][ct]{\matlabtextB $0.071$}%
\psfrag{014}[ct][ct]{\matlabtextB $0.062$}%
\psfrag{015}[ct][ct]{\matlabtextB $0.055$}%
\psfrag{016}[ct][ct]{\matlabtextB $0.050$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{000}[lc][lc]{\matlabtextB $0$}%
\psfrag{001}[lc][lc]{\matlabtextB $0.002$}%
\psfrag{002}[lc][lc]{\matlabtextB $0.004$}%
\psfrag{003}[lc][lc]{\matlabtextB $0.006$}%
\psfrag{004}[lc][lc]{\matlabtextB $0.008$}%
\psfrag{005}[lc][lc]{\matlabtextB $0.01$}%
\psfrag{006}[lc][lc]{\matlabtextB $0.012$}%
\psfrag{007}[lc][lc]{\matlabtextB $0.014$}%
\psfrag{017}[rc][rc]{\matlabtextB $20$}%
\psfrag{018}[rc][rc]{\matlabtextB $25$}%
\psfrag{019}[rc][rc]{\matlabtextB $30$}%
\psfrag{020}[rc][rc]{\matlabtextB $35$}%
\psfrag{021}[rc][rc]{\matlabtextB $40$}%
\psfrag{022}[rc][rc]{\matlabtextB $45$}%
\psfrag{023}[rc][rc]{\matlabtextB $50$}%
%
%% </ytick>


==> Figures/maxh1h2fit.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{12}{12}\selectfont\strut}%
\psfrag{024}[bc][bc]{\matlabtextA $\left[\left<h_1,h_1\right>/\left<h_2,h_2\right>\right]_{max}$}%
\psfrag{025}[bc][bc]{\matlabtextA Total mass /$M_\odot$}%
\psfrag{026}[tc][tc]{\matlabtextA $\eta$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\fontsize{10}{10}\selectfont\strut}%
\psfrag{008}[ct][ct]{\matlabtextB $0.222$}%
\psfrag{009}[ct][ct]{\matlabtextB $0.160$}%
\psfrag{010}[ct][ct]{\matlabtextB $0.122$}%
\psfrag{011}[ct][ct]{\matlabtextB $0.099$}%
\psfrag{012}[ct][ct]{\matlabtextB $0.083$}%
\psfrag{013}[ct][ct]{\matlabtextB $0.071$}%
\psfrag{014}[ct][ct]{\matlabtextB $0.062$}%
\psfrag{015}[ct][ct]{\matlabtextB $0.055$}%
\psfrag{016}[ct][ct]{\matlabtextB $0.050$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{000}[lc][lc]{\matlabtextB $0$}%
\psfrag{001}[lc][lc]{\matlabtextB $0.002$}%
\psfrag{002}[lc][lc]{\matlabtextB $0.004$}%
\psfrag{003}[lc][lc]{\matlabtextB $0.006$}%
\psfrag{004}[lc][lc]{\matlabtextB $0.008$}%
\psfrag{005}[lc][lc]{\matlabtextB $0.01$}%
\psfrag{006}[lc][lc]{\matlabtextB $0.012$}%
\psfrag{007}[lc][lc]{\matlabtextB $0.014$}%
\psfrag{017}[rc][rc]{\matlabtextB $20$}%
\psfrag{018}[rc][rc]{\matlabtextB $25$}%
\psfrag{019}[rc][rc]{\matlabtextB $30$}%
\psfrag{020}[rc][rc]{\matlabtextB $35$}%
\psfrag{021}[rc][rc]{\matlabtextB $40$}%
\psfrag{022}[rc][rc]{\matlabtextB $45$}%
\psfrag{023}[rc][rc]{\matlabtextB $50$}%
%
%% </ytick>


==> Figures/maxh3h2.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{12}{12}\selectfont\strut}%
\psfrag{024}[bc][bc]{\matlabtextA $\left[\left<h_3,h_3\right>/\left<h_2,h_2\right>\right]_{max}$}%
\psfrag{025}[bc][bc]{\matlabtextA Total mass /$M_\odot$}%
\psfrag{026}[tc][tc]{\matlabtextA $\eta$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\fontsize{10}{10}\selectfont\strut}%
\psfrag{006}[ct][ct]{\matlabtextB $0.222$}%
\psfrag{007}[ct][ct]{\matlabtextB $0.160$}%
\psfrag{008}[ct][ct]{\matlabtextB $0.122$}%
\psfrag{009}[ct][ct]{\matlabtextB $0.099$}%
\psfrag{010}[ct][ct]{\matlabtextB $0.083$}%
\psfrag{011}[ct][ct]{\matlabtextB $0.071$}%
\psfrag{012}[ct][ct]{\matlabtextB $0.062$}%
\psfrag{013}[ct][ct]{\matlabtextB $0.055$}%
\psfrag{014}[ct][ct]{\matlabtextB $0.050$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{000}[lc][lc]{\matlabtextB $0$}%
\psfrag{001}[lc][lc]{\matlabtextB $0.1$}%
\psfrag{002}[lc][lc]{\matlabtextB $0.2$}%
\psfrag{003}[lc][lc]{\matlabtextB $0.3$}%
\psfrag{004}[lc][lc]{\matlabtextB $0.4$}%
\psfrag{005}[lc][lc]{\matlabtextB $0.5$}%
\psfrag{015}[rc][rc]{\matlabtextB $20$}%
\psfrag{016}[rc][rc]{\matlabtextB $30$}%
\psfrag{017}[rc][rc]{\matlabtextB $40$}%
\psfrag{018}[rc][rc]{\matlabtextB $50$}%
\psfrag{019}[rc][rc]{\matlabtextB $60$}%
\psfrag{020}[rc][rc]{\matlabtextB $70$}%
\psfrag{021}[rc][rc]{\matlabtextB $80$}%
\psfrag{022}[rc][rc]{\matlabtextB $90$}%
\psfrag{023}[rc][rc]{\matlabtextB $100$}%
%
%% </ytick>


==> Figures/maxh3h2fit.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{12}{12}\selectfont\strut}%
\psfrag{020}[bc][bc]{\matlabtextA $\left[\left<h_3,h_3\right>/\left<h_2,h_2\right>\right]_{max}$}%
\psfrag{021}[bc][bc]{\matlabtextA Total mass /$M_\odot$}%
\psfrag{022}[tc][tc]{\matlabtextA $\eta$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\fontsize{10}{10}\selectfont\strut}%
\psfrag{006}[ct][ct]{\matlabtextB $0.222$}%
\psfrag{007}[ct][ct]{\matlabtextB $0.160$}%
\psfrag{008}[ct][ct]{\matlabtextB $0.122$}%
\psfrag{009}[ct][ct]{\matlabtextB $0.099$}%
\psfrag{010}[ct][ct]{\matlabtextB $0.083$}%
\psfrag{011}[ct][ct]{\matlabtextB $0.071$}%
\psfrag{012}[ct][ct]{\matlabtextB $0.062$}%
\psfrag{013}[ct][ct]{\matlabtextB $0.055$}%
\psfrag{014}[ct][ct]{\matlabtextB $0.050$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{000}[lc][lc]{\matlabtextB $0$}%
\psfrag{001}[lc][lc]{\matlabtextB $0.1$}%
\psfrag{002}[lc][lc]{\matlabtextB $0.2$}%
\psfrag{003}[lc][lc]{\matlabtextB $0.3$}%
\psfrag{004}[lc][lc]{\matlabtextB $0.4$}%
\psfrag{005}[lc][lc]{\matlabtextB $0.5$}%
\psfrag{015}[rc][rc]{\matlabtextB $20$}%
\psfrag{016}[rc][rc]{\matlabtextB $40$}%
\psfrag{017}[rc][rc]{\matlabtextB $60$}%
\psfrag{018}[rc][rc]{\matlabtextB $80$}%
\psfrag{019}[rc][rc]{\matlabtextB $100$}%
%
%% </ytick>


==> Figures/month1bns.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{017}[cl][cl]{\matlabtextA Combined}%
\psfrag{018}[cl][cl]{\matlabtextA H1H2L1}%
\psfrag{019}[cl][cl]{\matlabtextA H1L1}%
\psfrag{020}[cl][cl]{\matlabtextA H2L1}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{021}[bc][bc]{\matlabtextB BNS (month 1 only)}%
\psfrag{022}[bc][bc]{\matlabtextB Unnormalised probability}%
\psfrag{023}[tc][tc]{\matlabtextB Rate /$\, {\rm yr}^{-1}{\rm L}^{-1}_{10}$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $0$}%
\psfrag{001}[ct][ct]{\matlabtextC $0.2$}%
\psfrag{002}[ct][ct]{\matlabtextC $0.4$}%
\psfrag{003}[ct][ct]{\matlabtextC $0.6$}%
\psfrag{004}[ct][ct]{\matlabtextC $0.8$}%
\psfrag{005}[ct][ct]{\matlabtextC $1$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{006}[rc][rc]{\matlabtextC $0$}%
\psfrag{007}[rc][rc]{\matlabtextC $0.1$}%
\psfrag{008}[rc][rc]{\matlabtextC $0.2$}%
\psfrag{009}[rc][rc]{\matlabtextC $0.3$}%
\psfrag{010}[rc][rc]{\matlabtextC $0.4$}%
\psfrag{011}[rc][rc]{\matlabtextC $0.5$}%
\psfrag{012}[rc][rc]{\matlabtextC $0.6$}%
\psfrag{013}[rc][rc]{\matlabtextC $0.7$}%
\psfrag{014}[rc][rc]{\matlabtextC $0.8$}%
\psfrag{015}[rc][rc]{\matlabtextC $0.9$}%
\psfrag{016}[rc][rc]{\matlabtextC $1$}%
%
%% </ytick>

==> Figures/noconschidist.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{12}{12}\selectfont\strut}%
\psfrag{015}[bc][bc]{\matlabtextA Unconstrained $(10,20)M_\odot$}%
\psfrag{016}[tc][tc]{\matlabtextA SNR}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $0$}%
\psfrag{001}[ct][ct]{\matlabtextB $5$}%
\psfrag{002}[ct][ct]{\matlabtextB $10$}%
\psfrag{003}[ct][ct]{\matlabtextB $15$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{004}[rc][rc]{\matlabtextB $0$}%
\psfrag{005}[rc][rc]{\matlabtextB $1000$}%
\psfrag{006}[rc][rc]{\matlabtextB $2000$}%
\psfrag{007}[rc][rc]{\matlabtextB $3000$}%
\psfrag{008}[rc][rc]{\matlabtextB $4000$}%
\psfrag{009}[rc][rc]{\matlabtextB $5000$}%
\psfrag{010}[rc][rc]{\matlabtextB $6000$}%
\psfrag{011}[rc][rc]{\matlabtextB $7000$}%
\psfrag{012}[rc][rc]{\matlabtextB $8000$}%
\psfrag{013}[rc][rc]{\matlabtextB $9000$}%
\psfrag{014}[rc][rc]{\matlabtextB $10000$}%
%
%% </ytick>

==> Figures/noconschidistLMR.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{12}{12}\selectfont\strut}%
\psfrag{015}[bc][bc]{\matlabtextA Unconstrained $(1,49)M_\odot$}%
\psfrag{016}[tc][tc]{\matlabtextA SNR}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $0$}%
\psfrag{001}[ct][ct]{\matlabtextB $5$}%
\psfrag{002}[ct][ct]{\matlabtextB $10$}%
\psfrag{003}[ct][ct]{\matlabtextB $15$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{004}[rc][rc]{\matlabtextB $0$}%
\psfrag{005}[rc][rc]{\matlabtextB $1000$}%
\psfrag{006}[rc][rc]{\matlabtextB $2000$}%
\psfrag{007}[rc][rc]{\matlabtextB $3000$}%
\psfrag{008}[rc][rc]{\matlabtextB $4000$}%
\psfrag{009}[rc][rc]{\matlabtextB $5000$}%
\psfrag{010}[rc][rc]{\matlabtextB $6000$}%
\psfrag{011}[rc][rc]{\matlabtextB $7000$}%
\psfrag{012}[rc][rc]{\matlabtextB $8000$}%
\psfrag{013}[rc][rc]{\matlabtextB $9000$}%
\psfrag{014}[rc][rc]{\matlabtextB $10000$}%
%
%% </ytick>

==> Figures/normcheck.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{12}{12}\selectfont\strut}%
\psfrag{017}[bc][bc]{\matlabtextA $\frac{\sigma_\perp + \sigma_c}{\sigma_\perp}$}%
\psfrag{018}[tc][tc]{\matlabtextA Total mass /$M_\odot$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $0$}%
\psfrag{001}[ct][ct]{\matlabtextB $20$}%
\psfrag{002}[ct][ct]{\matlabtextB $40$}%
\psfrag{003}[ct][ct]{\matlabtextB $60$}%
\psfrag{004}[ct][ct]{\matlabtextB $80$}%
\psfrag{005}[ct][ct]{\matlabtextB $100$}%
\psfrag{006}[ct][ct]{\matlabtextB $120$}%
\psfrag{007}[ct][ct]{\matlabtextB $140$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{008}[rc][rc]{\matlabtextB $0.8$}%
\psfrag{009}[rc][rc]{\matlabtextB $0.85$}%
\psfrag{010}[rc][rc]{\matlabtextB $0.9$}%
\psfrag{011}[rc][rc]{\matlabtextB $0.95$}%
\psfrag{012}[rc][rc]{\matlabtextB $1$}%
\psfrag{013}[rc][rc]{\matlabtextB $1.05$}%
\psfrag{014}[rc][rc]{\matlabtextB $1.1$}%
\psfrag{015}[rc][rc]{\matlabtextB $1.15$}%
\psfrag{016}[rc][rc]{\matlabtextB $1.2$}%
%
%% </ytick>

==> Figures/overlap.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{014}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{015}[bc][bc]{\matlabtextB Overlap}%
\psfrag{016}[tc][tc]{\matlabtextB Injected total mass /$\, M_\odot$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $20$}%
\psfrag{001}[ct][ct]{\matlabtextC $30$}%
\psfrag{002}[ct][ct]{\matlabtextC $40$}%
\psfrag{003}[ct][ct]{\matlabtextC $50$}%
\psfrag{004}[ct][ct]{\matlabtextC $60$}%
\psfrag{005}[ct][ct]{\matlabtextC $70$}%
\psfrag{006}[ct][ct]{\matlabtextC $80$}%
\psfrag{007}[ct][ct]{\matlabtextC $90$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{008}[rc][rc]{\matlabtextC $0$}%
\psfrag{009}[rc][rc]{\matlabtextC $0.2$}%
\psfrag{010}[rc][rc]{\matlabtextC $0.4$}%
\psfrag{011}[rc][rc]{\matlabtextC $0.6$}%
\psfrag{012}[rc][rc]{\matlabtextC $0.8$}%
\psfrag{013}[rc][rc]{\matlabtextC $1$}%
%
%% </ytick>

==> Figures/ovrlptt3.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{014}[cl][cl]{\matlabtextA RWF (TT3)}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{015}[bc][bc]{\matlabtextB Overlap}%
\psfrag{016}[tc][tc]{\matlabtextB Injected total mass /$\, M_\odot$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $20$}%
\psfrag{001}[ct][ct]{\matlabtextC $30$}%
\psfrag{002}[ct][ct]{\matlabtextC $40$}%
\psfrag{003}[ct][ct]{\matlabtextC $50$}%
\psfrag{004}[ct][ct]{\matlabtextC $60$}%
\psfrag{005}[ct][ct]{\matlabtextC $70$}%
\psfrag{006}[ct][ct]{\matlabtextC $80$}%
\psfrag{007}[ct][ct]{\matlabtextC $90$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{008}[rc][rc]{\matlabtextC $0$}%
\psfrag{009}[rc][rc]{\matlabtextC $0.2$}%
\psfrag{010}[rc][rc]{\matlabtextC $0.4$}%
\psfrag{011}[rc][rc]{\matlabtextC $0.6$}%
\psfrag{012}[rc][rc]{\matlabtextC $0.8$}%
\psfrag{013}[rc][rc]{\matlabtextC $1$}%
%
%% </ytick>

==> Figures/pemonte100922/snr16_mt30_eta0-05_CHIRP.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{007}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{008}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{009}[bc][bc]{\matlabtextB Signal: $\rho=16$, $M_T=30M_\odot$, $\eta=0.05$}%
\psfrag{010}[bc][bc]{\matlabtextB $\#$}%
\psfrag{011}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 5$}%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $5$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{003}[rc][rc]{\matlabtextC $0$}%
\psfrag{004}[rc][rc]{\matlabtextC $200$}%
\psfrag{005}[rc][rc]{\matlabtextC $400$}%
\psfrag{006}[rc][rc]{\matlabtextC $600$}%
%
%% </ytick>

==> Figures/pemonte100922/snr16_mt30_eta0-05_CHIRPsmall.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{007}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{008}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{009}[bc][bc]{\matlabtextB Signal: $\rho=16$, $M_T=30M_\odot$, $\eta=0.05$}%
\psfrag{010}[bc][bc]{\matlabtextB $\#$}%
\psfrag{011}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 5$}%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $5$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{003}[rc][rc]{\matlabtextC $0$}%
\psfrag{004}[rc][rc]{\matlabtextC $200$}%
\psfrag{005}[rc][rc]{\matlabtextC $400$}%
\psfrag{006}[rc][rc]{\matlabtextC $600$}%
%
%% </ytick>

==> Figures/pemonte100922/snr16_mt30_eta0-075_CHIRP.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{010}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{011}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{012}[bc][bc]{\matlabtextB Signal: $\rho=16$, $M_T=30M_\odot$, $\eta=0.075$}%
\psfrag{013}[bc][bc]{\matlabtextB $\#$}%
\psfrag{014}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 4$}%
\psfrag{001}[ct][ct]{\matlabtextC $\matlabfragNegXTick 2$}%
\psfrag{002}[ct][ct]{\matlabtextC $0$}%
\psfrag{003}[ct][ct]{\matlabtextC $2$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{004}[rc][rc]{\matlabtextC $0$}%
\psfrag{005}[rc][rc]{\matlabtextC $100$}%
\psfrag{006}[rc][rc]{\matlabtextC $200$}%
\psfrag{007}[rc][rc]{\matlabtextC $300$}%
\psfrag{008}[rc][rc]{\matlabtextC $400$}%
\psfrag{009}[rc][rc]{\matlabtextC $500$}%
%
%% </ytick>

==> Figures/pemonte100922/snr16_mt30_eta0-075_CHIRPsmall.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{010}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{011}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{012}[bc][bc]{\matlabtextB Signal: $\rho=16$, $M_T=30M_\odot$, $\eta=0.075$}%
\psfrag{013}[bc][bc]{\matlabtextB $\#$}%
\psfrag{014}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 4$}%
\psfrag{001}[ct][ct]{\matlabtextC $\matlabfragNegXTick 2$}%
\psfrag{002}[ct][ct]{\matlabtextC $0$}%
\psfrag{003}[ct][ct]{\matlabtextC $2$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{004}[rc][rc]{\matlabtextC $0$}%
\psfrag{005}[rc][rc]{\matlabtextC $100$}%
\psfrag{006}[rc][rc]{\matlabtextC $200$}%
\psfrag{007}[rc][rc]{\matlabtextC $300$}%
\psfrag{008}[rc][rc]{\matlabtextC $400$}%
\psfrag{009}[rc][rc]{\matlabtextC $500$}%
%
%% </ytick>

==> Figures/pemonte100922/snr16_mt30_eta0-111_CHIRP.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{008}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{009}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{010}[bc][bc]{\matlabtextB Signal: $\rho=16$, $M_T=30M_\odot$, $\eta=0.111$}%
\psfrag{011}[bc][bc]{\matlabtextB $\#$}%
\psfrag{012}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 4$}%
\psfrag{001}[ct][ct]{\matlabtextC $\matlabfragNegXTick 2$}%
\psfrag{002}[ct][ct]{\matlabtextC $0$}%
\psfrag{003}[ct][ct]{\matlabtextC $2$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{004}[rc][rc]{\matlabtextC $0$}%
\psfrag{005}[rc][rc]{\matlabtextC $200$}%
\psfrag{006}[rc][rc]{\matlabtextC $400$}%
\psfrag{007}[rc][rc]{\matlabtextC $600$}%
%
%% </ytick>

==> Figures/pemonte100922/snr16_mt30_eta0-111_CHIRPsmall.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{008}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{009}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{010}[bc][bc]{\matlabtextB Signal: $\rho=16$, $M_T=30M_\odot$, $\eta=0.111$}%
\psfrag{011}[bc][bc]{\matlabtextB $\#$}%
\psfrag{012}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 4$}%
\psfrag{001}[ct][ct]{\matlabtextC $\matlabfragNegXTick 2$}%
\psfrag{002}[ct][ct]{\matlabtextC $0$}%
\psfrag{003}[ct][ct]{\matlabtextC $2$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{004}[rc][rc]{\matlabtextC $0$}%
\psfrag{005}[rc][rc]{\matlabtextC $200$}%
\psfrag{006}[rc][rc]{\matlabtextC $400$}%
\psfrag{007}[rc][rc]{\matlabtextC $600$}%
%
%% </ytick>

==> Figures/pemonte100922/snr16_mt30_eta0-167_CHIRP.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{009}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{010}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{011}[bc][bc]{\matlabtextB Signal: $\rho=16$, $M_T=30M_\odot$, $\eta=0.167$}%
\psfrag{012}[bc][bc]{\matlabtextB $\#$}%
\psfrag{013}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 5$}%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $5$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{003}[rc][rc]{\matlabtextC $0$}%
\psfrag{004}[rc][rc]{\matlabtextC $100$}%
\psfrag{005}[rc][rc]{\matlabtextC $200$}%
\psfrag{006}[rc][rc]{\matlabtextC $300$}%
\psfrag{007}[rc][rc]{\matlabtextC $400$}%
\psfrag{008}[rc][rc]{\matlabtextC $500$}%
%
%% </ytick>

==> Figures/pemonte100922/snr16_mt30_eta0-167_CHIRPsmall.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{009}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{010}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{011}[bc][bc]{\matlabtextB Signal: $\rho=16$, $M_T=30M_\odot$, $\eta=0.167$}%
\psfrag{012}[bc][bc]{\matlabtextB $\#$}%
\psfrag{013}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 5$}%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $5$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{003}[rc][rc]{\matlabtextC $0$}%
\psfrag{004}[rc][rc]{\matlabtextC $100$}%
\psfrag{005}[rc][rc]{\matlabtextC $200$}%
\psfrag{006}[rc][rc]{\matlabtextC $300$}%
\psfrag{007}[rc][rc]{\matlabtextC $400$}%
\psfrag{008}[rc][rc]{\matlabtextC $500$}%
%
%% </ytick>

==> Figures/pemonte100922/snr16_mt30_eta0-25_CHIRP.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{009}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{010}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{011}[bc][bc]{\matlabtextB Signal: $\rho=16$, $M_T=30M_\odot$, $\eta=0.25$}%
\psfrag{012}[bc][bc]{\matlabtextB $\#$}%
\psfrag{013}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 10$}%
\psfrag{001}[ct][ct]{\matlabtextC $\matlabfragNegXTick 5$}%
\psfrag{002}[ct][ct]{\matlabtextC $0$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{003}[rc][rc]{\matlabtextC $0$}%
\psfrag{004}[rc][rc]{\matlabtextC $200$}%
\psfrag{005}[rc][rc]{\matlabtextC $400$}%
\psfrag{006}[rc][rc]{\matlabtextC $600$}%
\psfrag{007}[rc][rc]{\matlabtextC $800$}%
\psfrag{008}[rc][rc]{\matlabtextC $1000$}%
%
%% </ytick>

==> Figures/pemonte100922/snr16_mt30_eta0-25_CHIRPsmall.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{009}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{010}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{011}[bc][bc]{\matlabtextB Signal: $\rho=16$, $M_T=30M_\odot$, $\eta=0.25$}%
\psfrag{012}[bc][bc]{\matlabtextB $\#$}%
\psfrag{013}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 10$}%
\psfrag{001}[ct][ct]{\matlabtextC $\matlabfragNegXTick 5$}%
\psfrag{002}[ct][ct]{\matlabtextC $0$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{003}[rc][rc]{\matlabtextC $0$}%
\psfrag{004}[rc][rc]{\matlabtextC $200$}%
\psfrag{005}[rc][rc]{\matlabtextC $400$}%
\psfrag{006}[rc][rc]{\matlabtextC $600$}%
\psfrag{007}[rc][rc]{\matlabtextC $800$}%
\psfrag{008}[rc][rc]{\matlabtextC $1000$}%
%
%% </ytick>

==> Figures/pemonte100922/snr16_mt45_eta0-05_CHIRP.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{006}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{007}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{008}[bc][bc]{\matlabtextB Signal: $\rho=16$, $M_T=45M_\odot$, $\eta=0.05$}%
\psfrag{009}[bc][bc]{\matlabtextB $\#$}%
\psfrag{010}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 40$}%
\psfrag{001}[ct][ct]{\matlabtextC $\matlabfragNegXTick 20$}%
\psfrag{002}[ct][ct]{\matlabtextC $0$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{003}[rc][rc]{\matlabtextC $0$}%
\psfrag{004}[rc][rc]{\matlabtextC $500$}%
\psfrag{005}[rc][rc]{\matlabtextC $1000$}%
%
%% </ytick>

==> Figures/pemonte100922/snr16_mt45_eta0-05_CHIRPsmall.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{006}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{007}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{008}[bc][bc]{\matlabtextB Signal: $\rho=16$, $M_T=45M_\odot$, $\eta=0.05$}%
\psfrag{009}[bc][bc]{\matlabtextB $\#$}%
\psfrag{010}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 40$}%
\psfrag{001}[ct][ct]{\matlabtextC $\matlabfragNegXTick 20$}%
\psfrag{002}[ct][ct]{\matlabtextC $0$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{003}[rc][rc]{\matlabtextC $0$}%
\psfrag{004}[rc][rc]{\matlabtextC $500$}%
\psfrag{005}[rc][rc]{\matlabtextC $1000$}%
%
%% </ytick>

==> Figures/pemonte100922/snr16_mt45_eta0-075_CHIRP.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{010}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{011}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{012}[bc][bc]{\matlabtextB Signal: $\rho=16$, $M_T=45M_\odot$, $\eta=0.075$}%
\psfrag{013}[bc][bc]{\matlabtextB $\#$}%
\psfrag{014}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 40$}%
\psfrag{001}[ct][ct]{\matlabtextC $\matlabfragNegXTick 20$}%
\psfrag{002}[ct][ct]{\matlabtextC $0$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{003}[rc][rc]{\matlabtextC $0$}%
\psfrag{004}[rc][rc]{\matlabtextC $200$}%
\psfrag{005}[rc][rc]{\matlabtextC $400$}%
\psfrag{006}[rc][rc]{\matlabtextC $600$}%
\psfrag{007}[rc][rc]{\matlabtextC $800$}%
\psfrag{008}[rc][rc]{\matlabtextC $1000$}%
\psfrag{009}[rc][rc]{\matlabtextC $1200$}%
%
%% </ytick>

==> Figures/pemonte100922/snr16_mt45_eta0-075_CHIRPsmall.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{010}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{011}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{012}[bc][bc]{\matlabtextB Signal: $\rho=16$, $M_T=45M_\odot$, $\eta=0.075$}%
\psfrag{013}[bc][bc]{\matlabtextB $\#$}%
\psfrag{014}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 40$}%
\psfrag{001}[ct][ct]{\matlabtextC $\matlabfragNegXTick 20$}%
\psfrag{002}[ct][ct]{\matlabtextC $0$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{003}[rc][rc]{\matlabtextC $0$}%
\psfrag{004}[rc][rc]{\matlabtextC $200$}%
\psfrag{005}[rc][rc]{\matlabtextC $400$}%
\psfrag{006}[rc][rc]{\matlabtextC $600$}%
\psfrag{007}[rc][rc]{\matlabtextC $800$}%
\psfrag{008}[rc][rc]{\matlabtextC $1000$}%
\psfrag{009}[rc][rc]{\matlabtextC $1200$}%
%
%% </ytick>

==> Figures/pemonte100922/snr16_mt45_eta0-111_CHIRP.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{011}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{012}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{013}[bc][bc]{\matlabtextB Signal: $\rho=16$, $M_T=45M_\odot$, $\eta=0.111$}%
\psfrag{014}[bc][bc]{\matlabtextB $\#$}%
\psfrag{015}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 10$}%
\psfrag{001}[ct][ct]{\matlabtextC $\matlabfragNegXTick 5$}%
\psfrag{002}[ct][ct]{\matlabtextC $0$}%
\psfrag{003}[ct][ct]{\matlabtextC $5$}%
\psfrag{004}[ct][ct]{\matlabtextC $10$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{005}[rc][rc]{\matlabtextC $0$}%
\psfrag{006}[rc][rc]{\matlabtextC $100$}%
\psfrag{007}[rc][rc]{\matlabtextC $200$}%
\psfrag{008}[rc][rc]{\matlabtextC $300$}%
\psfrag{009}[rc][rc]{\matlabtextC $400$}%
\psfrag{010}[rc][rc]{\matlabtextC $500$}%
%
%% </ytick>

==> Figures/pemonte100922/snr16_mt45_eta0-111_CHIRPsmall.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{011}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{012}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{013}[bc][bc]{\matlabtextB Signal: $\rho=16$, $M_T=45M_\odot$, $\eta=0.111$}%
\psfrag{014}[bc][bc]{\matlabtextB $\#$}%
\psfrag{015}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 10$}%
\psfrag{001}[ct][ct]{\matlabtextC $\matlabfragNegXTick 5$}%
\psfrag{002}[ct][ct]{\matlabtextC $0$}%
\psfrag{003}[ct][ct]{\matlabtextC $5$}%
\psfrag{004}[ct][ct]{\matlabtextC $10$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{005}[rc][rc]{\matlabtextC $0$}%
\psfrag{006}[rc][rc]{\matlabtextC $100$}%
\psfrag{007}[rc][rc]{\matlabtextC $200$}%
\psfrag{008}[rc][rc]{\matlabtextC $300$}%
\psfrag{009}[rc][rc]{\matlabtextC $400$}%
\psfrag{010}[rc][rc]{\matlabtextC $500$}%
%
%% </ytick>

==> Figures/pemonte100922/snr16_mt45_eta0-167_CHIRP.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{010}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{011}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{012}[bc][bc]{\matlabtextB Signal: $\rho=16$, $M_T=45M_\odot$, $\eta=0.167$}%
\psfrag{013}[bc][bc]{\matlabtextB $\#$}%
\psfrag{014}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 10$}%
\psfrag{001}[ct][ct]{\matlabtextC $\matlabfragNegXTick 5$}%
\psfrag{002}[ct][ct]{\matlabtextC $0$}%
\psfrag{003}[ct][ct]{\matlabtextC $5$}%
\psfrag{004}[ct][ct]{\matlabtextC $10$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{005}[rc][rc]{\matlabtextC $0$}%
\psfrag{006}[rc][rc]{\matlabtextC $100$}%
\psfrag{007}[rc][rc]{\matlabtextC $200$}%
\psfrag{008}[rc][rc]{\matlabtextC $300$}%
\psfrag{009}[rc][rc]{\matlabtextC $400$}%
%
%% </ytick>

==> Figures/pemonte100922/snr16_mt45_eta0-167_CHIRPsmall.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{010}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{011}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{012}[bc][bc]{\matlabtextB Signal: $\rho=16$, $M_T=45M_\odot$, $\eta=0.167$}%
\psfrag{013}[bc][bc]{\matlabtextB $\#$}%
\psfrag{014}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 10$}%
\psfrag{001}[ct][ct]{\matlabtextC $\matlabfragNegXTick 5$}%
\psfrag{002}[ct][ct]{\matlabtextC $0$}%
\psfrag{003}[ct][ct]{\matlabtextC $5$}%
\psfrag{004}[ct][ct]{\matlabtextC $10$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{005}[rc][rc]{\matlabtextC $0$}%
\psfrag{006}[rc][rc]{\matlabtextC $100$}%
\psfrag{007}[rc][rc]{\matlabtextC $200$}%
\psfrag{008}[rc][rc]{\matlabtextC $300$}%
\psfrag{009}[rc][rc]{\matlabtextC $400$}%
%
%% </ytick>

==> Figures/pemonte100922/snr16_mt45_eta0-25_CHIRP.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{010}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{011}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{012}[bc][bc]{\matlabtextB Signal: $\rho=16$, $M_T=45M_\odot$, $\eta=0.25$}%
\psfrag{013}[bc][bc]{\matlabtextB $\#$}%
\psfrag{014}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 15$}%
\psfrag{001}[ct][ct]{\matlabtextC $\matlabfragNegXTick 10$}%
\psfrag{002}[ct][ct]{\matlabtextC $\matlabfragNegXTick 5$}%
\psfrag{003}[ct][ct]{\matlabtextC $0$}%
\psfrag{004}[ct][ct]{\matlabtextC $5$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{005}[rc][rc]{\matlabtextC $0$}%
\psfrag{006}[rc][rc]{\matlabtextC $200$}%
\psfrag{007}[rc][rc]{\matlabtextC $400$}%
\psfrag{008}[rc][rc]{\matlabtextC $600$}%
\psfrag{009}[rc][rc]{\matlabtextC $800$}%
%
%% </ytick>

==> Figures/pemonte100922/snr16_mt45_eta0-25_CHIRPsmall.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{010}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{011}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{012}[bc][bc]{\matlabtextB Signal: $\rho=16$, $M_T=45M_\odot$, $\eta=0.25$}%
\psfrag{013}[bc][bc]{\matlabtextB $\#$}%
\psfrag{014}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 15$}%
\psfrag{001}[ct][ct]{\matlabtextC $\matlabfragNegXTick 10$}%
\psfrag{002}[ct][ct]{\matlabtextC $\matlabfragNegXTick 5$}%
\psfrag{003}[ct][ct]{\matlabtextC $0$}%
\psfrag{004}[ct][ct]{\matlabtextC $5$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{005}[rc][rc]{\matlabtextC $0$}%
\psfrag{006}[rc][rc]{\matlabtextC $200$}%
\psfrag{007}[rc][rc]{\matlabtextC $400$}%
\psfrag{008}[rc][rc]{\matlabtextC $600$}%
\psfrag{009}[rc][rc]{\matlabtextC $800$}%
%
%% </ytick>

==> Figures/pemonte100922/snr16_mt67-5_eta0-05_CHIRP.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{010}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{011}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{012}[bc][bc]{\matlabtextB Signal: $\rho=16$, $M_T=67.5M_\odot$, $\eta=0.05$}%
\psfrag{013}[bc][bc]{\matlabtextB $\#$}%
\psfrag{014}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 40$}%
\psfrag{001}[ct][ct]{\matlabtextC $\matlabfragNegXTick 20$}%
\psfrag{002}[ct][ct]{\matlabtextC $0$}%
\psfrag{003}[ct][ct]{\matlabtextC $20$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{004}[rc][rc]{\matlabtextC $0$}%
\psfrag{005}[rc][rc]{\matlabtextC $200$}%
\psfrag{006}[rc][rc]{\matlabtextC $400$}%
\psfrag{007}[rc][rc]{\matlabtextC $600$}%
\psfrag{008}[rc][rc]{\matlabtextC $800$}%
\psfrag{009}[rc][rc]{\matlabtextC $1000$}%
%
%% </ytick>

==> Figures/pemonte100922/snr16_mt67-5_eta0-05_CHIRPsmall.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{010}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{011}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{012}[bc][bc]{\matlabtextB Signal: $\rho=16$, $M_T=67.5M_\odot$, $\eta=0.05$}%
\psfrag{013}[bc][bc]{\matlabtextB $\#$}%
\psfrag{014}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 40$}%
\psfrag{001}[ct][ct]{\matlabtextC $\matlabfragNegXTick 20$}%
\psfrag{002}[ct][ct]{\matlabtextC $0$}%
\psfrag{003}[ct][ct]{\matlabtextC $20$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{004}[rc][rc]{\matlabtextC $0$}%
\psfrag{005}[rc][rc]{\matlabtextC $200$}%
\psfrag{006}[rc][rc]{\matlabtextC $400$}%
\psfrag{007}[rc][rc]{\matlabtextC $600$}%
\psfrag{008}[rc][rc]{\matlabtextC $800$}%
\psfrag{009}[rc][rc]{\matlabtextC $1000$}%
%
%% </ytick>

==> Figures/pemonte100922/snr16_mt67-5_eta0-075_CHIRP.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{010}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{011}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{012}[bc][bc]{\matlabtextB Signal: $\rho=16$, $M_T=67.5M_\odot$, $\eta=0.075$}%
\psfrag{013}[bc][bc]{\matlabtextB $\#$}%
\psfrag{014}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 40$}%
\psfrag{001}[ct][ct]{\matlabtextC $\matlabfragNegXTick 20$}%
\psfrag{002}[ct][ct]{\matlabtextC $0$}%
\psfrag{003}[ct][ct]{\matlabtextC $20$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{004}[rc][rc]{\matlabtextC $0$}%
\psfrag{005}[rc][rc]{\matlabtextC $200$}%
\psfrag{006}[rc][rc]{\matlabtextC $400$}%
\psfrag{007}[rc][rc]{\matlabtextC $600$}%
\psfrag{008}[rc][rc]{\matlabtextC $800$}%
\psfrag{009}[rc][rc]{\matlabtextC $1000$}%
%
%% </ytick>

==> Figures/pemonte100922/snr16_mt67-5_eta0-075_CHIRPsmall.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{010}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{011}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{012}[bc][bc]{\matlabtextB Signal: $\rho=16$, $M_T=67.5M_\odot$, $\eta=0.075$}%
\psfrag{013}[bc][bc]{\matlabtextB $\#$}%
\psfrag{014}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 40$}%
\psfrag{001}[ct][ct]{\matlabtextC $\matlabfragNegXTick 20$}%
\psfrag{002}[ct][ct]{\matlabtextC $0$}%
\psfrag{003}[ct][ct]{\matlabtextC $20$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{004}[rc][rc]{\matlabtextC $0$}%
\psfrag{005}[rc][rc]{\matlabtextC $200$}%
\psfrag{006}[rc][rc]{\matlabtextC $400$}%
\psfrag{007}[rc][rc]{\matlabtextC $600$}%
\psfrag{008}[rc][rc]{\matlabtextC $800$}%
\psfrag{009}[rc][rc]{\matlabtextC $1000$}%
%
%% </ytick>

==> Figures/pemonte100922/snr16_mt67-5_eta0-111_CHIRP.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{012}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{013}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{014}[bc][bc]{\matlabtextB Signal: $\rho=16$, $M_T=67.5M_\odot$, $\eta=0.111$}%
\psfrag{015}[bc][bc]{\matlabtextB $\#$}%
\psfrag{016}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 50$}%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $50$}%
\psfrag{003}[ct][ct]{\matlabtextC $100$}%
\psfrag{004}[ct][ct]{\matlabtextC $150$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{005}[rc][rc]{\matlabtextC $0$}%
\psfrag{006}[rc][rc]{\matlabtextC $200$}%
\psfrag{007}[rc][rc]{\matlabtextC $400$}%
\psfrag{008}[rc][rc]{\matlabtextC $600$}%
\psfrag{009}[rc][rc]{\matlabtextC $800$}%
\psfrag{010}[rc][rc]{\matlabtextC $1000$}%
\psfrag{011}[rc][rc]{\matlabtextC $1200$}%
%
%% </ytick>

==> Figures/pemonte100922/snr16_mt67-5_eta0-111_CHIRPsmall.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{012}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{013}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{014}[bc][bc]{\matlabtextB Signal: $\rho=16$, $M_T=67.5M_\odot$, $\eta=0.111$}%
\psfrag{015}[bc][bc]{\matlabtextB $\#$}%
\psfrag{016}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 50$}%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $50$}%
\psfrag{003}[ct][ct]{\matlabtextC $100$}%
\psfrag{004}[ct][ct]{\matlabtextC $150$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{005}[rc][rc]{\matlabtextC $0$}%
\psfrag{006}[rc][rc]{\matlabtextC $200$}%
\psfrag{007}[rc][rc]{\matlabtextC $400$}%
\psfrag{008}[rc][rc]{\matlabtextC $600$}%
\psfrag{009}[rc][rc]{\matlabtextC $800$}%
\psfrag{010}[rc][rc]{\matlabtextC $1000$}%
\psfrag{011}[rc][rc]{\matlabtextC $1200$}%
%
%% </ytick>

==> Figures/pemonte100922/snr16_mt67-5_eta0-167_CHIRP.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{011}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{012}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{013}[bc][bc]{\matlabtextB Signal: $\rho=16$, $M_T=67.5M_\odot$, $\eta=0.167$}%
\psfrag{014}[bc][bc]{\matlabtextB $\#$}%
\psfrag{015}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 20$}%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $20$}%
\psfrag{003}[ct][ct]{\matlabtextC $40$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{004}[rc][rc]{\matlabtextC $0$}%
\psfrag{005}[rc][rc]{\matlabtextC $100$}%
\psfrag{006}[rc][rc]{\matlabtextC $200$}%
\psfrag{007}[rc][rc]{\matlabtextC $300$}%
\psfrag{008}[rc][rc]{\matlabtextC $400$}%
\psfrag{009}[rc][rc]{\matlabtextC $500$}%
\psfrag{010}[rc][rc]{\matlabtextC $600$}%
%
%% </ytick>

==> Figures/pemonte100922/snr16_mt67-5_eta0-167_CHIRPsmall.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{011}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{012}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{013}[bc][bc]{\matlabtextB Signal: $\rho=16$, $M_T=67.5M_\odot$, $\eta=0.167$}%
\psfrag{014}[bc][bc]{\matlabtextB $\#$}%
\psfrag{015}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 20$}%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $20$}%
\psfrag{003}[ct][ct]{\matlabtextC $40$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{004}[rc][rc]{\matlabtextC $0$}%
\psfrag{005}[rc][rc]{\matlabtextC $100$}%
\psfrag{006}[rc][rc]{\matlabtextC $200$}%
\psfrag{007}[rc][rc]{\matlabtextC $300$}%
\psfrag{008}[rc][rc]{\matlabtextC $400$}%
\psfrag{009}[rc][rc]{\matlabtextC $500$}%
\psfrag{010}[rc][rc]{\matlabtextC $600$}%
%
%% </ytick>

==> Figures/pemonte100922/snr16_mt67-5_eta0-25_CHIRP.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{009}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{010}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{011}[bc][bc]{\matlabtextB Signal: $\rho=16$, $M_T=67.5M_\odot$, $\eta=0.25$}%
\psfrag{012}[bc][bc]{\matlabtextB $\#$}%
\psfrag{013}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 40$}%
\psfrag{001}[ct][ct]{\matlabtextC $\matlabfragNegXTick 20$}%
\psfrag{002}[ct][ct]{\matlabtextC $0$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{003}[rc][rc]{\matlabtextC $0$}%
\psfrag{004}[rc][rc]{\matlabtextC $100$}%
\psfrag{005}[rc][rc]{\matlabtextC $200$}%
\psfrag{006}[rc][rc]{\matlabtextC $300$}%
\psfrag{007}[rc][rc]{\matlabtextC $400$}%
\psfrag{008}[rc][rc]{\matlabtextC $500$}%
%
%% </ytick>

==> Figures/pemonte100922/snr16_mt67-5_eta0-25_CHIRPsmall.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{009}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{010}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{011}[bc][bc]{\matlabtextB Signal: $\rho=16$, $M_T=67.5M_\odot$, $\eta=0.25$}%
\psfrag{012}[bc][bc]{\matlabtextB $\#$}%
\psfrag{013}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 40$}%
\psfrag{001}[ct][ct]{\matlabtextC $\matlabfragNegXTick 20$}%
\psfrag{002}[ct][ct]{\matlabtextC $0$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{003}[rc][rc]{\matlabtextC $0$}%
\psfrag{004}[rc][rc]{\matlabtextC $100$}%
\psfrag{005}[rc][rc]{\matlabtextC $200$}%
\psfrag{006}[rc][rc]{\matlabtextC $300$}%
\psfrag{007}[rc][rc]{\matlabtextC $400$}%
\psfrag{008}[rc][rc]{\matlabtextC $500$}%
%
%% </ytick>

==> Figures/pemonte100922/snr16_mt80_eta0-05_CHIRP.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{008}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{009}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{010}[bc][bc]{\matlabtextB Signal: $\rho=16$, $M_T=80M_\odot$, $\eta=0.05$}%
\psfrag{011}[bc][bc]{\matlabtextB $\#$}%
\psfrag{012}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 50$}%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $50$}%
\psfrag{003}[ct][ct]{\matlabtextC $100$}%
\psfrag{004}[ct][ct]{\matlabtextC $150$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{005}[rc][rc]{\matlabtextC $0$}%
\psfrag{006}[rc][rc]{\matlabtextC $500$}%
\psfrag{007}[rc][rc]{\matlabtextC $1000$}%
%
%% </ytick>

==> Figures/pemonte100922/snr16_mt80_eta0-05_CHIRPsmall.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{008}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{009}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{010}[bc][bc]{\matlabtextB Signal: $\rho=16$, $M_T=80M_\odot$, $\eta=0.05$}%
\psfrag{011}[bc][bc]{\matlabtextB $\#$}%
\psfrag{012}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 50$}%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $50$}%
\psfrag{003}[ct][ct]{\matlabtextC $100$}%
\psfrag{004}[ct][ct]{\matlabtextC $150$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{005}[rc][rc]{\matlabtextC $0$}%
\psfrag{006}[rc][rc]{\matlabtextC $500$}%
\psfrag{007}[rc][rc]{\matlabtextC $1000$}%
%
%% </ytick>

==> Figures/pemonte100922/snr16_mt80_eta0-075_CHIRP.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{012}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{013}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{014}[bc][bc]{\matlabtextB Signal: $\rho=16$, $M_T=80M_\odot$, $\eta=0.075$}%
\psfrag{015}[bc][bc]{\matlabtextB $\#$}%
\psfrag{016}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 50$}%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $50$}%
\psfrag{003}[ct][ct]{\matlabtextC $100$}%
\psfrag{004}[ct][ct]{\matlabtextC $150$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{005}[rc][rc]{\matlabtextC $0$}%
\psfrag{006}[rc][rc]{\matlabtextC $200$}%
\psfrag{007}[rc][rc]{\matlabtextC $400$}%
\psfrag{008}[rc][rc]{\matlabtextC $600$}%
\psfrag{009}[rc][rc]{\matlabtextC $800$}%
\psfrag{010}[rc][rc]{\matlabtextC $1000$}%
\psfrag{011}[rc][rc]{\matlabtextC $1200$}%
%
%% </ytick>

==> Figures/pemonte100922/snr16_mt80_eta0-075_CHIRPsmall.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{012}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{013}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{014}[bc][bc]{\matlabtextB Signal: $\rho=16$, $M_T=80M_\odot$, $\eta=0.075$}%
\psfrag{015}[bc][bc]{\matlabtextB $\#$}%
\psfrag{016}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 50$}%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $50$}%
\psfrag{003}[ct][ct]{\matlabtextC $100$}%
\psfrag{004}[ct][ct]{\matlabtextC $150$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{005}[rc][rc]{\matlabtextC $0$}%
\psfrag{006}[rc][rc]{\matlabtextC $200$}%
\psfrag{007}[rc][rc]{\matlabtextC $400$}%
\psfrag{008}[rc][rc]{\matlabtextC $600$}%
\psfrag{009}[rc][rc]{\matlabtextC $800$}%
\psfrag{010}[rc][rc]{\matlabtextC $1000$}%
\psfrag{011}[rc][rc]{\matlabtextC $1200$}%
%
%% </ytick>

==> Figures/pemonte100922/snr16_mt80_eta0-111_CHIRP.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{009}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{010}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{011}[bc][bc]{\matlabtextB Signal: $\rho=16$, $M_T=80M_\odot$, $\eta=0.111$}%
\psfrag{012}[bc][bc]{\matlabtextB $\#$}%
\psfrag{013}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 50$}%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $50$}%
\psfrag{003}[ct][ct]{\matlabtextC $100$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{004}[rc][rc]{\matlabtextC $0$}%
\psfrag{005}[rc][rc]{\matlabtextC $200$}%
\psfrag{006}[rc][rc]{\matlabtextC $400$}%
\psfrag{007}[rc][rc]{\matlabtextC $600$}%
\psfrag{008}[rc][rc]{\matlabtextC $800$}%
%
%% </ytick>

==> Figures/pemonte100922/snr16_mt80_eta0-111_CHIRPsmall.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{009}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{010}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{011}[bc][bc]{\matlabtextB Signal: $\rho=16$, $M_T=80M_\odot$, $\eta=0.111$}%
\psfrag{012}[bc][bc]{\matlabtextB $\#$}%
\psfrag{013}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 50$}%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $50$}%
\psfrag{003}[ct][ct]{\matlabtextC $100$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{004}[rc][rc]{\matlabtextC $0$}%
\psfrag{005}[rc][rc]{\matlabtextC $200$}%
\psfrag{006}[rc][rc]{\matlabtextC $400$}%
\psfrag{007}[rc][rc]{\matlabtextC $600$}%
\psfrag{008}[rc][rc]{\matlabtextC $800$}%
%
%% </ytick>

==> Figures/pemonte100922/snr16_mt80_eta0-167_CHIRP.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{009}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{010}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{011}[bc][bc]{\matlabtextB Signal: $\rho=16$, $M_T=80M_\odot$, $\eta=0.167$}%
\psfrag{012}[bc][bc]{\matlabtextB $\#$}%
\psfrag{013}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 50$}%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $50$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{003}[rc][rc]{\matlabtextC $0$}%
\psfrag{004}[rc][rc]{\matlabtextC $100$}%
\psfrag{005}[rc][rc]{\matlabtextC $200$}%
\psfrag{006}[rc][rc]{\matlabtextC $300$}%
\psfrag{007}[rc][rc]{\matlabtextC $400$}%
\psfrag{008}[rc][rc]{\matlabtextC $500$}%
%
%% </ytick>

==> Figures/pemonte100922/snr16_mt80_eta0-167_CHIRPsmall.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{009}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{010}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{011}[bc][bc]{\matlabtextB Signal: $\rho=16$, $M_T=80M_\odot$, $\eta=0.167$}%
\psfrag{012}[bc][bc]{\matlabtextB $\#$}%
\psfrag{013}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 50$}%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $50$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{003}[rc][rc]{\matlabtextC $0$}%
\psfrag{004}[rc][rc]{\matlabtextC $100$}%
\psfrag{005}[rc][rc]{\matlabtextC $200$}%
\psfrag{006}[rc][rc]{\matlabtextC $300$}%
\psfrag{007}[rc][rc]{\matlabtextC $400$}%
\psfrag{008}[rc][rc]{\matlabtextC $500$}%
%
%% </ytick>

==> Figures/pemonte100922/snr16_mt80_eta0-25_CHIRP.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{010}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{011}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{012}[bc][bc]{\matlabtextB Signal: $\rho=16$, $M_T=80M_\odot$, $\eta=0.25$}%
\psfrag{013}[bc][bc]{\matlabtextB $\#$}%
\psfrag{014}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 60$}%
\psfrag{001}[ct][ct]{\matlabtextC $\matlabfragNegXTick 40$}%
\psfrag{002}[ct][ct]{\matlabtextC $\matlabfragNegXTick 20$}%
\psfrag{003}[ct][ct]{\matlabtextC $0$}%
\psfrag{004}[ct][ct]{\matlabtextC $20$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{005}[rc][rc]{\matlabtextC $0$}%
\psfrag{006}[rc][rc]{\matlabtextC $100$}%
\psfrag{007}[rc][rc]{\matlabtextC $200$}%
\psfrag{008}[rc][rc]{\matlabtextC $300$}%
\psfrag{009}[rc][rc]{\matlabtextC $400$}%
%
%% </ytick>

==> Figures/pemonte100922/snr16_mt80_eta0-25_CHIRPsmall.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{010}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{011}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{012}[bc][bc]{\matlabtextB Signal: $\rho=16$, $M_T=80M_\odot$, $\eta=0.25$}%
\psfrag{013}[bc][bc]{\matlabtextB $\#$}%
\psfrag{014}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 60$}%
\psfrag{001}[ct][ct]{\matlabtextC $\matlabfragNegXTick 40$}%
\psfrag{002}[ct][ct]{\matlabtextC $\matlabfragNegXTick 20$}%
\psfrag{003}[ct][ct]{\matlabtextC $0$}%
\psfrag{004}[ct][ct]{\matlabtextC $20$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{005}[rc][rc]{\matlabtextC $0$}%
\psfrag{006}[rc][rc]{\matlabtextC $100$}%
\psfrag{007}[rc][rc]{\matlabtextC $200$}%
\psfrag{008}[rc][rc]{\matlabtextC $300$}%
\psfrag{009}[rc][rc]{\matlabtextC $400$}%
%
%% </ytick>

==> Figures/pemonte100922/snr64_mt30_eta0-05_CHIRP.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{009}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{010}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{011}[bc][bc]{\matlabtextB Signal: $\rho=64$, $M_T=30M_\odot$, $\eta=0.05$}%
\psfrag{012}[bc][bc]{\matlabtextB $\#$}%
\psfrag{013}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 0.5$}%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $0.5$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{003}[rc][rc]{\matlabtextC $0$}%
\psfrag{004}[rc][rc]{\matlabtextC $200$}%
\psfrag{005}[rc][rc]{\matlabtextC $400$}%
\psfrag{006}[rc][rc]{\matlabtextC $600$}%
\psfrag{007}[rc][rc]{\matlabtextC $800$}%
\psfrag{008}[rc][rc]{\matlabtextC $1000$}%
%
%% </ytick>

==> Figures/pemonte100922/snr64_mt30_eta0-05_CHIRPsmall.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{009}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{010}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{011}[bc][bc]{\matlabtextB Signal: $\rho=64$, $M_T=30M_\odot$, $\eta=0.05$}%
\psfrag{012}[bc][bc]{\matlabtextB $\#$}%
\psfrag{013}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 0.5$}%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $0.5$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{003}[rc][rc]{\matlabtextC $0$}%
\psfrag{004}[rc][rc]{\matlabtextC $200$}%
\psfrag{005}[rc][rc]{\matlabtextC $400$}%
\psfrag{006}[rc][rc]{\matlabtextC $600$}%
\psfrag{007}[rc][rc]{\matlabtextC $800$}%
\psfrag{008}[rc][rc]{\matlabtextC $1000$}%
%
%% </ytick>

==> Figures/pemonte100922/snr64_mt30_eta0-075_CHIRP.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{006}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{007}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{008}[bc][bc]{\matlabtextB Signal: $\rho=64$, $M_T=30M_\odot$, $\eta=0.075$}%
\psfrag{009}[bc][bc]{\matlabtextB $\#$}%
\psfrag{010}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 0.5$}%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $0.5$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{003}[rc][rc]{\matlabtextC $0$}%
\psfrag{004}[rc][rc]{\matlabtextC $500$}%
\psfrag{005}[rc][rc]{\matlabtextC $1000$}%
%
%% </ytick>

==> Figures/pemonte100922/snr64_mt30_eta0-075_CHIRPsmall.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{006}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{007}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{008}[bc][bc]{\matlabtextB Signal: $\rho=64$, $M_T=30M_\odot$, $\eta=0.075$}%
\psfrag{009}[bc][bc]{\matlabtextB $\#$}%
\psfrag{010}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 0.5$}%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $0.5$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{003}[rc][rc]{\matlabtextC $0$}%
\psfrag{004}[rc][rc]{\matlabtextC $500$}%
\psfrag{005}[rc][rc]{\matlabtextC $1000$}%
%
%% </ytick>

==> Figures/pemonte100922/snr64_mt30_eta0-111_CHIRP.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{006}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{007}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{008}[bc][bc]{\matlabtextB Signal: $\rho=64$, $M_T=30M_\odot$, $\eta=0.111$}%
\psfrag{009}[bc][bc]{\matlabtextB $\#$}%
\psfrag{010}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 1$}%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $1$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{003}[rc][rc]{\matlabtextC $0$}%
\psfrag{004}[rc][rc]{\matlabtextC $500$}%
\psfrag{005}[rc][rc]{\matlabtextC $1000$}%
%
%% </ytick>

==> Figures/pemonte100922/snr64_mt30_eta0-111_CHIRPsmall.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{006}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{007}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{008}[bc][bc]{\matlabtextB Signal: $\rho=64$, $M_T=30M_\odot$, $\eta=0.111$}%
\psfrag{009}[bc][bc]{\matlabtextB $\#$}%
\psfrag{010}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 1$}%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $1$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{003}[rc][rc]{\matlabtextC $0$}%
\psfrag{004}[rc][rc]{\matlabtextC $500$}%
\psfrag{005}[rc][rc]{\matlabtextC $1000$}%
%
%% </ytick>

==> Figures/pemonte100922/snr64_mt30_eta0-167_CHIRP.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{012}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{013}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{014}[bc][bc]{\matlabtextB Signal: $\rho=64$, $M_T=30M_\odot$, $\eta=0.167$}%
\psfrag{015}[bc][bc]{\matlabtextB $\#$}%
\psfrag{016}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 2$}%
\psfrag{001}[ct][ct]{\matlabtextC $\matlabfragNegXTick 1$}%
\psfrag{002}[ct][ct]{\matlabtextC $0$}%
\psfrag{003}[ct][ct]{\matlabtextC $1$}%
\psfrag{004}[ct][ct]{\matlabtextC $2$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{005}[rc][rc]{\matlabtextC $0$}%
\psfrag{006}[rc][rc]{\matlabtextC $200$}%
\psfrag{007}[rc][rc]{\matlabtextC $400$}%
\psfrag{008}[rc][rc]{\matlabtextC $600$}%
\psfrag{009}[rc][rc]{\matlabtextC $800$}%
\psfrag{010}[rc][rc]{\matlabtextC $1000$}%
\psfrag{011}[rc][rc]{\matlabtextC $1200$}%
%
%% </ytick>

==> Figures/pemonte100922/snr64_mt30_eta0-167_CHIRPsmall.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{012}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{013}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{014}[bc][bc]{\matlabtextB Signal: $\rho=64$, $M_T=30M_\odot$, $\eta=0.167$}%
\psfrag{015}[bc][bc]{\matlabtextB $\#$}%
\psfrag{016}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 2$}%
\psfrag{001}[ct][ct]{\matlabtextC $\matlabfragNegXTick 1$}%
\psfrag{002}[ct][ct]{\matlabtextC $0$}%
\psfrag{003}[ct][ct]{\matlabtextC $1$}%
\psfrag{004}[ct][ct]{\matlabtextC $2$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{005}[rc][rc]{\matlabtextC $0$}%
\psfrag{006}[rc][rc]{\matlabtextC $200$}%
\psfrag{007}[rc][rc]{\matlabtextC $400$}%
\psfrag{008}[rc][rc]{\matlabtextC $600$}%
\psfrag{009}[rc][rc]{\matlabtextC $800$}%
\psfrag{010}[rc][rc]{\matlabtextC $1000$}%
\psfrag{011}[rc][rc]{\matlabtextC $1200$}%
%
%% </ytick>

==> Figures/pemonte100922/snr64_mt30_eta0-25_CHIRP.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{008}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{009}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{010}[bc][bc]{\matlabtextB Signal: $\rho=64$, $M_T=30M_\odot$, $\eta=0.25$}%
\psfrag{011}[bc][bc]{\matlabtextB $\#$}%
\psfrag{012}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 4$}%
\psfrag{001}[ct][ct]{\matlabtextC $\matlabfragNegXTick 3$}%
\psfrag{002}[ct][ct]{\matlabtextC $\matlabfragNegXTick 2$}%
\psfrag{003}[ct][ct]{\matlabtextC $\matlabfragNegXTick 1$}%
\psfrag{004}[ct][ct]{\matlabtextC $0$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{005}[rc][rc]{\matlabtextC $0$}%
\psfrag{006}[rc][rc]{\matlabtextC $500$}%
\psfrag{007}[rc][rc]{\matlabtextC $1000$}%
%
%% </ytick>

==> Figures/pemonte100922/snr64_mt30_eta0-25_CHIRPsmall.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{008}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{009}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{010}[bc][bc]{\matlabtextB Signal: $\rho=64$, $M_T=30M_\odot$, $\eta=0.25$}%
\psfrag{011}[bc][bc]{\matlabtextB $\#$}%
\psfrag{012}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 4$}%
\psfrag{001}[ct][ct]{\matlabtextC $\matlabfragNegXTick 3$}%
\psfrag{002}[ct][ct]{\matlabtextC $\matlabfragNegXTick 2$}%
\psfrag{003}[ct][ct]{\matlabtextC $\matlabfragNegXTick 1$}%
\psfrag{004}[ct][ct]{\matlabtextC $0$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{005}[rc][rc]{\matlabtextC $0$}%
\psfrag{006}[rc][rc]{\matlabtextC $500$}%
\psfrag{007}[rc][rc]{\matlabtextC $1000$}%
%
%% </ytick>

==> Figures/pemonte100922/snr64_mt45_eta0-05_CHIRP.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{010}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{011}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{012}[bc][bc]{\matlabtextB Signal: $\rho=64$, $M_T=45M_\odot$, $\eta=0.05$}%
\psfrag{013}[bc][bc]{\matlabtextB $\#$}%
\psfrag{014}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 1$}%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $1$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{003}[rc][rc]{\matlabtextC $0$}%
\psfrag{004}[rc][rc]{\matlabtextC $200$}%
\psfrag{005}[rc][rc]{\matlabtextC $400$}%
\psfrag{006}[rc][rc]{\matlabtextC $600$}%
\psfrag{007}[rc][rc]{\matlabtextC $800$}%
\psfrag{008}[rc][rc]{\matlabtextC $1000$}%
\psfrag{009}[rc][rc]{\matlabtextC $1200$}%
%
%% </ytick>

==> Figures/pemonte100922/snr64_mt45_eta0-05_CHIRPsmall.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{010}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{011}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{012}[bc][bc]{\matlabtextB Signal: $\rho=64$, $M_T=45M_\odot$, $\eta=0.05$}%
\psfrag{013}[bc][bc]{\matlabtextB $\#$}%
\psfrag{014}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 1$}%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $1$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{003}[rc][rc]{\matlabtextC $0$}%
\psfrag{004}[rc][rc]{\matlabtextC $200$}%
\psfrag{005}[rc][rc]{\matlabtextC $400$}%
\psfrag{006}[rc][rc]{\matlabtextC $600$}%
\psfrag{007}[rc][rc]{\matlabtextC $800$}%
\psfrag{008}[rc][rc]{\matlabtextC $1000$}%
\psfrag{009}[rc][rc]{\matlabtextC $1200$}%
%
%% </ytick>

==> Figures/pemonte100922/snr64_mt45_eta0-075_CHIRP.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{007}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{008}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{009}[bc][bc]{\matlabtextB Signal: $\rho=64$, $M_T=45M_\odot$, $\eta=0.075$}%
\psfrag{010}[bc][bc]{\matlabtextB $\#$}%
\psfrag{011}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 2$}%
\psfrag{001}[ct][ct]{\matlabtextC $\matlabfragNegXTick 1$}%
\psfrag{002}[ct][ct]{\matlabtextC $0$}%
\psfrag{003}[ct][ct]{\matlabtextC $1$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{004}[rc][rc]{\matlabtextC $0$}%
\psfrag{005}[rc][rc]{\matlabtextC $500$}%
\psfrag{006}[rc][rc]{\matlabtextC $1000$}%
%
%% </ytick>

==> Figures/pemonte100922/snr64_mt45_eta0-075_CHIRPsmall.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{007}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{008}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{009}[bc][bc]{\matlabtextB Signal: $\rho=64$, $M_T=45M_\odot$, $\eta=0.075$}%
\psfrag{010}[bc][bc]{\matlabtextB $\#$}%
\psfrag{011}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 2$}%
\psfrag{001}[ct][ct]{\matlabtextC $\matlabfragNegXTick 1$}%
\psfrag{002}[ct][ct]{\matlabtextC $0$}%
\psfrag{003}[ct][ct]{\matlabtextC $1$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{004}[rc][rc]{\matlabtextC $0$}%
\psfrag{005}[rc][rc]{\matlabtextC $500$}%
\psfrag{006}[rc][rc]{\matlabtextC $1000$}%
%
%% </ytick>

==> Figures/pemonte100922/snr64_mt45_eta0-111_CHIRP.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{009}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{010}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{011}[bc][bc]{\matlabtextB Signal: $\rho=64$, $M_T=45M_\odot$, $\eta=0.111$}%
\psfrag{012}[bc][bc]{\matlabtextB $\#$}%
\psfrag{013}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 2$}%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $2$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{003}[rc][rc]{\matlabtextC $0$}%
\psfrag{004}[rc][rc]{\matlabtextC $200$}%
\psfrag{005}[rc][rc]{\matlabtextC $400$}%
\psfrag{006}[rc][rc]{\matlabtextC $600$}%
\psfrag{007}[rc][rc]{\matlabtextC $800$}%
\psfrag{008}[rc][rc]{\matlabtextC $1000$}%
%
%% </ytick>

==> Figures/pemonte100922/snr64_mt45_eta0-111_CHIRPsmall.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{009}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{010}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{011}[bc][bc]{\matlabtextB Signal: $\rho=64$, $M_T=45M_\odot$, $\eta=0.111$}%
\psfrag{012}[bc][bc]{\matlabtextB $\#$}%
\psfrag{013}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 2$}%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $2$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{003}[rc][rc]{\matlabtextC $0$}%
\psfrag{004}[rc][rc]{\matlabtextC $200$}%
\psfrag{005}[rc][rc]{\matlabtextC $400$}%
\psfrag{006}[rc][rc]{\matlabtextC $600$}%
\psfrag{007}[rc][rc]{\matlabtextC $800$}%
\psfrag{008}[rc][rc]{\matlabtextC $1000$}%
%
%% </ytick>

==> Figures/pemonte100922/snr64_mt45_eta0-167_CHIRP.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{010}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{011}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{012}[bc][bc]{\matlabtextB Signal: $\rho=64$, $M_T=45M_\odot$, $\eta=0.167$}%
\psfrag{013}[bc][bc]{\matlabtextB $\#$}%
\psfrag{014}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 5$}%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $5$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{003}[rc][rc]{\matlabtextC $0$}%
\psfrag{004}[rc][rc]{\matlabtextC $100$}%
\psfrag{005}[rc][rc]{\matlabtextC $200$}%
\psfrag{006}[rc][rc]{\matlabtextC $300$}%
\psfrag{007}[rc][rc]{\matlabtextC $400$}%
\psfrag{008}[rc][rc]{\matlabtextC $500$}%
\psfrag{009}[rc][rc]{\matlabtextC $600$}%
%
%% </ytick>

==> Figures/pemonte100922/snr64_mt45_eta0-167_CHIRPsmall.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{010}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{011}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{012}[bc][bc]{\matlabtextB Signal: $\rho=64$, $M_T=45M_\odot$, $\eta=0.167$}%
\psfrag{013}[bc][bc]{\matlabtextB $\#$}%
\psfrag{014}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 5$}%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $5$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{003}[rc][rc]{\matlabtextC $0$}%
\psfrag{004}[rc][rc]{\matlabtextC $100$}%
\psfrag{005}[rc][rc]{\matlabtextC $200$}%
\psfrag{006}[rc][rc]{\matlabtextC $300$}%
\psfrag{007}[rc][rc]{\matlabtextC $400$}%
\psfrag{008}[rc][rc]{\matlabtextC $500$}%
\psfrag{009}[rc][rc]{\matlabtextC $600$}%
%
%% </ytick>

==> Figures/pemonte100922/snr64_mt45_eta0-25_CHIRP.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{009}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{010}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{011}[bc][bc]{\matlabtextB Signal: $\rho=64$, $M_T=45M_\odot$, $\eta=0.25$}%
\psfrag{012}[bc][bc]{\matlabtextB $\#$}%
\psfrag{013}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 6$}%
\psfrag{001}[ct][ct]{\matlabtextC $\matlabfragNegXTick 4$}%
\psfrag{002}[ct][ct]{\matlabtextC $\matlabfragNegXTick 2$}%
\psfrag{003}[ct][ct]{\matlabtextC $0$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{004}[rc][rc]{\matlabtextC $0$}%
\psfrag{005}[rc][rc]{\matlabtextC $200$}%
\psfrag{006}[rc][rc]{\matlabtextC $400$}%
\psfrag{007}[rc][rc]{\matlabtextC $600$}%
\psfrag{008}[rc][rc]{\matlabtextC $800$}%
%
%% </ytick>

==> Figures/pemonte100922/snr64_mt45_eta0-25_CHIRPsmall.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{009}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{010}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{011}[bc][bc]{\matlabtextB Signal: $\rho=64$, $M_T=45M_\odot$, $\eta=0.25$}%
\psfrag{012}[bc][bc]{\matlabtextB $\#$}%
\psfrag{013}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 6$}%
\psfrag{001}[ct][ct]{\matlabtextC $\matlabfragNegXTick 4$}%
\psfrag{002}[ct][ct]{\matlabtextC $\matlabfragNegXTick 2$}%
\psfrag{003}[ct][ct]{\matlabtextC $0$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{004}[rc][rc]{\matlabtextC $0$}%
\psfrag{005}[rc][rc]{\matlabtextC $200$}%
\psfrag{006}[rc][rc]{\matlabtextC $400$}%
\psfrag{007}[rc][rc]{\matlabtextC $600$}%
\psfrag{008}[rc][rc]{\matlabtextC $800$}%
%
%% </ytick>

==> Figures/pemonte100922/snr64_mt67-5_eta0-05_CHIRP.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{009}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{010}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{011}[bc][bc]{\matlabtextB Signal: $\rho=64$, $M_T=67.5M_\odot$, $\eta=0.05$}%
\psfrag{012}[bc][bc]{\matlabtextB $\#$}%
\psfrag{013}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 40$}%
\psfrag{001}[ct][ct]{\matlabtextC $\matlabfragNegXTick 20$}%
\psfrag{002}[ct][ct]{\matlabtextC $0$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{003}[rc][rc]{\matlabtextC $0$}%
\psfrag{004}[rc][rc]{\matlabtextC $200$}%
\psfrag{005}[rc][rc]{\matlabtextC $400$}%
\psfrag{006}[rc][rc]{\matlabtextC $600$}%
\psfrag{007}[rc][rc]{\matlabtextC $800$}%
\psfrag{008}[rc][rc]{\matlabtextC $1000$}%
%
%% </ytick>

==> Figures/pemonte100922/snr64_mt67-5_eta0-05_CHIRPsmall.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{009}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{010}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{011}[bc][bc]{\matlabtextB Signal: $\rho=64$, $M_T=67.5M_\odot$, $\eta=0.05$}%
\psfrag{012}[bc][bc]{\matlabtextB $\#$}%
\psfrag{013}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 40$}%
\psfrag{001}[ct][ct]{\matlabtextC $\matlabfragNegXTick 20$}%
\psfrag{002}[ct][ct]{\matlabtextC $0$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{003}[rc][rc]{\matlabtextC $0$}%
\psfrag{004}[rc][rc]{\matlabtextC $200$}%
\psfrag{005}[rc][rc]{\matlabtextC $400$}%
\psfrag{006}[rc][rc]{\matlabtextC $600$}%
\psfrag{007}[rc][rc]{\matlabtextC $800$}%
\psfrag{008}[rc][rc]{\matlabtextC $1000$}%
%
%% </ytick>

==> Figures/pemonte100922/snr64_mt67-5_eta0-075_CHIRP.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{012}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{013}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{014}[bc][bc]{\matlabtextB Signal: $\rho=64$, $M_T=67.5M_\odot$, $\eta=0.075$}%
\psfrag{015}[bc][bc]{\matlabtextB $\#$}%
\psfrag{016}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 5$}%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $5$}%
\psfrag{003}[ct][ct]{\matlabtextC $10$}%
\psfrag{004}[ct][ct]{\matlabtextC $15$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{005}[rc][rc]{\matlabtextC $0$}%
\psfrag{006}[rc][rc]{\matlabtextC $200$}%
\psfrag{007}[rc][rc]{\matlabtextC $400$}%
\psfrag{008}[rc][rc]{\matlabtextC $600$}%
\psfrag{009}[rc][rc]{\matlabtextC $800$}%
\psfrag{010}[rc][rc]{\matlabtextC $1000$}%
\psfrag{011}[rc][rc]{\matlabtextC $1200$}%
%
%% </ytick>

==> Figures/pemonte100922/snr64_mt67-5_eta0-075_CHIRPsmall.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{012}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{013}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{014}[bc][bc]{\matlabtextB Signal: $\rho=64$, $M_T=67.5M_\odot$, $\eta=0.075$}%
\psfrag{015}[bc][bc]{\matlabtextB $\#$}%
\psfrag{016}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 5$}%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $5$}%
\psfrag{003}[ct][ct]{\matlabtextC $10$}%
\psfrag{004}[ct][ct]{\matlabtextC $15$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{005}[rc][rc]{\matlabtextC $0$}%
\psfrag{006}[rc][rc]{\matlabtextC $200$}%
\psfrag{007}[rc][rc]{\matlabtextC $400$}%
\psfrag{008}[rc][rc]{\matlabtextC $600$}%
\psfrag{009}[rc][rc]{\matlabtextC $800$}%
\psfrag{010}[rc][rc]{\matlabtextC $1000$}%
\psfrag{011}[rc][rc]{\matlabtextC $1200$}%
%
%% </ytick>

==> Figures/pemonte100922/snr64_mt67-5_eta0-111_CHIRP.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{011}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{012}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{013}[bc][bc]{\matlabtextB Signal: $\rho=64$, $M_T=67.5M_\odot$, $\eta=0.111$}%
\psfrag{014}[bc][bc]{\matlabtextB $\#$}%
\psfrag{015}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 10$}%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $10$}%
\psfrag{003}[ct][ct]{\matlabtextC $20$}%
\psfrag{004}[ct][ct]{\matlabtextC $30$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{005}[rc][rc]{\matlabtextC $0$}%
\psfrag{006}[rc][rc]{\matlabtextC $200$}%
\psfrag{007}[rc][rc]{\matlabtextC $400$}%
\psfrag{008}[rc][rc]{\matlabtextC $600$}%
\psfrag{009}[rc][rc]{\matlabtextC $800$}%
\psfrag{010}[rc][rc]{\matlabtextC $1000$}%
%
%% </ytick>

==> Figures/pemonte100922/snr64_mt67-5_eta0-111_CHIRPsmall.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{011}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{012}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{013}[bc][bc]{\matlabtextB Signal: $\rho=64$, $M_T=67.5M_\odot$, $\eta=0.111$}%
\psfrag{014}[bc][bc]{\matlabtextB $\#$}%
\psfrag{015}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 10$}%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $10$}%
\psfrag{003}[ct][ct]{\matlabtextC $20$}%
\psfrag{004}[ct][ct]{\matlabtextC $30$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{005}[rc][rc]{\matlabtextC $0$}%
\psfrag{006}[rc][rc]{\matlabtextC $200$}%
\psfrag{007}[rc][rc]{\matlabtextC $400$}%
\psfrag{008}[rc][rc]{\matlabtextC $600$}%
\psfrag{009}[rc][rc]{\matlabtextC $800$}%
\psfrag{010}[rc][rc]{\matlabtextC $1000$}%
%
%% </ytick>

==> Figures/pemonte100922/snr64_mt67-5_eta0-167_CHIRP.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{009}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{010}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{011}[bc][bc]{\matlabtextB Signal: $\rho=64$, $M_T=67.5M_\odot$, $\eta=0.167$}%
\psfrag{012}[bc][bc]{\matlabtextB $\#$}%
\psfrag{013}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 10$}%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $10$}%
\psfrag{003}[ct][ct]{\matlabtextC $20$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{004}[rc][rc]{\matlabtextC $0$}%
\psfrag{005}[rc][rc]{\matlabtextC $200$}%
\psfrag{006}[rc][rc]{\matlabtextC $400$}%
\psfrag{007}[rc][rc]{\matlabtextC $600$}%
\psfrag{008}[rc][rc]{\matlabtextC $800$}%
%
%% </ytick>

==> Figures/pemonte100922/snr64_mt67-5_eta0-167_CHIRPsmall.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{009}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{010}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{011}[bc][bc]{\matlabtextB Signal: $\rho=64$, $M_T=67.5M_\odot$, $\eta=0.167$}%
\psfrag{012}[bc][bc]{\matlabtextB $\#$}%
\psfrag{013}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 10$}%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $10$}%
\psfrag{003}[ct][ct]{\matlabtextC $20$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{004}[rc][rc]{\matlabtextC $0$}%
\psfrag{005}[rc][rc]{\matlabtextC $200$}%
\psfrag{006}[rc][rc]{\matlabtextC $400$}%
\psfrag{007}[rc][rc]{\matlabtextC $600$}%
\psfrag{008}[rc][rc]{\matlabtextC $800$}%
%
%% </ytick>

==> Figures/pemonte100922/snr64_mt67-5_eta0-25_CHIRP.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{011}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{012}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{013}[bc][bc]{\matlabtextB Signal: $\rho=64$, $M_T=67.5M_\odot$, $\eta=0.25$}%
\psfrag{014}[bc][bc]{\matlabtextB $\#$}%
\psfrag{015}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 20$}%
\psfrag{001}[ct][ct]{\matlabtextC $\matlabfragNegXTick 15$}%
\psfrag{002}[ct][ct]{\matlabtextC $\matlabfragNegXTick 10$}%
\psfrag{003}[ct][ct]{\matlabtextC $\matlabfragNegXTick 5$}%
\psfrag{004}[ct][ct]{\matlabtextC $0$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{005}[rc][rc]{\matlabtextC $0$}%
\psfrag{006}[rc][rc]{\matlabtextC $200$}%
\psfrag{007}[rc][rc]{\matlabtextC $400$}%
\psfrag{008}[rc][rc]{\matlabtextC $600$}%
\psfrag{009}[rc][rc]{\matlabtextC $800$}%
\psfrag{010}[rc][rc]{\matlabtextC $1000$}%
%
%% </ytick>

==> Figures/pemonte100922/snr64_mt67-5_eta0-25_CHIRPsmall.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{011}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{012}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{013}[bc][bc]{\matlabtextB Signal: $\rho=64$, $M_T=67.5M_\odot$, $\eta=0.25$}%
\psfrag{014}[bc][bc]{\matlabtextB $\#$}%
\psfrag{015}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 20$}%
\psfrag{001}[ct][ct]{\matlabtextC $\matlabfragNegXTick 15$}%
\psfrag{002}[ct][ct]{\matlabtextC $\matlabfragNegXTick 10$}%
\psfrag{003}[ct][ct]{\matlabtextC $\matlabfragNegXTick 5$}%
\psfrag{004}[ct][ct]{\matlabtextC $0$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{005}[rc][rc]{\matlabtextC $0$}%
\psfrag{006}[rc][rc]{\matlabtextC $200$}%
\psfrag{007}[rc][rc]{\matlabtextC $400$}%
\psfrag{008}[rc][rc]{\matlabtextC $600$}%
\psfrag{009}[rc][rc]{\matlabtextC $800$}%
\psfrag{010}[rc][rc]{\matlabtextC $1000$}%
%
%% </ytick>

==> Figures/pemonte100922/snr64_mt80_eta0-05_CHIRP.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{008}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{009}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{010}[bc][bc]{\matlabtextB Signal: $\rho=64$, $M_T=80M_\odot$, $\eta=0.05$}%
\psfrag{011}[bc][bc]{\matlabtextB $\#$}%
\psfrag{012}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 40$}%
\psfrag{001}[ct][ct]{\matlabtextC $\matlabfragNegXTick 20$}%
\psfrag{002}[ct][ct]{\matlabtextC $0$}%
\psfrag{003}[ct][ct]{\matlabtextC $20$}%
\psfrag{004}[ct][ct]{\matlabtextC $40$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{005}[rc][rc]{\matlabtextC $0$}%
\psfrag{006}[rc][rc]{\matlabtextC $500$}%
\psfrag{007}[rc][rc]{\matlabtextC $1000$}%
%
%% </ytick>

==> Figures/pemonte100922/snr64_mt80_eta0-05_CHIRPsmall.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{008}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{009}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{010}[bc][bc]{\matlabtextB Signal: $\rho=64$, $M_T=80M_\odot$, $\eta=0.05$}%
\psfrag{011}[bc][bc]{\matlabtextB $\#$}%
\psfrag{012}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 40$}%
\psfrag{001}[ct][ct]{\matlabtextC $\matlabfragNegXTick 20$}%
\psfrag{002}[ct][ct]{\matlabtextC $0$}%
\psfrag{003}[ct][ct]{\matlabtextC $20$}%
\psfrag{004}[ct][ct]{\matlabtextC $40$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{005}[rc][rc]{\matlabtextC $0$}%
\psfrag{006}[rc][rc]{\matlabtextC $500$}%
\psfrag{007}[rc][rc]{\matlabtextC $1000$}%
%
%% </ytick>

==> Figures/pemonte100922/snr64_mt80_eta0-075_CHIRP.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{008}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{009}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{010}[bc][bc]{\matlabtextB Signal: $\rho=64$, $M_T=80M_\odot$, $\eta=0.075$}%
\psfrag{011}[bc][bc]{\matlabtextB $\#$}%
\psfrag{012}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 50$}%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $50$}%
\psfrag{003}[ct][ct]{\matlabtextC $100$}%
\psfrag{004}[ct][ct]{\matlabtextC $150$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{005}[rc][rc]{\matlabtextC $0$}%
\psfrag{006}[rc][rc]{\matlabtextC $500$}%
\psfrag{007}[rc][rc]{\matlabtextC $1000$}%
%
%% </ytick>

==> Figures/pemonte100922/snr64_mt80_eta0-075_CHIRPsmall.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{008}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{009}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{010}[bc][bc]{\matlabtextB Signal: $\rho=64$, $M_T=80M_\odot$, $\eta=0.075$}%
\psfrag{011}[bc][bc]{\matlabtextB $\#$}%
\psfrag{012}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 50$}%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $50$}%
\psfrag{003}[ct][ct]{\matlabtextC $100$}%
\psfrag{004}[ct][ct]{\matlabtextC $150$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{005}[rc][rc]{\matlabtextC $0$}%
\psfrag{006}[rc][rc]{\matlabtextC $500$}%
\psfrag{007}[rc][rc]{\matlabtextC $1000$}%
%
%% </ytick>

==> Figures/pemonte100922/snr64_mt80_eta0-111_CHIRP.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{006}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{007}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{008}[bc][bc]{\matlabtextB Signal: $\rho=64$, $M_T=80M_\odot$, $\eta=0.111$}%
\psfrag{009}[bc][bc]{\matlabtextB $\#$}%
\psfrag{010}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $0$}%
\psfrag{001}[ct][ct]{\matlabtextC $50$}%
\psfrag{002}[ct][ct]{\matlabtextC $100$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{003}[rc][rc]{\matlabtextC $0$}%
\psfrag{004}[rc][rc]{\matlabtextC $500$}%
\psfrag{005}[rc][rc]{\matlabtextC $1000$}%
%
%% </ytick>

==> Figures/pemonte100922/snr64_mt80_eta0-111_CHIRPsmall.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{006}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{007}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{008}[bc][bc]{\matlabtextB Signal: $\rho=64$, $M_T=80M_\odot$, $\eta=0.111$}%
\psfrag{009}[bc][bc]{\matlabtextB $\#$}%
\psfrag{010}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $0$}%
\psfrag{001}[ct][ct]{\matlabtextC $50$}%
\psfrag{002}[ct][ct]{\matlabtextC $100$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{003}[rc][rc]{\matlabtextC $0$}%
\psfrag{004}[rc][rc]{\matlabtextC $500$}%
\psfrag{005}[rc][rc]{\matlabtextC $1000$}%
%
%% </ytick>

==> Figures/pemonte100922/snr64_mt80_eta0-167_CHIRP.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{010}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{011}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{012}[bc][bc]{\matlabtextB Signal: $\rho=64$, $M_T=80M_\odot$, $\eta=0.167$}%
\psfrag{013}[bc][bc]{\matlabtextB $\#$}%
\psfrag{014}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 20$}%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $20$}%
\psfrag{003}[ct][ct]{\matlabtextC $40$}%
\psfrag{004}[ct][ct]{\matlabtextC $60$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{005}[rc][rc]{\matlabtextC $0$}%
\psfrag{006}[rc][rc]{\matlabtextC $200$}%
\psfrag{007}[rc][rc]{\matlabtextC $400$}%
\psfrag{008}[rc][rc]{\matlabtextC $600$}%
\psfrag{009}[rc][rc]{\matlabtextC $800$}%
%
%% </ytick>

==> Figures/pemonte100922/snr64_mt80_eta0-167_CHIRPsmall.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{010}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{011}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{012}[bc][bc]{\matlabtextB Signal: $\rho=64$, $M_T=80M_\odot$, $\eta=0.167$}%
\psfrag{013}[bc][bc]{\matlabtextB $\#$}%
\psfrag{014}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 20$}%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $20$}%
\psfrag{003}[ct][ct]{\matlabtextC $40$}%
\psfrag{004}[ct][ct]{\matlabtextC $60$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{005}[rc][rc]{\matlabtextC $0$}%
\psfrag{006}[rc][rc]{\matlabtextC $200$}%
\psfrag{007}[rc][rc]{\matlabtextC $400$}%
\psfrag{008}[rc][rc]{\matlabtextC $600$}%
\psfrag{009}[rc][rc]{\matlabtextC $800$}%
%
%% </ytick>

==> Figures/pemonte100922/snr64_mt80_eta0-25_CHIRP.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{010}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{011}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{012}[bc][bc]{\matlabtextB Signal: $\rho=64$, $M_T=80M_\odot$, $\eta=0.25$}%
\psfrag{013}[bc][bc]{\matlabtextB $\#$}%
\psfrag{014}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 30$}%
\psfrag{001}[ct][ct]{\matlabtextC $\matlabfragNegXTick 20$}%
\psfrag{002}[ct][ct]{\matlabtextC $\matlabfragNegXTick 10$}%
\psfrag{003}[ct][ct]{\matlabtextC $0$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{004}[rc][rc]{\matlabtextC $0$}%
\psfrag{005}[rc][rc]{\matlabtextC $100$}%
\psfrag{006}[rc][rc]{\matlabtextC $200$}%
\psfrag{007}[rc][rc]{\matlabtextC $300$}%
\psfrag{008}[rc][rc]{\matlabtextC $400$}%
\psfrag{009}[rc][rc]{\matlabtextC $500$}%
%
%% </ytick>

==> Figures/pemonte100922/snr64_mt80_eta0-25_CHIRPsmall.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{010}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{011}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{012}[bc][bc]{\matlabtextB Signal: $\rho=64$, $M_T=80M_\odot$, $\eta=0.25$}%
\psfrag{013}[bc][bc]{\matlabtextB $\#$}%
\psfrag{014}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 30$}%
\psfrag{001}[ct][ct]{\matlabtextC $\matlabfragNegXTick 20$}%
\psfrag{002}[ct][ct]{\matlabtextC $\matlabfragNegXTick 10$}%
\psfrag{003}[ct][ct]{\matlabtextC $0$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{004}[rc][rc]{\matlabtextC $0$}%
\psfrag{005}[rc][rc]{\matlabtextC $100$}%
\psfrag{006}[rc][rc]{\matlabtextC $200$}%
\psfrag{007}[rc][rc]{\matlabtextC $300$}%
\psfrag{008}[rc][rc]{\matlabtextC $400$}%
\psfrag{009}[rc][rc]{\matlabtextC $500$}%
%
%% </ytick>

==> Figures/pemonte100922/snr8_mt30_eta0-05_CHIRP.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{014}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{015}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{016}[bc][bc]{\matlabtextB Signal: $\rho=8$, $M_T=30M_\odot$, $\eta=0.05$}%
\psfrag{017}[bc][bc]{\matlabtextB $\#$}%
\psfrag{018}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $0$}%
\psfrag{001}[ct][ct]{\matlabtextC $100$}%
\psfrag{002}[ct][ct]{\matlabtextC $200$}%
\psfrag{003}[ct][ct]{\matlabtextC $300$}%
\psfrag{004}[ct][ct]{\matlabtextC $400$}%
\psfrag{005}[ct][ct]{\matlabtextC $500$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{006}[rc][rc]{\matlabtextC $0$}%
\psfrag{007}[rc][rc]{\matlabtextC $200$}%
\psfrag{008}[rc][rc]{\matlabtextC $400$}%
\psfrag{009}[rc][rc]{\matlabtextC $600$}%
\psfrag{010}[rc][rc]{\matlabtextC $800$}%
\psfrag{011}[rc][rc]{\matlabtextC $1000$}%
\psfrag{012}[rc][rc]{\matlabtextC $1200$}%
\psfrag{013}[rc][rc]{\matlabtextC $1400$}%
%
%% </ytick>

==> Figures/pemonte100922/snr8_mt30_eta0-05_CHIRPsmall.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{014}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{015}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{016}[bc][bc]{\matlabtextB Signal: $\rho=8$, $M_T=30M_\odot$, $\eta=0.05$}%
\psfrag{017}[bc][bc]{\matlabtextB $\#$}%
\psfrag{018}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $0$}%
\psfrag{001}[ct][ct]{\matlabtextC $100$}%
\psfrag{002}[ct][ct]{\matlabtextC $200$}%
\psfrag{003}[ct][ct]{\matlabtextC $300$}%
\psfrag{004}[ct][ct]{\matlabtextC $400$}%
\psfrag{005}[ct][ct]{\matlabtextC $500$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{006}[rc][rc]{\matlabtextC $0$}%
\psfrag{007}[rc][rc]{\matlabtextC $200$}%
\psfrag{008}[rc][rc]{\matlabtextC $400$}%
\psfrag{009}[rc][rc]{\matlabtextC $600$}%
\psfrag{010}[rc][rc]{\matlabtextC $800$}%
\psfrag{011}[rc][rc]{\matlabtextC $1000$}%
\psfrag{012}[rc][rc]{\matlabtextC $1200$}%
\psfrag{013}[rc][rc]{\matlabtextC $1400$}%
%
%% </ytick>

==> Figures/pemonte100922/snr8_mt30_eta0-075_CHIRP.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{008}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{009}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{010}[bc][bc]{\matlabtextB Signal: $\rho=8$, $M_T=30M_\odot$, $\eta=0.075$}%
\psfrag{011}[bc][bc]{\matlabtextB $\#$}%
\psfrag{012}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 50$}%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $50$}%
\psfrag{003}[ct][ct]{\matlabtextC $100$}%
\psfrag{004}[ct][ct]{\matlabtextC $150$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{005}[rc][rc]{\matlabtextC $0$}%
\psfrag{006}[rc][rc]{\matlabtextC $500$}%
\psfrag{007}[rc][rc]{\matlabtextC $1000$}%
%
%% </ytick>

==> Figures/pemonte100922/snr8_mt30_eta0-075_CHIRPsmall.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{008}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{009}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{010}[bc][bc]{\matlabtextB Signal: $\rho=8$, $M_T=30M_\odot$, $\eta=0.075$}%
\psfrag{011}[bc][bc]{\matlabtextB $\#$}%
\psfrag{012}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 50$}%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $50$}%
\psfrag{003}[ct][ct]{\matlabtextC $100$}%
\psfrag{004}[ct][ct]{\matlabtextC $150$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{005}[rc][rc]{\matlabtextC $0$}%
\psfrag{006}[rc][rc]{\matlabtextC $500$}%
\psfrag{007}[rc][rc]{\matlabtextC $1000$}%
%
%% </ytick>

==> Figures/pemonte100922/snr8_mt30_eta0-111_CHIRP.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{011}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{012}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{013}[bc][bc]{\matlabtextB Signal: $\rho=8$, $M_T=30M_\odot$, $\eta=0.111$}%
\psfrag{014}[bc][bc]{\matlabtextB $\#$}%
\psfrag{015}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 50$}%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $50$}%
\psfrag{003}[ct][ct]{\matlabtextC $100$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{004}[rc][rc]{\matlabtextC $0$}%
\psfrag{005}[rc][rc]{\matlabtextC $200$}%
\psfrag{006}[rc][rc]{\matlabtextC $400$}%
\psfrag{007}[rc][rc]{\matlabtextC $600$}%
\psfrag{008}[rc][rc]{\matlabtextC $800$}%
\psfrag{009}[rc][rc]{\matlabtextC $1000$}%
\psfrag{010}[rc][rc]{\matlabtextC $1200$}%
%
%% </ytick>

==> Figures/pemonte100922/snr8_mt30_eta0-111_CHIRPsmall.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{011}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{012}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{013}[bc][bc]{\matlabtextB Signal: $\rho=8$, $M_T=30M_\odot$, $\eta=0.111$}%
\psfrag{014}[bc][bc]{\matlabtextB $\#$}%
\psfrag{015}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 50$}%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $50$}%
\psfrag{003}[ct][ct]{\matlabtextC $100$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{004}[rc][rc]{\matlabtextC $0$}%
\psfrag{005}[rc][rc]{\matlabtextC $200$}%
\psfrag{006}[rc][rc]{\matlabtextC $400$}%
\psfrag{007}[rc][rc]{\matlabtextC $600$}%
\psfrag{008}[rc][rc]{\matlabtextC $800$}%
\psfrag{009}[rc][rc]{\matlabtextC $1000$}%
\psfrag{010}[rc][rc]{\matlabtextC $1200$}%
%
%% </ytick>

==> Figures/pemonte100922/snr8_mt30_eta0-167_CHIRP.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{009}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{010}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{011}[bc][bc]{\matlabtextB Signal: $\rho=8$, $M_T=30M_\odot$, $\eta=0.167$}%
\psfrag{012}[bc][bc]{\matlabtextB $\#$}%
\psfrag{013}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 50$}%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $50$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{003}[rc][rc]{\matlabtextC $0$}%
\psfrag{004}[rc][rc]{\matlabtextC $200$}%
\psfrag{005}[rc][rc]{\matlabtextC $400$}%
\psfrag{006}[rc][rc]{\matlabtextC $600$}%
\psfrag{007}[rc][rc]{\matlabtextC $800$}%
\psfrag{008}[rc][rc]{\matlabtextC $1000$}%
%
%% </ytick>

==> Figures/pemonte100922/snr8_mt30_eta0-167_CHIRPsmall.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{009}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{010}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{011}[bc][bc]{\matlabtextB Signal: $\rho=8$, $M_T=30M_\odot$, $\eta=0.167$}%
\psfrag{012}[bc][bc]{\matlabtextB $\#$}%
\psfrag{013}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 50$}%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $50$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{003}[rc][rc]{\matlabtextC $0$}%
\psfrag{004}[rc][rc]{\matlabtextC $200$}%
\psfrag{005}[rc][rc]{\matlabtextC $400$}%
\psfrag{006}[rc][rc]{\matlabtextC $600$}%
\psfrag{007}[rc][rc]{\matlabtextC $800$}%
\psfrag{008}[rc][rc]{\matlabtextC $1000$}%
%
%% </ytick>

==> Figures/pemonte100922/snr8_mt30_eta0-25_CHIRP.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{007}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{008}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{009}[bc][bc]{\matlabtextB Signal: $\rho=8$, $M_T=30M_\odot$, $\eta=0.25$}%
\psfrag{010}[bc][bc]{\matlabtextB $\#$}%
\psfrag{011}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 100$}%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $100$}%
\psfrag{003}[ct][ct]{\matlabtextC $200$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{004}[rc][rc]{\matlabtextC $0$}%
\psfrag{005}[rc][rc]{\matlabtextC $500$}%
\psfrag{006}[rc][rc]{\matlabtextC $1000$}%
%
%% </ytick>

==> Figures/pemonte100922/snr8_mt30_eta0-25_CHIRPsmall.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{007}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{008}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{009}[bc][bc]{\matlabtextB Signal: $\rho=8$, $M_T=30M_\odot$, $\eta=0.25$}%
\psfrag{010}[bc][bc]{\matlabtextB $\#$}%
\psfrag{011}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 100$}%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $100$}%
\psfrag{003}[ct][ct]{\matlabtextC $200$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{004}[rc][rc]{\matlabtextC $0$}%
\psfrag{005}[rc][rc]{\matlabtextC $500$}%
\psfrag{006}[rc][rc]{\matlabtextC $1000$}%
%
%% </ytick>

==> Figures/pemonte100922/snr8_mt45_eta0-05_CHIRP.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{007}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{008}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{009}[bc][bc]{\matlabtextB Signal: $\rho=8$, $M_T=45M_\odot$, $\eta=0.05$}%
\psfrag{010}[bc][bc]{\matlabtextB $\#$}%
\psfrag{011}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 50$}%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $50$}%
\psfrag{003}[ct][ct]{\matlabtextC $100$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{004}[rc][rc]{\matlabtextC $0$}%
\psfrag{005}[rc][rc]{\matlabtextC $500$}%
\psfrag{006}[rc][rc]{\matlabtextC $1000$}%
%
%% </ytick>

==> Figures/pemonte100922/snr8_mt45_eta0-05_CHIRPsmall.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{007}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{008}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{009}[bc][bc]{\matlabtextB Signal: $\rho=8$, $M_T=45M_\odot$, $\eta=0.05$}%
\psfrag{010}[bc][bc]{\matlabtextB $\#$}%
\psfrag{011}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 50$}%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $50$}%
\psfrag{003}[ct][ct]{\matlabtextC $100$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{004}[rc][rc]{\matlabtextC $0$}%
\psfrag{005}[rc][rc]{\matlabtextC $500$}%
\psfrag{006}[rc][rc]{\matlabtextC $1000$}%
%
%% </ytick>

==> Figures/pemonte100922/snr8_mt45_eta0-075_CHIRP.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{008}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{009}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{010}[bc][bc]{\matlabtextB Signal: $\rho=8$, $M_T=45M_\odot$, $\eta=0.075$}%
\psfrag{011}[bc][bc]{\matlabtextB $\#$}%
\psfrag{012}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 50$}%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $50$}%
\psfrag{003}[ct][ct]{\matlabtextC $100$}%
\psfrag{004}[ct][ct]{\matlabtextC $150$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{005}[rc][rc]{\matlabtextC $0$}%
\psfrag{006}[rc][rc]{\matlabtextC $500$}%
\psfrag{007}[rc][rc]{\matlabtextC $1000$}%
%
%% </ytick>

==> Figures/pemonte100922/snr8_mt45_eta0-075_CHIRPsmall.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{008}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{009}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{010}[bc][bc]{\matlabtextB Signal: $\rho=8$, $M_T=45M_\odot$, $\eta=0.075$}%
\psfrag{011}[bc][bc]{\matlabtextB $\#$}%
\psfrag{012}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 50$}%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $50$}%
\psfrag{003}[ct][ct]{\matlabtextC $100$}%
\psfrag{004}[ct][ct]{\matlabtextC $150$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{005}[rc][rc]{\matlabtextC $0$}%
\psfrag{006}[rc][rc]{\matlabtextC $500$}%
\psfrag{007}[rc][rc]{\matlabtextC $1000$}%
%
%% </ytick>

==> Figures/pemonte100922/snr8_mt45_eta0-111_CHIRP.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{011}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{012}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{013}[bc][bc]{\matlabtextB Signal: $\rho=8$, $M_T=45M_\odot$, $\eta=0.111$}%
\psfrag{014}[bc][bc]{\matlabtextB $\#$}%
\psfrag{015}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 100$}%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $100$}%
\psfrag{003}[ct][ct]{\matlabtextC $200$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{004}[rc][rc]{\matlabtextC $0$}%
\psfrag{005}[rc][rc]{\matlabtextC $200$}%
\psfrag{006}[rc][rc]{\matlabtextC $400$}%
\psfrag{007}[rc][rc]{\matlabtextC $600$}%
\psfrag{008}[rc][rc]{\matlabtextC $800$}%
\psfrag{009}[rc][rc]{\matlabtextC $1000$}%
\psfrag{010}[rc][rc]{\matlabtextC $1200$}%
%
%% </ytick>

==> Figures/pemonte100922/snr8_mt45_eta0-111_CHIRPsmall.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{011}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{012}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{013}[bc][bc]{\matlabtextB Signal: $\rho=8$, $M_T=45M_\odot$, $\eta=0.111$}%
\psfrag{014}[bc][bc]{\matlabtextB $\#$}%
\psfrag{015}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 100$}%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $100$}%
\psfrag{003}[ct][ct]{\matlabtextC $200$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{004}[rc][rc]{\matlabtextC $0$}%
\psfrag{005}[rc][rc]{\matlabtextC $200$}%
\psfrag{006}[rc][rc]{\matlabtextC $400$}%
\psfrag{007}[rc][rc]{\matlabtextC $600$}%
\psfrag{008}[rc][rc]{\matlabtextC $800$}%
\psfrag{009}[rc][rc]{\matlabtextC $1000$}%
\psfrag{010}[rc][rc]{\matlabtextC $1200$}%
%
%% </ytick>

==> Figures/pemonte100922/snr8_mt45_eta0-167_CHIRP.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{009}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{010}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{011}[bc][bc]{\matlabtextB Signal: $\rho=8$, $M_T=45M_\odot$, $\eta=0.167$}%
\psfrag{012}[bc][bc]{\matlabtextB $\#$}%
\psfrag{013}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 100$}%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $100$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{003}[rc][rc]{\matlabtextC $0$}%
\psfrag{004}[rc][rc]{\matlabtextC $200$}%
\psfrag{005}[rc][rc]{\matlabtextC $400$}%
\psfrag{006}[rc][rc]{\matlabtextC $600$}%
\psfrag{007}[rc][rc]{\matlabtextC $800$}%
\psfrag{008}[rc][rc]{\matlabtextC $1000$}%
%
%% </ytick>

==> Figures/pemonte100922/snr8_mt45_eta0-167_CHIRPsmall.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{009}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{010}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{011}[bc][bc]{\matlabtextB Signal: $\rho=8$, $M_T=45M_\odot$, $\eta=0.167$}%
\psfrag{012}[bc][bc]{\matlabtextB $\#$}%
\psfrag{013}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 100$}%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $100$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{003}[rc][rc]{\matlabtextC $0$}%
\psfrag{004}[rc][rc]{\matlabtextC $200$}%
\psfrag{005}[rc][rc]{\matlabtextC $400$}%
\psfrag{006}[rc][rc]{\matlabtextC $600$}%
\psfrag{007}[rc][rc]{\matlabtextC $800$}%
\psfrag{008}[rc][rc]{\matlabtextC $1000$}%
%
%% </ytick>

==> Figures/pemonte100922/snr8_mt45_eta0-25_CHIRP.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{013}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{014}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{015}[bc][bc]{\matlabtextB Signal: $\rho=8$, $M_T=45M_\odot$, $\eta=0.25$}%
\psfrag{016}[bc][bc]{\matlabtextB $\#$}%
\psfrag{017}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 80$}%
\psfrag{001}[ct][ct]{\matlabtextC $\matlabfragNegXTick 60$}%
\psfrag{002}[ct][ct]{\matlabtextC $\matlabfragNegXTick 40$}%
\psfrag{003}[ct][ct]{\matlabtextC $\matlabfragNegXTick 20$}%
\psfrag{004}[ct][ct]{\matlabtextC $0$}%
\psfrag{005}[ct][ct]{\matlabtextC $20$}%
\psfrag{006}[ct][ct]{\matlabtextC $40$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{007}[rc][rc]{\matlabtextC $0$}%
\psfrag{008}[rc][rc]{\matlabtextC $200$}%
\psfrag{009}[rc][rc]{\matlabtextC $400$}%
\psfrag{010}[rc][rc]{\matlabtextC $600$}%
\psfrag{011}[rc][rc]{\matlabtextC $800$}%
\psfrag{012}[rc][rc]{\matlabtextC $1000$}%
%
%% </ytick>

==> Figures/pemonte100922/snr8_mt45_eta0-25_CHIRPsmall.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{013}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{014}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{015}[bc][bc]{\matlabtextB Signal: $\rho=8$, $M_T=45M_\odot$, $\eta=0.25$}%
\psfrag{016}[bc][bc]{\matlabtextB $\#$}%
\psfrag{017}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 80$}%
\psfrag{001}[ct][ct]{\matlabtextC $\matlabfragNegXTick 60$}%
\psfrag{002}[ct][ct]{\matlabtextC $\matlabfragNegXTick 40$}%
\psfrag{003}[ct][ct]{\matlabtextC $\matlabfragNegXTick 20$}%
\psfrag{004}[ct][ct]{\matlabtextC $0$}%
\psfrag{005}[ct][ct]{\matlabtextC $20$}%
\psfrag{006}[ct][ct]{\matlabtextC $40$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{007}[rc][rc]{\matlabtextC $0$}%
\psfrag{008}[rc][rc]{\matlabtextC $200$}%
\psfrag{009}[rc][rc]{\matlabtextC $400$}%
\psfrag{010}[rc][rc]{\matlabtextC $600$}%
\psfrag{011}[rc][rc]{\matlabtextC $800$}%
\psfrag{012}[rc][rc]{\matlabtextC $1000$}%
%
%% </ytick>

==> Figures/pemonte100922/snr8_mt67-5_eta0-05_CHIRP.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{011}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{012}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{013}[bc][bc]{\matlabtextB Signal: $\rho=8$, $M_T=67.5M_\odot$, $\eta=0.05$}%
\psfrag{014}[bc][bc]{\matlabtextB $\#$}%
\psfrag{015}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 100$}%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $100$}%
\psfrag{003}[ct][ct]{\matlabtextC $200$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{004}[rc][rc]{\matlabtextC $0$}%
\psfrag{005}[rc][rc]{\matlabtextC $200$}%
\psfrag{006}[rc][rc]{\matlabtextC $400$}%
\psfrag{007}[rc][rc]{\matlabtextC $600$}%
\psfrag{008}[rc][rc]{\matlabtextC $800$}%
\psfrag{009}[rc][rc]{\matlabtextC $1000$}%
\psfrag{010}[rc][rc]{\matlabtextC $1200$}%
%
%% </ytick>

==> Figures/pemonte100922/snr8_mt67-5_eta0-05_CHIRPsmall.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{011}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{012}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{013}[bc][bc]{\matlabtextB Signal: $\rho=8$, $M_T=67.5M_\odot$, $\eta=0.05$}%
\psfrag{014}[bc][bc]{\matlabtextB $\#$}%
\psfrag{015}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 100$}%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $100$}%
\psfrag{003}[ct][ct]{\matlabtextC $200$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{004}[rc][rc]{\matlabtextC $0$}%
\psfrag{005}[rc][rc]{\matlabtextC $200$}%
\psfrag{006}[rc][rc]{\matlabtextC $400$}%
\psfrag{007}[rc][rc]{\matlabtextC $600$}%
\psfrag{008}[rc][rc]{\matlabtextC $800$}%
\psfrag{009}[rc][rc]{\matlabtextC $1000$}%
\psfrag{010}[rc][rc]{\matlabtextC $1200$}%
%
%% </ytick>

==> Figures/pemonte100922/snr8_mt67-5_eta0-075_CHIRP.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{009}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{010}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{011}[bc][bc]{\matlabtextB Signal: $\rho=8$, $M_T=67.5M_\odot$, $\eta=0.075$}%
\psfrag{012}[bc][bc]{\matlabtextB $\#$}%
\psfrag{013}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 100$}%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $100$}%
\psfrag{003}[ct][ct]{\matlabtextC $200$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{004}[rc][rc]{\matlabtextC $0$}%
\psfrag{005}[rc][rc]{\matlabtextC $200$}%
\psfrag{006}[rc][rc]{\matlabtextC $400$}%
\psfrag{007}[rc][rc]{\matlabtextC $600$}%
\psfrag{008}[rc][rc]{\matlabtextC $800$}%
%
%% </ytick>

==> Figures/pemonte100922/snr8_mt67-5_eta0-075_CHIRPsmall.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{009}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{010}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{011}[bc][bc]{\matlabtextB Signal: $\rho=8$, $M_T=67.5M_\odot$, $\eta=0.075$}%
\psfrag{012}[bc][bc]{\matlabtextB $\#$}%
\psfrag{013}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 100$}%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $100$}%
\psfrag{003}[ct][ct]{\matlabtextC $200$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{004}[rc][rc]{\matlabtextC $0$}%
\psfrag{005}[rc][rc]{\matlabtextC $200$}%
\psfrag{006}[rc][rc]{\matlabtextC $400$}%
\psfrag{007}[rc][rc]{\matlabtextC $600$}%
\psfrag{008}[rc][rc]{\matlabtextC $800$}%
%
%% </ytick>

==> Figures/pemonte100922/snr8_mt67-5_eta0-111_CHIRP.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{010}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{011}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{012}[bc][bc]{\matlabtextB Signal: $\rho=8$, $M_T=67.5M_\odot$, $\eta=0.111$}%
\psfrag{013}[bc][bc]{\matlabtextB $\#$}%
\psfrag{014}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 100$}%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $100$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{003}[rc][rc]{\matlabtextC $0$}%
\psfrag{004}[rc][rc]{\matlabtextC $100$}%
\psfrag{005}[rc][rc]{\matlabtextC $200$}%
\psfrag{006}[rc][rc]{\matlabtextC $300$}%
\psfrag{007}[rc][rc]{\matlabtextC $400$}%
\psfrag{008}[rc][rc]{\matlabtextC $500$}%
\psfrag{009}[rc][rc]{\matlabtextC $600$}%
%
%% </ytick>

==> Figures/pemonte100922/snr8_mt67-5_eta0-111_CHIRPsmall.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{010}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{011}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{012}[bc][bc]{\matlabtextB Signal: $\rho=8$, $M_T=67.5M_\odot$, $\eta=0.111$}%
\psfrag{013}[bc][bc]{\matlabtextB $\#$}%
\psfrag{014}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 100$}%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $100$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{003}[rc][rc]{\matlabtextC $0$}%
\psfrag{004}[rc][rc]{\matlabtextC $100$}%
\psfrag{005}[rc][rc]{\matlabtextC $200$}%
\psfrag{006}[rc][rc]{\matlabtextC $300$}%
\psfrag{007}[rc][rc]{\matlabtextC $400$}%
\psfrag{008}[rc][rc]{\matlabtextC $500$}%
\psfrag{009}[rc][rc]{\matlabtextC $600$}%
%
%% </ytick>

==> Figures/pemonte100922/snr8_mt67-5_eta0-167_CHIRP.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{011}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{012}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{013}[bc][bc]{\matlabtextB Signal: $\rho=8$, $M_T=67.5M_\odot$, $\eta=0.167$}%
\psfrag{014}[bc][bc]{\matlabtextB $\#$}%
\psfrag{015}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 100$}%
\psfrag{001}[ct][ct]{\matlabtextC $\matlabfragNegXTick 50$}%
\psfrag{002}[ct][ct]{\matlabtextC $0$}%
\psfrag{003}[ct][ct]{\matlabtextC $50$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{004}[rc][rc]{\matlabtextC $0$}%
\psfrag{005}[rc][rc]{\matlabtextC $100$}%
\psfrag{006}[rc][rc]{\matlabtextC $200$}%
\psfrag{007}[rc][rc]{\matlabtextC $300$}%
\psfrag{008}[rc][rc]{\matlabtextC $400$}%
\psfrag{009}[rc][rc]{\matlabtextC $500$}%
\psfrag{010}[rc][rc]{\matlabtextC $600$}%
%
%% </ytick>

==> Figures/pemonte100922/snr8_mt67-5_eta0-167_CHIRPsmall.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{011}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{012}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{013}[bc][bc]{\matlabtextB Signal: $\rho=8$, $M_T=67.5M_\odot$, $\eta=0.167$}%
\psfrag{014}[bc][bc]{\matlabtextB $\#$}%
\psfrag{015}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 100$}%
\psfrag{001}[ct][ct]{\matlabtextC $\matlabfragNegXTick 50$}%
\psfrag{002}[ct][ct]{\matlabtextC $0$}%
\psfrag{003}[ct][ct]{\matlabtextC $50$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{004}[rc][rc]{\matlabtextC $0$}%
\psfrag{005}[rc][rc]{\matlabtextC $100$}%
\psfrag{006}[rc][rc]{\matlabtextC $200$}%
\psfrag{007}[rc][rc]{\matlabtextC $300$}%
\psfrag{008}[rc][rc]{\matlabtextC $400$}%
\psfrag{009}[rc][rc]{\matlabtextC $500$}%
\psfrag{010}[rc][rc]{\matlabtextC $600$}%
%
%% </ytick>

==> Figures/pemonte100922/snr8_mt67-5_eta0-25_CHIRP.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{009}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{010}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{011}[bc][bc]{\matlabtextB Signal: $\rho=8$, $M_T=67.5M_\odot$, $\eta=0.25$}%
\psfrag{012}[bc][bc]{\matlabtextB $\#$}%
\psfrag{013}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 100$}%
\psfrag{001}[ct][ct]{\matlabtextC $\matlabfragNegXTick 50$}%
\psfrag{002}[ct][ct]{\matlabtextC $0$}%
\psfrag{003}[ct][ct]{\matlabtextC $50$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{004}[rc][rc]{\matlabtextC $0$}%
\psfrag{005}[rc][rc]{\matlabtextC $100$}%
\psfrag{006}[rc][rc]{\matlabtextC $200$}%
\psfrag{007}[rc][rc]{\matlabtextC $300$}%
\psfrag{008}[rc][rc]{\matlabtextC $400$}%
%
%% </ytick>

==> Figures/pemonte100922/snr8_mt67-5_eta0-25_CHIRPsmall.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{009}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{010}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{011}[bc][bc]{\matlabtextB Signal: $\rho=8$, $M_T=67.5M_\odot$, $\eta=0.25$}%
\psfrag{012}[bc][bc]{\matlabtextB $\#$}%
\psfrag{013}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 100$}%
\psfrag{001}[ct][ct]{\matlabtextC $\matlabfragNegXTick 50$}%
\psfrag{002}[ct][ct]{\matlabtextC $0$}%
\psfrag{003}[ct][ct]{\matlabtextC $50$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{004}[rc][rc]{\matlabtextC $0$}%
\psfrag{005}[rc][rc]{\matlabtextC $100$}%
\psfrag{006}[rc][rc]{\matlabtextC $200$}%
\psfrag{007}[rc][rc]{\matlabtextC $300$}%
\psfrag{008}[rc][rc]{\matlabtextC $400$}%
%
%% </ytick>

==> Figures/pemonte100922/snr8_mt80_eta0-05_CHIRP.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{010}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{011}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{012}[bc][bc]{\matlabtextB Signal: $\rho=8$, $M_T=80M_\odot$, $\eta=0.05$}%
\psfrag{013}[bc][bc]{\matlabtextB $\#$}%
\psfrag{014}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 100$}%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $100$}%
\psfrag{003}[ct][ct]{\matlabtextC $200$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{004}[rc][rc]{\matlabtextC $0$}%
\psfrag{005}[rc][rc]{\matlabtextC $200$}%
\psfrag{006}[rc][rc]{\matlabtextC $400$}%
\psfrag{007}[rc][rc]{\matlabtextC $600$}%
\psfrag{008}[rc][rc]{\matlabtextC $800$}%
\psfrag{009}[rc][rc]{\matlabtextC $1000$}%
%
%% </ytick>

==> Figures/pemonte100922/snr8_mt80_eta0-05_CHIRPsmall.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{010}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{011}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{012}[bc][bc]{\matlabtextB Signal: $\rho=8$, $M_T=80M_\odot$, $\eta=0.05$}%
\psfrag{013}[bc][bc]{\matlabtextB $\#$}%
\psfrag{014}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 100$}%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $100$}%
\psfrag{003}[ct][ct]{\matlabtextC $200$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{004}[rc][rc]{\matlabtextC $0$}%
\psfrag{005}[rc][rc]{\matlabtextC $200$}%
\psfrag{006}[rc][rc]{\matlabtextC $400$}%
\psfrag{007}[rc][rc]{\matlabtextC $600$}%
\psfrag{008}[rc][rc]{\matlabtextC $800$}%
\psfrag{009}[rc][rc]{\matlabtextC $1000$}%
%
%% </ytick>

==> Figures/pemonte100922/snr8_mt80_eta0-075_CHIRP.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{007}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{008}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{009}[bc][bc]{\matlabtextB Signal: $\rho=8$, $M_T=80M_\odot$, $\eta=0.075$}%
\psfrag{010}[bc][bc]{\matlabtextB $\#$}%
\psfrag{011}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 100$}%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $100$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{003}[rc][rc]{\matlabtextC $0$}%
\psfrag{004}[rc][rc]{\matlabtextC $200$}%
\psfrag{005}[rc][rc]{\matlabtextC $400$}%
\psfrag{006}[rc][rc]{\matlabtextC $600$}%
%
%% </ytick>

==> Figures/pemonte100922/snr8_mt80_eta0-075_CHIRPsmall.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{007}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{008}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{009}[bc][bc]{\matlabtextB Signal: $\rho=8$, $M_T=80M_\odot$, $\eta=0.075$}%
\psfrag{010}[bc][bc]{\matlabtextB $\#$}%
\psfrag{011}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 100$}%
\psfrag{001}[ct][ct]{\matlabtextC $0$}%
\psfrag{002}[ct][ct]{\matlabtextC $100$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{003}[rc][rc]{\matlabtextC $0$}%
\psfrag{004}[rc][rc]{\matlabtextC $200$}%
\psfrag{005}[rc][rc]{\matlabtextC $400$}%
\psfrag{006}[rc][rc]{\matlabtextC $600$}%
%
%% </ytick>

==> Figures/pemonte100922/snr8_mt80_eta0-111_CHIRP.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{011}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{012}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{013}[bc][bc]{\matlabtextB Signal: $\rho=8$, $M_T=80M_\odot$, $\eta=0.111$}%
\psfrag{014}[bc][bc]{\matlabtextB $\#$}%
\psfrag{015}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 100$}%
\psfrag{001}[ct][ct]{\matlabtextC $\matlabfragNegXTick 50$}%
\psfrag{002}[ct][ct]{\matlabtextC $0$}%
\psfrag{003}[ct][ct]{\matlabtextC $50$}%
\psfrag{004}[ct][ct]{\matlabtextC $100$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{005}[rc][rc]{\matlabtextC $0$}%
\psfrag{006}[rc][rc]{\matlabtextC $100$}%
\psfrag{007}[rc][rc]{\matlabtextC $200$}%
\psfrag{008}[rc][rc]{\matlabtextC $300$}%
\psfrag{009}[rc][rc]{\matlabtextC $400$}%
\psfrag{010}[rc][rc]{\matlabtextC $500$}%
%
%% </ytick>

==> Figures/pemonte100922/snr8_mt80_eta0-111_CHIRPsmall.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{011}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{012}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{013}[bc][bc]{\matlabtextB Signal: $\rho=8$, $M_T=80M_\odot$, $\eta=0.111$}%
\psfrag{014}[bc][bc]{\matlabtextB $\#$}%
\psfrag{015}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 100$}%
\psfrag{001}[ct][ct]{\matlabtextC $\matlabfragNegXTick 50$}%
\psfrag{002}[ct][ct]{\matlabtextC $0$}%
\psfrag{003}[ct][ct]{\matlabtextC $50$}%
\psfrag{004}[ct][ct]{\matlabtextC $100$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{005}[rc][rc]{\matlabtextC $0$}%
\psfrag{006}[rc][rc]{\matlabtextC $100$}%
\psfrag{007}[rc][rc]{\matlabtextC $200$}%
\psfrag{008}[rc][rc]{\matlabtextC $300$}%
\psfrag{009}[rc][rc]{\matlabtextC $400$}%
\psfrag{010}[rc][rc]{\matlabtextC $500$}%
%
%% </ytick>

==> Figures/pemonte100922/snr8_mt80_eta0-167_CHIRP.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{008}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{009}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{010}[bc][bc]{\matlabtextB Signal: $\rho=8$, $M_T=80M_\odot$, $\eta=0.167$}%
\psfrag{011}[bc][bc]{\matlabtextB $\#$}%
\psfrag{012}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 100$}%
\psfrag{001}[ct][ct]{\matlabtextC $\matlabfragNegXTick 50$}%
\psfrag{002}[ct][ct]{\matlabtextC $0$}%
\psfrag{003}[ct][ct]{\matlabtextC $50$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{004}[rc][rc]{\matlabtextC $0$}%
\psfrag{005}[rc][rc]{\matlabtextC $100$}%
\psfrag{006}[rc][rc]{\matlabtextC $200$}%
\psfrag{007}[rc][rc]{\matlabtextC $300$}%
%
%% </ytick>

==> Figures/pemonte100922/snr8_mt80_eta0-167_CHIRPsmall.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{008}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{009}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{010}[bc][bc]{\matlabtextB Signal: $\rho=8$, $M_T=80M_\odot$, $\eta=0.167$}%
\psfrag{011}[bc][bc]{\matlabtextB $\#$}%
\psfrag{012}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 100$}%
\psfrag{001}[ct][ct]{\matlabtextC $\matlabfragNegXTick 50$}%
\psfrag{002}[ct][ct]{\matlabtextC $0$}%
\psfrag{003}[ct][ct]{\matlabtextC $50$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{004}[rc][rc]{\matlabtextC $0$}%
\psfrag{005}[rc][rc]{\matlabtextC $100$}%
\psfrag{006}[rc][rc]{\matlabtextC $200$}%
\psfrag{007}[rc][rc]{\matlabtextC $300$}%
%
%% </ytick>

==> Figures/pemonte100922/snr8_mt80_eta0-25_CHIRP.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{010}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{011}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{012}[bc][bc]{\matlabtextB Signal: $\rho=8$, $M_T=80M_\odot$, $\eta=0.25$}%
\psfrag{013}[bc][bc]{\matlabtextB $\#$}%
\psfrag{014}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 100$}%
\psfrag{001}[ct][ct]{\matlabtextC $\matlabfragNegXTick 50$}%
\psfrag{002}[ct][ct]{\matlabtextC $0$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{003}[rc][rc]{\matlabtextC $0$}%
\psfrag{004}[rc][rc]{\matlabtextC $50$}%
\psfrag{005}[rc][rc]{\matlabtextC $100$}%
\psfrag{006}[rc][rc]{\matlabtextC $150$}%
\psfrag{007}[rc][rc]{\matlabtextC $200$}%
\psfrag{008}[rc][rc]{\matlabtextC $250$}%
\psfrag{009}[rc][rc]{\matlabtextC $300$}%
%
%% </ytick>

==> Figures/pemonte100922/snr8_mt80_eta0-25_CHIRPsmall.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{010}[cl][cl]{\matlabtextA RWF (TT3)}%
\psfrag{011}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{012}[bc][bc]{\matlabtextB Signal: $\rho=8$, $M_T=80M_\odot$, $\eta=0.25$}%
\psfrag{013}[bc][bc]{\matlabtextB $\#$}%
\psfrag{014}[tc][tc]{\matlabtextB Percentage error in chirp mass}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 100$}%
\psfrag{001}[ct][ct]{\matlabtextC $\matlabfragNegXTick 50$}%
\psfrag{002}[ct][ct]{\matlabtextC $0$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{003}[rc][rc]{\matlabtextC $0$}%
\psfrag{004}[rc][rc]{\matlabtextC $50$}%
\psfrag{005}[rc][rc]{\matlabtextC $100$}%
\psfrag{006}[rc][rc]{\matlabtextC $150$}%
\psfrag{007}[rc][rc]{\matlabtextC $200$}%
\psfrag{008}[rc][rc]{\matlabtextC $250$}%
\psfrag{009}[rc][rc]{\matlabtextC $300$}%
%
%% </ytick>

==> Figures/pephase.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{012}[cl][cl]{\matlabtextA (3.8,14)$M_\odot$ 3rd harmonic}%
\psfrag{013}[cl][cl]{\matlabtextA (1.4,10)$M_\odot$ 2nd harmonic}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{014}[tc][tc]{\matlabtextB Time to coalescence /s}%
\psfrag{015}[bc][bc]{\matlabtextB Phase}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 2$}%
\psfrag{001}[ct][ct]{\matlabtextC $\matlabfragNegXTick 1.5$}%
\psfrag{002}[ct][ct]{\matlabtextC $\matlabfragNegXTick 1$}%
\psfrag{003}[ct][ct]{\matlabtextC $\matlabfragNegXTick 0.5$}%
\psfrag{004}[ct][ct]{\matlabtextC $0$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{005}[rc][rc]{\matlabtextC $-1200$}%
\psfrag{006}[rc][rc]{\matlabtextC $-1000$}%
\psfrag{007}[rc][rc]{\matlabtextC $-800$}%
\psfrag{008}[rc][rc]{\matlabtextC $-600$}%
\psfrag{009}[rc][rc]{\matlabtextC $-400$}%
\psfrag{010}[rc][rc]{\matlabtextC $-200$}%
\psfrag{011}[rc][rc]{\matlabtextC $0$}%
%
%% </ytick>


==> Figures/pespec.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{029}[cl][cl]{\matlabtextA (3.8,14)$M_\odot$ 3rd harmonic}%
\psfrag{030}[cl][cl]{\matlabtextA (1.4,10)$M_\odot$ 2nd harmonic}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{031}[bc][bc]{\matlabtextB Normalised observed spectra}%
\psfrag{032}[tc][tc]{\matlabtextB f /Hz}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{022}[ct][ct]{\matlabtextC $10^{1}$}%
\psfrag{023}[ct][ct]{\matlabtextC $10^{2}$}%
\psfrag{024}[ct][ct]{\matlabtextC $10^{3}$}%
%
\providecommand\matlabtextD{\fontsize{16}{16}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextD $0$}%
\psfrag{001}[ct][ct]{\matlabtextD $0.1$}%
\psfrag{002}[ct][ct]{\matlabtextD $0.2$}%
\psfrag{003}[ct][ct]{\matlabtextD $0.3$}%
\psfrag{004}[ct][ct]{\matlabtextD $0.4$}%
\psfrag{005}[ct][ct]{\matlabtextD $0.5$}%
\psfrag{006}[ct][ct]{\matlabtextD $0.6$}%
\psfrag{007}[ct][ct]{\matlabtextD $0.7$}%
\psfrag{008}[ct][ct]{\matlabtextD $0.8$}%
\psfrag{009}[ct][ct]{\matlabtextD $0.9$}%
\psfrag{010}[ct][ct]{\matlabtextD $1$}%
%
%% </xtick>
%
%% <ytick>
%
\providecommand\matlabtextE{\fontsize{10}{10}\selectfont\strut}%
\psfrag{025}[rc][rc]{\matlabtextE $10^{-6}$}%
\psfrag{026}[rc][rc]{\matlabtextE $10^{-5}$}%
\psfrag{027}[rc][rc]{\matlabtextE $10^{-4}$}%
\psfrag{028}[rc][rc]{\matlabtextE $10^{-3}$}%
%
\providecommand\matlabtextF{\fontsize{16}{16}\selectfont\strut}%
\psfrag{011}[rc][rc]{\matlabtextF $0$}%
\psfrag{012}[rc][rc]{\matlabtextF $0.1$}%
\psfrag{013}[rc][rc]{\matlabtextF $0.2$}%
\psfrag{014}[rc][rc]{\matlabtextF $0.3$}%
\psfrag{015}[rc][rc]{\matlabtextF $0.4$}%
\psfrag{016}[rc][rc]{\matlabtextF $0.5$}%
\psfrag{017}[rc][rc]{\matlabtextF $0.6$}%
\psfrag{018}[rc][rc]{\matlabtextF $0.7$}%
\psfrag{019}[rc][rc]{\matlabtextF $0.8$}%
\psfrag{020}[rc][rc]{\matlabtextF $0.9$}%
\psfrag{021}[rc][rc]{\matlabtextF $1$}%
%
%% </ytick>


==> Figures/polars.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{12}{12}\selectfont\strut}%
\psfrag{000}[bc][bc]{\matlabtextA y}%
\psfrag{001}[tc][tc]{\matlabtextA x}%
%
%% </text>

==> Figures/sepevolve.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{12}{12}\selectfont\strut}%
\psfrag{000}[bc][bc]{\matlabtextA $a(t)$}%
\psfrag{001}[tc][tc]{\matlabtextA Time}%
%
%% </text>

==> Figures/snrvsmass.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{014}[cl][cl]{\matlabtextA Tapered}%
\psfrag{015}[cl][cl]{\matlabtextA Untapered}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{016}[bc][bc]{\matlabtextB SNR}%
\psfrag{017}[tc][tc]{\matlabtextB Total mass /$M_\odot$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $0$}%
\psfrag{001}[ct][ct]{\matlabtextC $20$}%
\psfrag{002}[ct][ct]{\matlabtextC $40$}%
\psfrag{003}[ct][ct]{\matlabtextC $60$}%
\psfrag{004}[ct][ct]{\matlabtextC $80$}%
\psfrag{005}[ct][ct]{\matlabtextC $100$}%
\psfrag{006}[ct][ct]{\matlabtextC $120$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{007}[rc][rc]{\matlabtextC $4$}%
\psfrag{008}[rc][rc]{\matlabtextC $6$}%
\psfrag{009}[rc][rc]{\matlabtextC $8$}%
\psfrag{010}[rc][rc]{\matlabtextC $10$}%
\psfrag{011}[rc][rc]{\matlabtextC $12$}%
\psfrag{012}[rc][rc]{\matlabtextC $14$}%
\psfrag{013}[rc][rc]{\matlabtextC $16$}%
%
%% </ytick>


==> Figures/spaambbbh1.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{020}[bc][bc]{\matlabtextA RWF (SPA)}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{021}[bc][bc]{\matlabtextB $\tau_3 /{\, \rm s}$}%
\psfrag{022}[tc][tc]{\matlabtextB $\tau_0 /{\, \rm s}$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{006}[ct][ct]{\matlabtextC $2$}%
\psfrag{007}[ct][ct]{\matlabtextC $4$}%
\psfrag{008}[ct][ct]{\matlabtextC $6$}%
\psfrag{009}[ct][ct]{\matlabtextC $8$}%
\psfrag{010}[ct][ct]{\matlabtextC $10$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{000}[lc][lc]{\matlabtextC $0$}%
\psfrag{001}[lc][lc]{\matlabtextC $0.2$}%
\psfrag{002}[lc][lc]{\matlabtextC $0.4$}%
\psfrag{003}[lc][lc]{\matlabtextC $0.6$}%
\psfrag{004}[lc][lc]{\matlabtextC $0.8$}%
\psfrag{005}[lc][lc]{\matlabtextC $1$}%
\psfrag{011}[rc][rc]{\matlabtextC $0.3$}%
\psfrag{012}[rc][rc]{\matlabtextC $0.4$}%
\psfrag{013}[rc][rc]{\matlabtextC $0.5$}%
\psfrag{014}[rc][rc]{\matlabtextC $0.6$}%
\psfrag{015}[rc][rc]{\matlabtextC $0.7$}%
\psfrag{016}[rc][rc]{\matlabtextC $0.8$}%
\psfrag{017}[rc][rc]{\matlabtextC $0.9$}%
\psfrag{018}[rc][rc]{\matlabtextC $1$}%
\psfrag{019}[rc][rc]{\matlabtextC $1.1$}%
%
%% </ytick>

==> Figures/spaambbbh2.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{017}[bc][bc]{\matlabtextA RWF (SPA)}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{018}[bc][bc]{\matlabtextB $\tau_3 /{\, \rm s}$}%
\psfrag{019}[tc][tc]{\matlabtextB $\tau_0 /{\, \rm s}$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{006}[ct][ct]{\matlabtextC $1$}%
\psfrag{007}[ct][ct]{\matlabtextC $2$}%
\psfrag{008}[ct][ct]{\matlabtextC $3$}%
\psfrag{009}[ct][ct]{\matlabtextC $4$}%
\psfrag{010}[ct][ct]{\matlabtextC $5$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{000}[lc][lc]{\matlabtextC $0$}%
\psfrag{001}[lc][lc]{\matlabtextC $0.2$}%
\psfrag{002}[lc][lc]{\matlabtextC $0.4$}%
\psfrag{003}[lc][lc]{\matlabtextC $0.6$}%
\psfrag{004}[lc][lc]{\matlabtextC $0.8$}%
\psfrag{005}[lc][lc]{\matlabtextC $1$}%
\psfrag{011}[rc][rc]{\matlabtextC $0.2$}%
\psfrag{012}[rc][rc]{\matlabtextC $0.4$}%
\psfrag{013}[rc][rc]{\matlabtextC $0.6$}%
\psfrag{014}[rc][rc]{\matlabtextC $0.8$}%
\psfrag{015}[rc][rc]{\matlabtextC $1$}%
\psfrag{016}[rc][rc]{\matlabtextC $1.2$}%
%
%% </ytick>

==> Figures/spaambbns.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{020}[bc][bc]{\matlabtextA RWF (SPA)}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{021}[bc][bc]{\matlabtextB $\tau_3 /{\, \rm s}$}%
\psfrag{022}[tc][tc]{\matlabtextB $\tau_0 /{\, \rm s}$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{006}[ct][ct]{\matlabtextC $22$}%
\psfrag{007}[ct][ct]{\matlabtextC $24$}%
\psfrag{008}[ct][ct]{\matlabtextC $26$}%
\psfrag{009}[ct][ct]{\matlabtextC $28$}%
\psfrag{010}[ct][ct]{\matlabtextC $30$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{000}[lc][lc]{\matlabtextC $0$}%
\psfrag{001}[lc][lc]{\matlabtextC $0.2$}%
\psfrag{002}[lc][lc]{\matlabtextC $0.4$}%
\psfrag{003}[lc][lc]{\matlabtextC $0.6$}%
\psfrag{004}[lc][lc]{\matlabtextC $0.8$}%
\psfrag{005}[lc][lc]{\matlabtextC $1$}%
\psfrag{011}[rc][rc]{\matlabtextC $0.82$}%
\psfrag{012}[rc][rc]{\matlabtextC $0.84$}%
\psfrag{013}[rc][rc]{\matlabtextC $0.86$}%
\psfrag{014}[rc][rc]{\matlabtextC $0.88$}%
\psfrag{015}[rc][rc]{\matlabtextC $0.9$}%
\psfrag{016}[rc][rc]{\matlabtextC $0.92$}%
\psfrag{017}[rc][rc]{\matlabtextC $0.94$}%
\psfrag{018}[rc][rc]{\matlabtextC $0.96$}%
\psfrag{019}[rc][rc]{\matlabtextC $0.98$}%
%
%% </ytick>

==> Figures/spaambimbbh1.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{016}[bc][bc]{\matlabtextA RWF (SPA)}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{017}[bc][bc]{\matlabtextB $\tau_3 /{\, \rm s}$}%
\psfrag{018}[tc][tc]{\matlabtextB $\tau_0 /{\, \rm s}$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{006}[ct][ct]{\matlabtextC $0$}%
\psfrag{007}[ct][ct]{\matlabtextC $0.5$}%
\psfrag{008}[ct][ct]{\matlabtextC $1$}%
\psfrag{009}[ct][ct]{\matlabtextC $1.5$}%
\psfrag{010}[ct][ct]{\matlabtextC $2$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{000}[lc][lc]{\matlabtextC $0$}%
\psfrag{001}[lc][lc]{\matlabtextC $0.2$}%
\psfrag{002}[lc][lc]{\matlabtextC $0.4$}%
\psfrag{003}[lc][lc]{\matlabtextC $0.6$}%
\psfrag{004}[lc][lc]{\matlabtextC $0.8$}%
\psfrag{005}[lc][lc]{\matlabtextC $1$}%
\psfrag{011}[rc][rc]{\matlabtextC $0$}%
\psfrag{012}[rc][rc]{\matlabtextC $0.5$}%
\psfrag{013}[rc][rc]{\matlabtextC $1$}%
\psfrag{014}[rc][rc]{\matlabtextC $1.5$}%
\psfrag{015}[rc][rc]{\matlabtextC $2$}%
%
%% </ytick>

==> Figures/spaambimbbh2.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{016}[bc][bc]{\matlabtextA RWF (SPA)}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{017}[bc][bc]{\matlabtextB $\tau_3 /{\, \rm s}$}%
\psfrag{018}[tc][tc]{\matlabtextB $\tau_0 /{\, \rm s}$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{006}[ct][ct]{\matlabtextC $0$}%
\psfrag{007}[ct][ct]{\matlabtextC $0.5$}%
\psfrag{008}[ct][ct]{\matlabtextC $1$}%
\psfrag{009}[ct][ct]{\matlabtextC $1.5$}%
\psfrag{010}[ct][ct]{\matlabtextC $2$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{000}[lc][lc]{\matlabtextC $0$}%
\psfrag{001}[lc][lc]{\matlabtextC $0.2$}%
\psfrag{002}[lc][lc]{\matlabtextC $0.4$}%
\psfrag{003}[lc][lc]{\matlabtextC $0.6$}%
\psfrag{004}[lc][lc]{\matlabtextC $0.8$}%
\psfrag{005}[lc][lc]{\matlabtextC $1$}%
\psfrag{011}[rc][rc]{\matlabtextC $0$}%
\psfrag{012}[rc][rc]{\matlabtextC $0.5$}%
\psfrag{013}[rc][rc]{\matlabtextC $1$}%
\psfrag{014}[rc][rc]{\matlabtextC $1.5$}%
\psfrag{015}[rc][rc]{\matlabtextC $2$}%
%
%% </ytick>

==> Figures/spaambnsbh.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{017}[bc][bc]{\matlabtextA RWF (SPA)}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{018}[bc][bc]{\matlabtextB $\tau_3 /{\, \rm s}$}%
\psfrag{019}[tc][tc]{\matlabtextB $\tau_0 /{\, \rm s}$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{006}[ct][ct]{\matlabtextC $0$}%
\psfrag{007}[ct][ct]{\matlabtextC $5$}%
\psfrag{008}[ct][ct]{\matlabtextC $10$}%
\psfrag{009}[ct][ct]{\matlabtextC $15$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{000}[lc][lc]{\matlabtextC $0$}%
\psfrag{001}[lc][lc]{\matlabtextC $0.2$}%
\psfrag{002}[lc][lc]{\matlabtextC $0.4$}%
\psfrag{003}[lc][lc]{\matlabtextC $0.6$}%
\psfrag{004}[lc][lc]{\matlabtextC $0.8$}%
\psfrag{005}[lc][lc]{\matlabtextC $1$}%
\psfrag{010}[rc][rc]{\matlabtextC $0.2$}%
\psfrag{011}[rc][rc]{\matlabtextC $0.4$}%
\psfrag{012}[rc][rc]{\matlabtextC $0.6$}%
\psfrag{013}[rc][rc]{\matlabtextC $0.8$}%
\psfrag{014}[rc][rc]{\matlabtextC $1$}%
\psfrag{015}[rc][rc]{\matlabtextC $1.2$}%
\psfrag{016}[rc][rc]{\matlabtextC $1.4$}%
%
%% </ytick>

==> Figures/spec010mr10.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{014}[cl][cl]{\matlabtextA RWF}%
\psfrag{015}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{016}[bc][bc]{\matlabtextB $f{\left|H(f)\right|}^2/S_h(f)$}%
\psfrag{017}[tc][tc]{\matlabtextB f /Hz}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $10^{2}$}%
\psfrag{001}[ct][ct]{\matlabtextC $10^{3}$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{002}[rc][rc]{\matlabtextC $0$}%
\psfrag{003}[rc][rc]{\matlabtextC $100$}%
\psfrag{004}[rc][rc]{\matlabtextC $200$}%
\psfrag{005}[rc][rc]{\matlabtextC $300$}%
\psfrag{006}[rc][rc]{\matlabtextC $400$}%
\psfrag{007}[rc][rc]{\matlabtextC $500$}%
\psfrag{008}[rc][rc]{\matlabtextC $0$}%
\psfrag{009}[rc][rc]{\matlabtextC $100$}%
\psfrag{010}[rc][rc]{\matlabtextC $200$}%
\psfrag{011}[rc][rc]{\matlabtextC $300$}%
\psfrag{012}[rc][rc]{\matlabtextC $400$}%
\psfrag{013}[rc][rc]{\matlabtextC $500$}%
%
%% </ytick>

==> Figures/spec110mr10.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{011}[cl][cl]{\matlabtextA RWF}%
\psfrag{012}[cl][cl]{\matlabtextA FWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{013}[bc][bc]{\matlabtextB $f{\left|H(f)\right|}^2S_h(f)$}%
\psfrag{014}[tc][tc]{\matlabtextB f /Hz}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $10^{2}$}%
\psfrag{001}[ct][ct]{\matlabtextC $10^{3}$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{002}[rc][rc]{\matlabtextC $1000$}%
\psfrag{003}[rc][rc]{\matlabtextC $2000$}%
\psfrag{004}[rc][rc]{\matlabtextC $3000$}%
\psfrag{005}[rc][rc]{\matlabtextC $4000$}%
\psfrag{006}[rc][rc]{\matlabtextC $0$}%
\psfrag{007}[rc][rc]{\matlabtextC $1000$}%
\psfrag{008}[rc][rc]{\matlabtextC $2000$}%
\psfrag{009}[rc][rc]{\matlabtextC $3000$}%
\psfrag{010}[rc][rc]{\matlabtextC $4000$}%
%
%% </ytick>

==> Figures/spectra20.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{008}[cl][cl]{\matlabtextA SPA}%
\psfrag{009}[cl][cl]{\matlabtextA H$_\sigma$}%
\psfrag{010}[cl][cl]{\matlabtextA H$_S$}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{011}[bc][bc]{\matlabtextB $20\ M_\odot$}%
\psfrag{012}[bc][bc]{\matlabtextB $f.|H(f)|^2 / S_h(f)$}%
\psfrag{013}[tc][tc]{\matlabtextB Frequency $/\, \rm Hz$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $10^2$}%
\psfrag{001}[ct][ct]{\matlabtextC $10^3$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{002}[rc][rc]{\matlabtextC $10^-8$}%
\psfrag{003}[rc][rc]{\matlabtextC $10^-7$}%
\psfrag{004}[rc][rc]{\matlabtextC $10^-6$}%
\psfrag{005}[rc][rc]{\matlabtextC $10^-5$}%
\psfrag{006}[rc][rc]{\matlabtextC $10^-4$}%
\psfrag{007}[rc][rc]{\matlabtextC $10^-3$}%
%
%% </ytick>


==> Figures/spectra80.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{008}[cl][cl]{\matlabtextA SPA}%
\psfrag{009}[cl][cl]{\matlabtextA H$_\sigma$}%
\psfrag{010}[cl][cl]{\matlabtextA H$_S$}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{011}[bc][bc]{\matlabtextB $80\ M_\odot$}%
\psfrag{012}[bc][bc]{\matlabtextB $f.|H(f)|^2 / S_h(f)$}%
\psfrag{013}[tc][tc]{\matlabtextB Frequency $/\, \rm Hz$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $10^2$}%
\psfrag{001}[ct][ct]{\matlabtextC $10^3$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{002}[rc][rc]{\matlabtextC $10^-8$}%
\psfrag{003}[rc][rc]{\matlabtextC $10^-7$}%
\psfrag{004}[rc][rc]{\matlabtextC $10^-6$}%
\psfrag{005}[rc][rc]{\matlabtextC $10^-5$}%
\psfrag{006}[rc][rc]{\matlabtextC $10^-4$}%
\psfrag{007}[rc][rc]{\matlabtextC $10^-3$}%
%
%% </ytick>


==> Figures/taperapplication2.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{12}{12}\selectfont\strut}%
\psfrag{004}[tc][tc]{\matlabtextA Array index}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $0$}%
\psfrag{001}[ct][ct]{\matlabtextB $50$}%
\psfrag{002}[ct][ct]{\matlabtextB $100$}%
\psfrag{003}[ct][ct]{\matlabtextB $150$}%
%
%% </xtick>

==> Figures/tddiffs.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{12}{12}\selectfont\strut}%
\psfrag{006}[tc][tc]{\matlabtextA $x$-$y$ same scale for given system}%
\psfrag{007}[bc][bc]{\matlabtextA TD optimal template for LIGO ($h_+$)}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $(3,10)M_\odot$}%
\psfrag{001}[ct][ct]{\matlabtextB $(3,15)M_\odot$}%
\psfrag{002}[ct][ct]{\matlabtextB $(3,30)M_\odot$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{003}[rc][rc]{\matlabtextB $i=90^\circ$}%
\psfrag{004}[rc][rc]{\matlabtextB $i=45^\circ$}%
\psfrag{005}[rc][rc]{\matlabtextB $i=0^\circ$}%
%
%% </ytick>


==> Figures/tf2SNR10_1.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{12}{12}\selectfont\strut}%
\psfrag{019}[bc][bc]{\matlabtextA Recovered total mass /$M_\odot$}%
\psfrag{020}[tc][tc]{\matlabtextA Injected total mass /$M_\odot$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\fontsize{10}{10}\selectfont\strut}%
\psfrag{004}[ct][ct]{\matlabtextB $20$}%
\psfrag{005}[ct][ct]{\matlabtextB $40$}%
\psfrag{006}[ct][ct]{\matlabtextB $60$}%
\psfrag{007}[ct][ct]{\matlabtextB $80$}%
\psfrag{008}[ct][ct]{\matlabtextB $100$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{000}[lc][lc]{\matlabtextB $0$}%
\psfrag{001}[lc][lc]{\matlabtextB $5$}%
\psfrag{002}[lc][lc]{\matlabtextB $10$}%
\psfrag{003}[lc][lc]{\matlabtextB $15$}%
\psfrag{009}[rc][rc]{\matlabtextB $10$}%
\psfrag{010}[rc][rc]{\matlabtextB $20$}%
\psfrag{011}[rc][rc]{\matlabtextB $30$}%
\psfrag{012}[rc][rc]{\matlabtextB $40$}%
\psfrag{013}[rc][rc]{\matlabtextB $50$}%
\psfrag{014}[rc][rc]{\matlabtextB $60$}%
\psfrag{015}[rc][rc]{\matlabtextB $70$}%
\psfrag{016}[rc][rc]{\matlabtextB $80$}%
\psfrag{017}[rc][rc]{\matlabtextB $90$}%
\psfrag{018}[rc][rc]{\matlabtextB $100$}%
%
%% </ytick>

==> Figures/timewindows2.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{009}[bc][bc]{\matlabtextA $w_T(t;0.033)$}%
\psfrag{010}[tc][tc]{\matlabtextA $w_T(t;0.1)$}%
\psfrag{011}[bc][bc]{\matlabtextA $w_T(t;0.01)$}%
\psfrag{012}[bc][bc]{\matlabtextA $s_T(t)$}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{008}[tc][tc]{\matlabtextB Time /s}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $0.8$}%
\psfrag{001}[ct][ct]{\matlabtextC $0.85$}%
\psfrag{002}[ct][ct]{\matlabtextC $0.9$}%
\psfrag{003}[ct][ct]{\matlabtextC $0.95$}%
\psfrag{004}[ct][ct]{\matlabtextC $1$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{005}[rc][rc]{\matlabtextC $0$}%
\psfrag{006}[rc][rc]{\matlabtextC $0.5$}%
\psfrag{007}[rc][rc]{\matlabtextC $1$}%
%
%% </ytick>


==> Figures/tt3SNR10.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{018}[bc][bc]{\matlabtextA RWF}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{019}[bc][bc]{\matlabtextB Recovered total mass /$\, M_\odot$}%
\psfrag{020}[tc][tc]{\matlabtextB Injected total mass /$\, M_\odot$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{004}[ct][ct]{\matlabtextC $20$}%
\psfrag{005}[ct][ct]{\matlabtextC $40$}%
\psfrag{006}[ct][ct]{\matlabtextC $60$}%
\psfrag{007}[ct][ct]{\matlabtextC $80$}%
\psfrag{008}[ct][ct]{\matlabtextC $100$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{000}[lc][lc]{\matlabtextC $0$}%
\psfrag{001}[lc][lc]{\matlabtextC $5$}%
\psfrag{002}[lc][lc]{\matlabtextC $10$}%
\psfrag{003}[lc][lc]{\matlabtextC $15$}%
\psfrag{009}[rc][rc]{\matlabtextC $20$}%
\psfrag{010}[rc][rc]{\matlabtextC $30$}%
\psfrag{011}[rc][rc]{\matlabtextC $40$}%
\psfrag{012}[rc][rc]{\matlabtextC $50$}%
\psfrag{013}[rc][rc]{\matlabtextC $60$}%
\psfrag{014}[rc][rc]{\matlabtextC $70$}%
\psfrag{015}[rc][rc]{\matlabtextC $80$}%
\psfrag{016}[rc][rc]{\matlabtextC $90$}%
\psfrag{017}[rc][rc]{\matlabtextC $100$}%
%
%% </ytick>

==> Figures/tt3SNR10_1.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{12}{12}\selectfont\strut}%
\psfrag{019}[bc][bc]{\matlabtextA Recovered total mass /$M_\odot$}%
\psfrag{020}[tc][tc]{\matlabtextA Injected total mass /$M_\odot$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\fontsize{10}{10}\selectfont\strut}%
\psfrag{004}[ct][ct]{\matlabtextB $20$}%
\psfrag{005}[ct][ct]{\matlabtextB $40$}%
\psfrag{006}[ct][ct]{\matlabtextB $60$}%
\psfrag{007}[ct][ct]{\matlabtextB $80$}%
\psfrag{008}[ct][ct]{\matlabtextB $100$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{000}[lc][lc]{\matlabtextB $0$}%
\psfrag{001}[lc][lc]{\matlabtextB $5$}%
\psfrag{002}[lc][lc]{\matlabtextB $10$}%
\psfrag{003}[lc][lc]{\matlabtextB $15$}%
\psfrag{009}[rc][rc]{\matlabtextB $10$}%
\psfrag{010}[rc][rc]{\matlabtextB $20$}%
\psfrag{011}[rc][rc]{\matlabtextB $30$}%
\psfrag{012}[rc][rc]{\matlabtextB $40$}%
\psfrag{013}[rc][rc]{\matlabtextB $50$}%
\psfrag{014}[rc][rc]{\matlabtextB $60$}%
\psfrag{015}[rc][rc]{\matlabtextB $70$}%
\psfrag{016}[rc][rc]{\matlabtextB $80$}%
\psfrag{017}[rc][rc]{\matlabtextB $90$}%
\psfrag{018}[rc][rc]{\matlabtextB $100$}%
%
%% </ytick>

==> Figures/tt3SNR10new.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{018}[bc][bc]{\matlabtextA RWF (TT3)}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{019}[bc][bc]{\matlabtextB Recovered total mass /$\, M_\odot$}%
\psfrag{020}[tc][tc]{\matlabtextB Injected total mass /$\, M_\odot$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{004}[ct][ct]{\matlabtextC $20$}%
\psfrag{005}[ct][ct]{\matlabtextC $40$}%
\psfrag{006}[ct][ct]{\matlabtextC $60$}%
\psfrag{007}[ct][ct]{\matlabtextC $80$}%
\psfrag{008}[ct][ct]{\matlabtextC $100$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{000}[lc][lc]{\matlabtextC $0$}%
\psfrag{001}[lc][lc]{\matlabtextC $5$}%
\psfrag{002}[lc][lc]{\matlabtextC $10$}%
\psfrag{003}[lc][lc]{\matlabtextC $15$}%
\psfrag{009}[rc][rc]{\matlabtextC $20$}%
\psfrag{010}[rc][rc]{\matlabtextC $30$}%
\psfrag{011}[rc][rc]{\matlabtextC $40$}%
\psfrag{012}[rc][rc]{\matlabtextC $50$}%
\psfrag{013}[rc][rc]{\matlabtextC $60$}%
\psfrag{014}[rc][rc]{\matlabtextC $70$}%
\psfrag{015}[rc][rc]{\matlabtextC $80$}%
\psfrag{016}[rc][rc]{\matlabtextC $90$}%
\psfrag{017}[rc][rc]{\matlabtextC $100$}%
%
%% </ytick>

==> Figures/tt3ambbbh1.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{020}[bc][bc]{\matlabtextA RWF (TT3)}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{021}[bc][bc]{\matlabtextB $\tau_3 /{\, \rm s}$}%
\psfrag{022}[tc][tc]{\matlabtextB $\tau_0 /{\, \rm s}$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{006}[ct][ct]{\matlabtextC $2$}%
\psfrag{007}[ct][ct]{\matlabtextC $4$}%
\psfrag{008}[ct][ct]{\matlabtextC $6$}%
\psfrag{009}[ct][ct]{\matlabtextC $8$}%
\psfrag{010}[ct][ct]{\matlabtextC $10$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{000}[lc][lc]{\matlabtextC $0$}%
\psfrag{001}[lc][lc]{\matlabtextC $0.2$}%
\psfrag{002}[lc][lc]{\matlabtextC $0.4$}%
\psfrag{003}[lc][lc]{\matlabtextC $0.6$}%
\psfrag{004}[lc][lc]{\matlabtextC $0.8$}%
\psfrag{005}[lc][lc]{\matlabtextC $1$}%
\psfrag{011}[rc][rc]{\matlabtextC $0.3$}%
\psfrag{012}[rc][rc]{\matlabtextC $0.4$}%
\psfrag{013}[rc][rc]{\matlabtextC $0.5$}%
\psfrag{014}[rc][rc]{\matlabtextC $0.6$}%
\psfrag{015}[rc][rc]{\matlabtextC $0.7$}%
\psfrag{016}[rc][rc]{\matlabtextC $0.8$}%
\psfrag{017}[rc][rc]{\matlabtextC $0.9$}%
\psfrag{018}[rc][rc]{\matlabtextC $1$}%
\psfrag{019}[rc][rc]{\matlabtextC $1.1$}%
%
%% </ytick>

==> Figures/tt3ambbbh2.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{021}[bc][bc]{\matlabtextA RWF (TT3)}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{022}[bc][bc]{\matlabtextB $\tau_3 /{\, \rm s}$}%
\psfrag{023}[tc][tc]{\matlabtextB $\tau_0 /{\, \rm s}$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{006}[ct][ct]{\matlabtextC $0$}%
\psfrag{007}[ct][ct]{\matlabtextC $1$}%
\psfrag{008}[ct][ct]{\matlabtextC $2$}%
\psfrag{009}[ct][ct]{\matlabtextC $3$}%
\psfrag{010}[ct][ct]{\matlabtextC $4$}%
\psfrag{011}[ct][ct]{\matlabtextC $5$}%
\psfrag{012}[ct][ct]{\matlabtextC $6$}%
\psfrag{013}[ct][ct]{\matlabtextC $7$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{000}[lc][lc]{\matlabtextC $0$}%
\psfrag{001}[lc][lc]{\matlabtextC $0.2$}%
\psfrag{002}[lc][lc]{\matlabtextC $0.4$}%
\psfrag{003}[lc][lc]{\matlabtextC $0.6$}%
\psfrag{004}[lc][lc]{\matlabtextC $0.8$}%
\psfrag{005}[lc][lc]{\matlabtextC $1$}%
\psfrag{014}[rc][rc]{\matlabtextC $0.2$}%
\psfrag{015}[rc][rc]{\matlabtextC $0.4$}%
\psfrag{016}[rc][rc]{\matlabtextC $0.6$}%
\psfrag{017}[rc][rc]{\matlabtextC $0.8$}%
\psfrag{018}[rc][rc]{\matlabtextC $1$}%
\psfrag{019}[rc][rc]{\matlabtextC $1.2$}%
\psfrag{020}[rc][rc]{\matlabtextC $1.4$}%
%
%% </ytick>

==> Figures/tt3ambbns.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{020}[bc][bc]{\matlabtextA RWF (TT3)}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{021}[bc][bc]{\matlabtextB $\tau_3 /{\, \rm s}$}%
\psfrag{022}[tc][tc]{\matlabtextB $\tau_0 /{\, \rm s}$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{006}[ct][ct]{\matlabtextC $22$}%
\psfrag{007}[ct][ct]{\matlabtextC $24$}%
\psfrag{008}[ct][ct]{\matlabtextC $26$}%
\psfrag{009}[ct][ct]{\matlabtextC $28$}%
\psfrag{010}[ct][ct]{\matlabtextC $30$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{000}[lc][lc]{\matlabtextC $0$}%
\psfrag{001}[lc][lc]{\matlabtextC $0.2$}%
\psfrag{002}[lc][lc]{\matlabtextC $0.4$}%
\psfrag{003}[lc][lc]{\matlabtextC $0.6$}%
\psfrag{004}[lc][lc]{\matlabtextC $0.8$}%
\psfrag{005}[lc][lc]{\matlabtextC $1$}%
\psfrag{011}[rc][rc]{\matlabtextC $0.82$}%
\psfrag{012}[rc][rc]{\matlabtextC $0.84$}%
\psfrag{013}[rc][rc]{\matlabtextC $0.86$}%
\psfrag{014}[rc][rc]{\matlabtextC $0.88$}%
\psfrag{015}[rc][rc]{\matlabtextC $0.9$}%
\psfrag{016}[rc][rc]{\matlabtextC $0.92$}%
\psfrag{017}[rc][rc]{\matlabtextC $0.94$}%
\psfrag{018}[rc][rc]{\matlabtextC $0.96$}%
\psfrag{019}[rc][rc]{\matlabtextC $0.98$}%
%
%% </ytick>

==> Figures/tt3ambimbbh1.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{017}[bc][bc]{\matlabtextA RWF (TT3)}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{018}[bc][bc]{\matlabtextB $\tau_3 /{\, \rm s}$}%
\psfrag{019}[tc][tc]{\matlabtextB $\tau_0 /{\, \rm s}$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{006}[ct][ct]{\matlabtextC $0$}%
\psfrag{007}[ct][ct]{\matlabtextC $1$}%
\psfrag{008}[ct][ct]{\matlabtextC $2$}%
\psfrag{009}[ct][ct]{\matlabtextC $3$}%
\psfrag{010}[ct][ct]{\matlabtextC $4$}%
\psfrag{011}[ct][ct]{\matlabtextC $5$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{000}[lc][lc]{\matlabtextC $0$}%
\psfrag{001}[lc][lc]{\matlabtextC $0.2$}%
\psfrag{002}[lc][lc]{\matlabtextC $0.4$}%
\psfrag{003}[lc][lc]{\matlabtextC $0.6$}%
\psfrag{004}[lc][lc]{\matlabtextC $0.8$}%
\psfrag{005}[lc][lc]{\matlabtextC $1$}%
\psfrag{012}[rc][rc]{\matlabtextC $0$}%
\psfrag{013}[rc][rc]{\matlabtextC $0.5$}%
\psfrag{014}[rc][rc]{\matlabtextC $1$}%
\psfrag{015}[rc][rc]{\matlabtextC $1.5$}%
\psfrag{016}[rc][rc]{\matlabtextC $2$}%
%
%% </ytick>

==> Figures/tt3ambimbbh2.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{016}[bc][bc]{\matlabtextA RWF (TT3)}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{017}[bc][bc]{\matlabtextB $\tau_3 /{\, \rm s}$}%
\psfrag{018}[tc][tc]{\matlabtextB $\tau_0 /{\, \rm s}$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{006}[ct][ct]{\matlabtextC $0$}%
\psfrag{007}[ct][ct]{\matlabtextC $0.5$}%
\psfrag{008}[ct][ct]{\matlabtextC $1$}%
\psfrag{009}[ct][ct]{\matlabtextC $1.5$}%
\psfrag{010}[ct][ct]{\matlabtextC $2$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{000}[lc][lc]{\matlabtextC $0$}%
\psfrag{001}[lc][lc]{\matlabtextC $0.2$}%
\psfrag{002}[lc][lc]{\matlabtextC $0.4$}%
\psfrag{003}[lc][lc]{\matlabtextC $0.6$}%
\psfrag{004}[lc][lc]{\matlabtextC $0.8$}%
\psfrag{005}[lc][lc]{\matlabtextC $1$}%
\psfrag{011}[rc][rc]{\matlabtextC $0$}%
\psfrag{012}[rc][rc]{\matlabtextC $0.5$}%
\psfrag{013}[rc][rc]{\matlabtextC $1$}%
\psfrag{014}[rc][rc]{\matlabtextC $1.5$}%
\psfrag{015}[rc][rc]{\matlabtextC $2$}%
%
%% </ytick>

==> Figures/tt3ambnsbh.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{020}[bc][bc]{\matlabtextA RWF (TT3)}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{021}[bc][bc]{\matlabtextB $\tau_3 /{\, \rm s}$}%
\psfrag{022}[tc][tc]{\matlabtextB $\tau_0 /{\, \rm s}$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{006}[ct][ct]{\matlabtextC $0$}%
\psfrag{007}[ct][ct]{\matlabtextC $5$}%
\psfrag{008}[ct][ct]{\matlabtextC $10$}%
\psfrag{009}[ct][ct]{\matlabtextC $15$}%
\psfrag{010}[ct][ct]{\matlabtextC $20$}%
\psfrag{011}[ct][ct]{\matlabtextC $25$}%
\psfrag{012}[ct][ct]{\matlabtextC $30$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{000}[lc][lc]{\matlabtextC $0$}%
\psfrag{001}[lc][lc]{\matlabtextC $0.2$}%
\psfrag{002}[lc][lc]{\matlabtextC $0.4$}%
\psfrag{003}[lc][lc]{\matlabtextC $0.6$}%
\psfrag{004}[lc][lc]{\matlabtextC $0.8$}%
\psfrag{005}[lc][lc]{\matlabtextC $1$}%
\psfrag{013}[rc][rc]{\matlabtextC $0.2$}%
\psfrag{014}[rc][rc]{\matlabtextC $0.4$}%
\psfrag{015}[rc][rc]{\matlabtextC $0.6$}%
\psfrag{016}[rc][rc]{\matlabtextC $0.8$}%
\psfrag{017}[rc][rc]{\matlabtextC $1$}%
\psfrag{018}[rc][rc]{\matlabtextC $1.2$}%
\psfrag{019}[rc][rc]{\matlabtextC $1.4$}%
%
%% </ytick>

==> Figures/tt3mchirp.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{020}[bc][bc]{\matlabtextA RWF (TT3)}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{021}[bc][bc]{\matlabtextB Recovered chirp mass /$\, M_\odot$}%
\psfrag{022}[tc][tc]{\matlabtextB Injected chirp mass /\, $M_\odot$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{006}[ct][ct]{\matlabtextC $0$}%
\psfrag{007}[ct][ct]{\matlabtextC $10$}%
\psfrag{008}[ct][ct]{\matlabtextC $20$}%
\psfrag{009}[ct][ct]{\matlabtextC $30$}%
\psfrag{010}[ct][ct]{\matlabtextC $40$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{000}[lc][lc]{\matlabtextC $0$}%
\psfrag{001}[lc][lc]{\matlabtextC $0.2$}%
\psfrag{002}[lc][lc]{\matlabtextC $0.4$}%
\psfrag{003}[lc][lc]{\matlabtextC $0.6$}%
\psfrag{004}[lc][lc]{\matlabtextC $0.8$}%
\psfrag{005}[lc][lc]{\matlabtextC $1$}%
\psfrag{011}[rc][rc]{\matlabtextC $0$}%
\psfrag{012}[rc][rc]{\matlabtextC $5$}%
\psfrag{013}[rc][rc]{\matlabtextC $10$}%
\psfrag{014}[rc][rc]{\matlabtextC $15$}%
\psfrag{015}[rc][rc]{\matlabtextC $20$}%
\psfrag{016}[rc][rc]{\matlabtextC $25$}%
\psfrag{017}[rc][rc]{\matlabtextC $30$}%
\psfrag{018}[rc][rc]{\matlabtextC $35$}%
\psfrag{019}[rc][rc]{\matlabtextC $40$}%
%
%% </ytick>

==> Figures/tt3mtot.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{10}{10}\selectfont\strut}%
\psfrag{020}[bc][bc]{\matlabtextA RWF (TT3)}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{021}[bc][bc]{\matlabtextB Recovered total mass /$\, M_\odot$}%
\psfrag{022}[tc][tc]{\matlabtextB Injected total mass /$\ ,M_\odot$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\fontsize{10}{10}\selectfont\strut}%
\psfrag{006}[ct][ct]{\matlabtextC $20$}%
\psfrag{007}[ct][ct]{\matlabtextC $40$}%
\psfrag{008}[ct][ct]{\matlabtextC $60$}%
\psfrag{009}[ct][ct]{\matlabtextC $80$}%
\psfrag{010}[ct][ct]{\matlabtextC $100$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{000}[lc][lc]{\matlabtextC $0$}%
\psfrag{001}[lc][lc]{\matlabtextC $0.2$}%
\psfrag{002}[lc][lc]{\matlabtextC $0.4$}%
\psfrag{003}[lc][lc]{\matlabtextC $0.6$}%
\psfrag{004}[lc][lc]{\matlabtextC $0.8$}%
\psfrag{005}[lc][lc]{\matlabtextC $1$}%
\psfrag{011}[rc][rc]{\matlabtextC $20$}%
\psfrag{012}[rc][rc]{\matlabtextC $30$}%
\psfrag{013}[rc][rc]{\matlabtextC $40$}%
\psfrag{014}[rc][rc]{\matlabtextC $50$}%
\psfrag{015}[rc][rc]{\matlabtextC $60$}%
\psfrag{016}[rc][rc]{\matlabtextC $70$}%
\psfrag{017}[rc][rc]{\matlabtextC $80$}%
\psfrag{018}[rc][rc]{\matlabtextC $90$}%
\psfrag{019}[rc][rc]{\matlabtextC $100$}%
%
%% </ytick>

==> Figures/twobody.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{12}{12}\selectfont\strut}%
\psfrag{001}[tr][tr]{\matlabtextA $y$}%
\psfrag{002}[tl][tl]{\matlabtextA $x$}%
%
\providecommand\matlabtextB{\fontsize{12}{12}\selectfont\strut}%
\psfrag{000}[bc][bc]{\matlabtextB Time}%
%
%% </text>


==> Figures/ulbhmass.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{12}{12}\selectfont\strut}%
\psfrag{008}[tc][tc]{\matlabtextA Black hole mass /$M_\odot$}%
\psfrag{009}[bc][bc]{\matlabtextA Rate /$\, {\rm yr}^{-1}{\rm L}^{-1}_{10}$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $5$}%
\psfrag{001}[ct][ct]{\matlabtextB $10$}%
\psfrag{002}[ct][ct]{\matlabtextB $15$}%
\psfrag{003}[ct][ct]{\matlabtextB $20$}%
\psfrag{004}[ct][ct]{\matlabtextB $25$}%
\psfrag{005}[ct][ct]{\matlabtextB $30$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{006}[rc][rc]{\matlabtextB $10^{-3}$}%
\psfrag{007}[rc][rc]{\matlabtextB $10^{-2}$}%
%
%% </ytick>

==> Figures/ultotal.tex <==

%
%% <text>
%
\providecommand\matlabtextA{\fontsize{12}{12}\selectfont\strut}%
\psfrag{009}[tc][tc]{\matlabtextA Total mass /$M_\odot$}%
\psfrag{010}[bc][bc]{\matlabtextA Rate /$\, {\rm yr}^{-1}{\rm L}^{-1}_{10}$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $5$}%
\psfrag{001}[ct][ct]{\matlabtextB $10$}%
\psfrag{002}[ct][ct]{\matlabtextB $15$}%
\psfrag{003}[ct][ct]{\matlabtextB $20$}%
\psfrag{004}[ct][ct]{\matlabtextB $25$}%
\psfrag{005}[ct][ct]{\matlabtextB $30$}%
\psfrag{006}[ct][ct]{\matlabtextB $35$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{007}[rc][rc]{\matlabtextB $10^{-3}$}%
\psfrag{008}[rc][rc]{\matlabtextB $10^{-2}$}%
%
%% </ytick>
